Single-Modal Entropy based Active Learning for Visual Question Answering

Constructing a large-scale labeled dataset in the real world, especially for high-level tasks (eg, Visual Question Answering), can be expensive and time-consuming. In addition, with the ever-growing amounts of data and architecture complexity, Active Learning has become an important aspect of computer vision research. In this work, we address Active Learning in the multi-modal setting of Visual Question Answering (VQA). In light of the multi-modal inputs, image and question, we propose a novel method for effective sample acquisition through the use of ad hoc single-modal branches for each input to leverage its information. Our mutual information based sample acquisition strategy Single-Modal Entropic Measure (SMEM) in addition to our self-distillation technique enables the sample acquisitor to exploit all present modalities and find the most informative samples. Our novel idea is simple to implement, cost-efficient, and readily adaptable to other multi-modal tasks. We confirm our findings on various VQA datasets through state-of-the-art performance by comparing to existing Active Learning baselines.

==> Legacy/unused_1_sec_intro.tex <==
%1) X is an important problem and core challenges
%2) Previous work on X has addressed these with Y, but the problems with this are Z.
%3) In this work we do W. Thorough explanation.
%4) Contributions, and experiments



%1) X is an important problem and core challenges
% \textbf{(Recently, deep active Learning has been studied extensively. Active Learning is important to resolve data issues in various deep learning tasks.)}
The recent successes of learning-based computer vision methods relies heavily on abundant annotated training examples, which may be prohibitively costly to label or impossible to obtain at large scale~\cite{deng2009imagenet}. 
In order to mitigate this drawback, Active Learning (AL)~\cite{cohn1996active} has been introduced to minimize the number of expensive labels for the supervised training of deep neural networks by selecting (or \emph{sampling}) a subset of informative samples from a large unlabeled collection of data~\cite{settles2009active,tong2001support}.
AL has shown high classification performance with low labeling costs for computer vision tasks such as image classification~\cite{beluch2018power,gal2017deep,li2013adaptive,sener2017active} and semantic segmentation~\cite{gorriz2017cost,kuo2018cost,yang2017suggestive}. 

% do we need to explain active learning? ----------------------

% Active learning algorithms aim to minimize the number of expensive labels for supervised training of deep neural networks (DNNs) by selecting a subset of informative examples from a large unlabeled collection of data~\cite{tong2001support,settles2009active}.
% The subset is annotated by an oracle in semi-supervised setting and added to the training dataset in a single pool or, more often, in an iterative fashion. 
% The goal is to maximize prediction accuracy while minimizing the pool size and number of iterations.
% Active learning has been shown to require relatively fewer training instances when applied to computer vision tasks such as image classification~\cite{sener2017active,li2013adaptive,gal2017deep,beluch2018power} and semantic segmentation~\cite{yang2017suggestive,kuo2018cost,gorriz2017cost}.
% -------------------------------------------------------


% \textbf{(Traditional study has been only focused on limited applications, such as classification or detection. To the best of our knowledge, active learning on high-level tasks, such as VQA, has been rarely studied.)}


%2) Previous work on X has addressed these with Y, but the problems with this are Z.
More recently, AL has proven to be a potential solution~\cite{tong2001support} 
% to maximize learning while reducing the data annotation cost 
for vision~\&~language tasks 
% like Visual Question Answering (VQA)~\cite{misra2018learning} 
% \djkim{(Maybe not mentioning VQA? Or maybe change the expression? Reviewers might ask to compare)} 
like image captioning~\cite{shen2019learning} that rely extensively on large, expensive, curated datasets~\cite{antol2015vqa,gurari2018vizwiz,krishna2017visual,zhu2016visual7w}. 
Nonetheless, applying existing AL strategies to these tasks do not result in the performance increase when compared to random annotations~\cite{figueroa2012active,mairesse2010phrase,settles2008active}. 
A key difference in vision~\&~language tasks is the presence of \emph{multi-modal} inputs.
% For example, the VQA task requires a model to take an image and question pair as an input to predict an answer to the question based on the image~\cite{antol2015vqa}.
% VQA takes two inputs with different modalities.
Previous AL works such as~\cite{beluch2018power,gal2017deep,gorriz2017cost,kuo2018cost,li2013adaptive,sener2017active,yang2017suggestive, yoo2019learning} have focused more on single-modal inputs; hence, studies of AL with multi-modality is less prevalent. 
Since multi-modal tasks also suffer the same data issues, we find the pertinence of studying AL algorithms.
% for these tasks and see potential for our method to be a segue for other multi-modal tasks.
% such as multi-modal action recognition, audio-visual tasks, visual grounding, \emph{etc}. 
% -----

% too wordy... maybe not necessary and wordy -------------
% are founded on the assumption that the input of the model is only a single modality; hence, studies in active learning using multi-modality is comparably less prevalent than single modal applications.
% the scenario for the model that takes multi-modal inputs has been barely studied.
% However, in the real scenario, there are numerous tasks that takes multi-modal input, such as visual question answering~\cite{}, multi-modal action recognition~\cite{},
% C audio-visual tasks~\cite{}, \etc.
% ------------------------------

% and can make a prediction. 

% However, that also makes us wonder how informative the each modality is to the prediction as even though the model might receive both modalities as inputs, it can focus only on a single modality.



%3) In this work we do W. Thorough explanation.
In this work, we define a novel pool-based AL strategy to measure informativeness in AL for the Visual Question Answering (VQA) task
% for deep neural networks with multi-modal inputs 
in the form of \emph{mutual information} %(or statistical distance) 
as VQA takes in multi-modal inputs in the form of Image and Question. 
% In this regime, the model has the privilege of information from two different modalities;
In this regime, we tackle the question of informativeness of each modality in VQA models, {namely that of images and questions} as VQA models have been shown to be reliant on single modalities~\cite{agrawal2016analyzevqa,goyal2017making}.
To combat this, we leverage each modality separately using a multi-branch approach to evaluate the informativeness of each modality when sampling.
In this multi-branch model, the ``main'' branch relies on all present modalities and if a single-modal prediction $P(A|V)$ or $P(A|Q)$ is different from the ``main'' prediction $P(A|V,Q)$, it may signify that the missing modality is informative.
Hence we propose a method that we call Single-Modal Entropic Measure (SMEM). Our method selects instances for labeling from the unlabeled data pool based on the differences among the predictions from the single-modal and main predictions while our network also learns to minimize the differences between these predictions.
In effect, we propose an uncertainty sampling paradigm that relies on uncertainty measures instead of simple and naive single-modal entropy.
% Our key contribution is the novel AL uncertainty sampling paradigm that estimates uncertainty via uncertainty measure instead of simple and naive single modal entropy.
Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) and show the effectiveness of our strategy when compared to other existing AL approaches.
We demonstrate the efficacy of our approach in the VQA setting as it represents a challenging multi-modal task, but also believe that our solution is potentially extendable to any multi-modal task while being easy to implement.


% In this multi-branch model, the 'main' branch relies on all present modalities for its output while the remaining branches (number depending on how many modalities are present), relies solely on individual modalities. Or method selects instances for labeling from the unlabeled pool based on the distances of the single-modal output and the multi-modal output. 
% In this mutual information based system, our model selects instances for labeling based on distances of the single-model and multi-modal outputs as the model learns to minimize the distance for more effective sampling.

% Our approach is extremely simple to implement, and it consistently improves the performance.

% We propose new acquisition function for AL.
% It is based on mutual information between the single modal output and the multimodal output.
% If a single modal output is different from the multimodal output, it means the missing modality is important.



% We introduce a pool-based active learning strategy which learns a similarity (statistical distance) between single modal output and multimodal output using multi-branch model via self-distillation~\cite{}.
% Self-distillation technique has been recently introduced for effective image classification with multiple branch.
% We extend this idea to multi-modal learning scenario to help active learning.
% Our method selects instances for labeling from the unlabeled pool that that has high distance between singlemodal output and multimodal output, and the model learns to minimize the distance for more effective sampling.



% \textbf{(In this regard, we propose a novel sampling strategy for active learning on VQA. In addition, we adopt self distillation technique in order to effetely train a target model.)}

% Instead of simply computing the multi-modal entropy, we propose to compute the mutual information, which is the entropy difference between multi-modal output and single-modal outputs.
% We believe this allows the model to learn the discrepancy between the multi-modal input and the single-modal inputs as the mutual information constantly being minimized in the training stage, ultimately aiding in better and more robust sampling.\djkim{(Maybe redundant paragraph? Merge with previous paragraph?)}


% It allows the model to learn the discrepancy between multi-modal input and single modal input.

In addition, we introduce a novel self-distillation technique~\cite{phuong2019distillation,zhang2019your} to help with mutual information sampling by forcing the single-modal branches to generate outputs similar to that of the main branch. 
Self-distillation has been recently introduced for effective image classification~\cite{phuong2019distillation,zhang2019your} with multiple branches via regularization. 
We extend this idea to the multi-modal learning scenario to aid in AL with the motivation that if the discrepancy between the single- and multi-modal outputs is still large despite self-distillation, sampling that sample is highly likely to have large information gain.
We empirically show the significant performance gain of utilizing the self-distillation technique.

Through our experiments, we show the effectiveness of our uncertainty sampling strategy for VQA on the VQA v2.0~\cite{antol2015vqa} dataset.
% We observe that 
Our solution achieves favorable performance in VQA metrics~\cite{antol2015vqa} compared to existing sampling strategies~\cite{culotta2005reducing,scheffer2001active,shen2017deep}, while being cost-efficient.
In particular, the proposed method is able to decrease labeling efforts by about 40\% compared to prior methods.

Our main contributions are summarized as follows.
(1) We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task.
(2) In order to better train the Active Learning model, we extend the recently explored technique of self-distillation to show further performance gains on Active Learning.
(3) Through extensive experimentation, we show the effectiveness of our model on the VQA 2.0 dataset compared to various competing Active Learning methods.
%{\setdefaultleftmargin{3mm}{}{}{}{}{}
%\begin{enumerate}
%    \item We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task
%    \item In order to better train the Active Learning model, we extend the recently explored technique of self-distillation to show further performance gains on Active Learning
%    \item Through extensive experimentation, we show the effectiveness of our model on the VQA 2.0 dataset compared to various competing Active Learning methods
%\end{enumerate}
%}
\vspace{-2mm}

==> Legacy/unused_1_sec_intro_AAAI.tex <==
%1) X is an important problem and core challenges
%2) Previous work on X has addressed these with Y, but the problems with this are Z.
%3) In this work we do W. Thorough explanation.
%4) Contributions, and experiments


%1) X is an important problem and core challenges
% \textbf{(Recently, deep active Learning has been studied extensively. Active Learning is important to resolve data issues in various deep learning tasks.)}
Recent successes of learning-based computer vision methods rely heavily on abundant annotated training examples, which may be prohibitively costly to label or impossible to obtain at large scale~\cite{deng2009imagenet}. 
In order to mitigate this drawback, Active Learning (AL)~\cite{cohn1996active} has been introduced to minimize the number of expensive labels for the supervised training of deep neural networks by selecting (or \emph{sampling}) a subset of informative samples from a large unlabeled collection of data~\cite{settles2009active,tong2001support}.
AL has shown high classification performance with low labeling costs for computer vision tasks such as image classification~\cite{beluch2018power,gal2017deep,li2013adaptive,sener2017active, yoo2019learning} and semantic segmentation~\cite{gorriz2017cost,kuo2018cost}. 

% do we need to explain active learning? ----------------------
% Active learning algorithms aim to minimize the number of expensive labels for supervised training of deep neural networks (DNNs) by selecting a subset of informative examples from a large unlabeled collection of data~\cite{tong2001support,settles2009active}.
% The subset is annotated by an oracle in semi-supervised setting and added to the training dataset in a single pool or, more often, in an iterative fashion. 
% The goal is to maximize prediction accuracy while minimizing the pool size and number of iterations.
% Active learning has been shown to require relatively fewer training instances when applied to computer vision tasks such as image classification~\cite{sener2017active,li2013adaptive,gal2017deep,beluch2018power} and semantic segmentation~\cite{yang2017suggestive,kuo2018cost,gorriz2017cost}.
% -------------------------------------------------------


% \textbf{(Traditional study has been only focused on limited applications, such as classification or detection. To the best of our knowledge, active learning on high-level tasks, such as VQA, has been rarely studied.)}


%2) Previous work on X has addressed these with Y, but the problems with this are Z.
More recently, AL has been shown to be a potential solution~\cite{tong2001support} 
% to maximize learning while reducing the data annotation cost 
for vision~\&~language tasks 
% like Visual Question Answering (VQA)~\cite{misra2018learning} 
% \djkim{(Maybe not mentioning VQA? Or maybe change the expression? Reviewers might ask to compare)} 
like image captioning~\cite{shen2019learning} that rely extensively on large, expensive, curated datasets~\cite{antol2015vqa,gurari2018vizwiz,krishna2017visual,zhu2016visual7w}. 
Nonetheless, applying existing AL strategies to these tasks do not result in the performance increase when compared to random sampling
% annotations
~\cite{figueroa2012active,mairesse2010phrase,settles2008active}. 
A key difference in vision~\&~language tasks is the presence of \emph{multi-modal} inputs.
% For example, the VQA task requires a model to take an image and question pair as an input to predict an answer to the question based on the image~\cite{antol2015vqa}.
% VQA takes two inputs with different modalities.
Previous AL works 
% such as~\cite{beluch2018power,gal2017deep,gorriz2017cost,kuo2018cost,li2013adaptive,sener2017active,yang2017suggestive, yoo2019learning} 
have focused more on single-modal inputs; hence, studies of AL with multi-modality is less prevalent. 
Since multi-modal tasks also suffer the same data issues, we turn our focus to the Visual Question Answering (VQA) task as it provides a simple multi-modal input, single output classification framework.
% we find the pertinence of studying AL algorithms.

% \djkim{(Why not dealing other vision\&language tasks? we need to specify to VQA in this paragraph.)}
% for these tasks and see potential for our method to be a segue for other multi-modal tasks.
% such as multi-modal action recognition, audio-visual tasks, visual grounding, \emph{etc}. 
% -----

% too wordy... maybe not necessary and wordy -------------
% are founded on the assumption that the input of the model is only a single modality; hence, studies in active learning using multi-modality is comparably less prevalent than single modal applications.
% the scenario for the model that takes multi-modal inputs has been barely studied.
% However, in the real scenario, there are numerous tasks that takes multi-modal input, such as visual question answering~\cite{}, multi-modal action recognition~\cite{},
% C audio-visual tasks~\cite{}, \etc.
% ------------------------------

% and can make a prediction. 

% However, that also makes us wonder how informative the each modality is to the prediction as even though the model might receive both modalities as inputs, it can focus only on a single modality.


% \djkim{(Practicality of the scenario, image-question ``pair'' as unlabeled sample. It is realistic enough! For example, VizWiz, blind people can obtain both visual and question at the same time. )}

% \djkim{(tone down about the bias issue. Reviewers might ask about works about bias in VQA.)}


%3) In this work we do W. Thorough explanation.
In this work, we define a novel pool-based AL strategy to measure informativeness in AL for VQA
% for deep neural networks with multi-modal inputs 
in the form of \emph{mutual information} of the multiple inputs: %(or statistical distance) 
image and question.
% In this regime, the model has the privilege of information from two different modalities;
In this regime, we tackle the question of informativeness of each modality in VQA models
% {namely that of images and questions} 
as some studies have shown that VQA models are reliant on single modalities~\cite{goyal2017making,cadene2019rubi}.
To combat this, we leverage each modality separately using a multi-branch approach to evaluate the informativeness of each modality when sampling.
In this multi-branch model, the ``main'' branch relies on all present modalities and if a single-modal prediction $P(A|V)$ or $P(A|Q)$ is different from the ``main'' prediction $P(A|V,Q)$, it may signify that the missing modality is informative, where $A$, $V$, and $Q$ are the answer output, visual input, and question input respectively.

Hence we propose a method that we call Single-Modal Entropic Measure (SMEM). 
Our method selects instances for labeling from the unlabeled data pool based on the differences among the predictions from the single-modal and ``main'' predictions while our network also learns to minimize the differences between these predictions.
We show that we can take the differences among the predictions from the single-modal and ``main'' predictions into account by simply computing the \emph{entropy of the single-modal} predictions.
In effect, we propose an uncertainty sampling paradigm that enables simple inference without any ad hoc steps to measure uncertainty by relying on the multi-modal uncertainty instead of the simple and naive entropy of the main predictions.
% Our key contribution is the novel AL uncertainty sampling paradigm that estimates uncertainty via uncertainty measure instead of simple and naive single modal entropy.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
%~\jwcho{(wont they ask us to compare this if we add this?)}\djkim{(hmm... let's think about it)} and show the effectiveness of our strategy when compared to other existing AL approaches \jwcho{that do not include additional steps (like this? but more elegantly)}.
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
We demonstrate the efficacy of our approach on multiple VQA settings as VQA represents a challenging multi-modal task.
%, but also believe that our solution is potentially extendable to other multi-modal tasks while being easy to implement.
We also evaluate our method on another multi-modal task, action recognition, to show the generalizability of our approach while being easy to implement.


% In this multi-branch model, the 'main' branch relies on all present modalities for its output while the remaining branches (number depending on how many modalities are present), relies solely on individual modalities. Or method selects instances for labeling from the unlabeled pool based on the distances of the single-modal output and the multi-modal output. 
% In this mutual information based system, our model selects instances for labeling based on distances of the single-model and multi-modal outputs as the model learns to minimize the distance for more effective sampling.

% Our approach is extremely simple to implement, and it consistently improves the performance.

% We propose new acquisition function for AL.
% It is based on mutual information between the single modal output and the multimodal output.
% If a single modal output is different from the multimodal output, it means the missing modality is important.



% We introduce a pool-based active learning strategy which learns a similarity (statistical distance) between single modal output and multimodal output using multi-branch model via self-distillation~\cite{}.
% Self-distillation technique has been recently introduced for effective image classification with multiple branch.
% We extend this idea to multi-modal learning scenario to help active learning.
% Our method selects instances for labeling from the unlabeled pool that that has high distance between singlemodal output and multimodal output, and the model learns to minimize the distance for more effective sampling.



% \textbf{(In this regard, we propose a novel sampling strategy for active learning on VQA. In addition, we adopt self distillation technique in order to effetely train a target model.)}

% Instead of simply computing the multi-modal entropy, we propose to compute the mutual information, which is the entropy difference between multi-modal output and single-modal outputs.
% We believe this allows the model to learn the discrepancy between the multi-modal input and the single-modal inputs as the mutual information constantly being minimized in the training stage, ultimately aiding in better and more robust sampling.\djkim{(Maybe redundant paragraph? Merge with previous paragraph?)}


% It allows the model to learn the discrepancy between multi-modal input and single modal input.

In addition, we introduce a novel self-distillation technique~\cite{phuong2019distillation,zhang2019your} to help with mutual information sampling by forcing the single-modal branches to generate outputs similar to that of the ``main'' branch. 
Self-distillation has been recently introduced for effective image classification~\cite{phuong2019distillation,zhang2019your} with multiple branches via regularization. \djkim{(we don't use it as a regularizer!)}
We extend this idea to the multi-modal learning scenario to aid in AL with the motivation that if the discrepancy between the single- and multi-modal outputs is still large despite self-distillation, sampling that sample is highly likely to have large information gain.
We empirically show the significant performance gain of utilizing the self-distillation technique.

Through our experimentation, we show the effectiveness of our uncertainty sampling strategy on multiple VQA datasets including VQA v2.0~\cite{antol2015vqa}, VizWiz VQA~\cite{gurari2018vizwiz}, and VQA-CP2~\cite{goyal2017making}.
In addition, although we design our model with multi-modal inputs in mind (\emph{e.g.}, vision-language tasks), we also evaluate our model on NTU RGB+D dataset~\cite{shahroudy2016ntu} in order to show the extensibility of our approach.
% We observe that 
Our solution achieves favorable performance in VQA metrics~\cite{antol2015vqa} compared to existing sampling strategies~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning}, while being cost-efficient.
In particular, the proposed method is able to decrease labeling efforts by about 30\%.
% compared to prior methods.

Our main contributions are summarized as follows.
(1) We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task.
(2) 
% \jsc{In order to better train}
For a more effective training of the 
% Active Learning 
single-modal branches for Active Learning,
% \jwcho{(actually we are not training the ``active learning''  model, and this might be a little bit misleading, causing people to question our architectural advantages...)}, 
% \jsc{we extend the recently explored technique of}
we employ self-distillation between the main branch and ad hoc single-modal branches.
% to show further performance gains on Active Learning.
\djkim{(we should tone down contribution2. Might be confused that we firstly use self-distillation. ``novel usage of self-distillation?'')}
(3) Through extensive experimentation, we show the effectiveness of our model on 
%the VQA v2.0 dataset 
multiple VQA datasets
compared to various competing Active Learning methods.
%{\setdefaultleftmargin{3mm}{}{}{}{}{}
%\begin{enumerate}
%    \item We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task
%    \item In order to better train the Active Learning model, we extend the recently explored technique of self-distillation to show further performance gains on Active Learning
%    \item Through extensive experimentation, we show the effectiveness of our model on the VQA v2.0 dataset compared to various competing Active Learning methods
%\end{enumerate}
%}
\vspace{-2mm}

==> Legacy/unused_1_sec_intro_ICML.tex <==
%1) X is an important problem and core challenges
%2) Previous work on X has addressed these with Y, but the problems with this are Z.
%3) In this work we do W. Thorough explanation.
%4) Contributions, and experiments


%1) X is an important problem and core challenges
% \textbf{(Recently, deep active Learning has been studied extensively. Active Learning is important to resolve data issues in various deep learning tasks.)}
Recent successes of learning-based computer vision methods rely heavily on abundant annotated training examples, which may be prohibitively costly to label or impossible to obtain at large scale~\cite{deng2009imagenet}. 
In order 
to mitigate this drawback, Active Learning (AL)~\cite{cohn1996active} has been introduced to minimize the number of expensive labels for the supervised training of deep neural networks by selecting (or \emph{sampling}) a subset of informative samples from a large unlabeled collection of data~\cite{settles2009active,tong2001support}.
AL has shown high classification performance with low labeling costs for computer vision tasks such as image classification~\cite{sener2017active, yoo2019learning, sinha2019variational} and semantic segmentation~\cite{gorriz2017cost,kuo2018cost}. 


%2) Previous work on X has addressed these with Y, but the problems with this are Z.
More recently, AL has been shown to be a potential solution~\cite{tong2001support} 
% to maximize learning while reducing the data annotation cost 
for vision~\&~language tasks 
% like Visual Question Answering (VQA)~\cite{misra2018learning} 
like image captioning~\cite{shen2019learning} that rely extensively on large, expensive, curated datasets~\cite{antol2015vqa,gurari2018vizwiz,krishna2017visual,zhu2016visual7w}. 
Nonetheless, applying existing AL strategies to these tasks do not result in the performance increase {even} when compared to random sampling
% annotations
~\cite{figueroa2012active,mairesse2010phrase,settles2008active}. 
A key distinction in
vision~\&~language tasks is the presence of \emph{multi-modal} inputs.
% For example, the VQA task requires a model to take an image and question pair as an input to predict an answer to the question based on the image~\cite{antol2015vqa}.
% VQA takes two inputs with different modalities.
Previous AL works 
% such as~\cite{beluch2018power,gal2017deep,gorriz2017cost,kuo2018cost,li2013adaptive,sener2017active,yang2017suggestive, yoo2019learning} 
have focused more on single-modal inputs; hence, studies of AL with multi-modality is less prevalent. 
Since multi-modal tasks also suffer the same data issues, we turn our focus to the Visual Question Answering (VQA) task as it provides a simple multi-modal input, single output classification framework.
% we find the pertinence of studying AL algorithms.

% \djkim{(Why not dealing other vision\&language tasks? we need to specify to VQA in this paragraph.)}
% for these tasks and see potential for our method to be a segue for other multi-modal tasks.
% such as multi-modal action recognition, audio-visual tasks, visual grounding, \emph{etc}. 
% -----

% too wordy... maybe not necessary and wordy -------------
% are founded on the assumption that the input of the model is only a single modality; hence, studies in active learning using multi-modality is comparably less prevalent than single modal applications.
% the scenario for the model that takes multi-modal inputs has been barely studied.
% However, in the real scenario, there are numerous tasks that takes multi-modal input, such as visual question answering~\cite{}, multi-modal action recognition~\cite{},
% C audio-visual tasks~\cite{}, \etc.
% ------------------------------

% and can make a prediction. 

% However, that also makes us wonder how informative the each modality is to the prediction as even though the model might receive both modalities as inputs, it can focus only on a single modality.




%3) In this work we do W. Thorough explanation.
In this work, we define a novel pool-based AL strategy to measure informativeness in AL for VQA
% for deep neural networks with multi-modal inputs 
in the form of \emph{mutual information} of the multiple inputs: %(or statistical distance) 
image and question.
% In this regime, the model has the privilege of information from two different modalities;
In this regime, we tackle the question of informativeness of each modality in VQA models
% {namely that of images and questions} 
as some studies have shown that VQA models are reliant on single modalities~\cite{goyal2017making,cadene2019rubi}.
To combat this, we leverage each modality separately using a multi-branch approach to evaluate the informativeness of each modality when sampling.
In this multi-branch model, the ``main'' branch relies on all present modalities and if a single-modal prediction $P(A|V)$ or $P(A|Q)$ is different from the ``main'' prediction $P(A|V,Q)$, it may signify that the missing modality is informative, where $A$, $V$, and $Q$ are the answer output, visual input, and question input respectively.





Hence we propose a method that we call Single-Modal Entropic Measure (SMEM). 
Our method selects instances for labeling from the unlabeled data pool based on the differences among the predictions from the single-modal and ``main'' predictions while the single-modal branch also learns to minimize the difference of the prediction with the ``main'' branch.
We show that we can take the differences among the predictions from the single-modal and ``main'' predictions into account by simply computing the \emph{entropy of the single-modal} predictions.
In effect, we propose an uncertainty based sampling paradigm that enables simple inference without any ad hoc steps to measure uncertainty by relying on the multi-modal uncertainty instead of the simple and naive entropy of the main predictions.
% Our key contribution is the novel AL uncertainty sampling paradigm that estimates uncertainty via uncertainty measure instead of simple and naive single modal entropy.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
%~\jwcho{(wont they ask us to compare this if we add this?)}\djkim{(hmm... let's think about it)} and show the effectiveness of our strategy when compared to other existing AL approaches \jwcho{that do not include additional steps (like this? but more elegantly)}.
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
%%%%
% \jwcho{(this is repeated in the next next paragraph)}
% We demonstrate the efficacy of our approach on multiple VQA settings as VQA represents a challenging multi-modal task.
% %, but also believe that our solution is potentially extendable to other multi-modal tasks while being easy to implement.
% We also evaluate our method on another multi-modal task, action recognition, to show the generalizability of our approach while being easy to implement.
%%%%%


% In this multi-branch model, the 'main' branch relies on all present modalities for its output while the remaining branches (number depending on how many modalities are present), relies solely on individual modalities. Or method selects instances for labeling from the unlabeled pool based on the distances of the single-modal output and the multi-modal output. 
% In this mutual information based system, our model selects instances for labeling based on distances of the single-model and multi-modal outputs as the model learns to minimize the distance for more effective sampling.

% Our approach is extremely simple to implement, and it consistently improves the performance.

% We propose new acquisition function for AL.
% It is based on mutual information between the single modal output and the multimodal output.
% If a single modal output is different from the multimodal output, it means the missing modality is important.



% We introduce a pool-based active learning strategy which learns a similarity (statistical distance) between single modal output and multimodal output using multi-branch model via self-distillation~\cite{}.
% Self-distillation technique has been recently introduced for effective image classification with multiple branch.
% We extend this idea to multi-modal learning scenario to help active learning.
% Our method selects instances for labeling from the unlabeled pool that that has high distance between singlemodal output and multimodal output, and the model learns to minimize the distance for more effective sampling.



% \textbf{(In this regard, we propose a novel sampling strategy for active learning on VQA. In addition, we adopt self distillation technique in order to effetely train a target model.)}

% Instead of simply computing the multi-modal entropy, we propose to compute the mutual information, which is the entropy difference between multi-modal output and single-modal outputs.
% We believe this allows the model to learn the discrepancy between the multi-modal input and the single-modal inputs as the mutual information constantly being minimized in the training stage, ultimately aiding in better and more robust sampling.\djkim{(Maybe redundant paragraph? Merge with previous paragraph?)}


% It allows the model to learn the discrepancy between multi-modal input and single modal input.

In addition, we utilize a self-distillation technique to directly aid in mutual information sampling by forcing the single modal branches to generate outputs similar to that of the ``main'' branch.
% with mutual information sampling by forcing the single-modal branches to generate outputs similar to that of the ``main'' branch. 
Self-distillation has been recently introduced for effective image classification~\cite{phuong2019distillation,zhang2019your} with multiple branches as a regularization.
We extend this idea to the multi-modal learning scenario, \emph{not as a regularizer} for the model, but to aid in AL with the motivation that if the discrepancy between the single- and multi-modal outputs is still large despite self-distillation, sampling that sample is highly likely to have large information gain.
We empirically show the significant performance gain of utilizing the self-distillation technique.

Through our experimentation, we show the effectiveness of our sample acquisition method on multiple VQA datasets including VQA v2.0~\cite{antol2015vqa}, VizWiz VQA~\cite{gurari2018vizwiz}, and VQA-CP2~\cite{goyal2017making}.
In addition, although we design our model with multi-modal inputs in mind (\emph{e.g.}, vision-language tasks), we also evaluate our model on NTU RGB+D dataset~\cite{shahroudy2016ntu} in order to show the extensibility of our approach.
% We observe that 
Our solution achieves favorable performance in VQA metrics~\cite{antol2015vqa} compared to existing sampling strategies~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning,sinha2019variational,zhang2020state}, while being cost-efficient.
In particular, the proposed method is able to decrease labeling efforts by about 30\%.
% compared to prior methods.

Our main contributions are summarized as follows.
(1) {We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task.}
(2) {
% \jsc{In order to better train}
To better sample from the single-modal branches for Active Learning,
% For a more effective training of the 
% Active Learning 
% single-modal branches for Active Learning,
% \jwcho{(actually we are not training the ``active learning''  model, and this might be a little bit misleading, causing people to question our architectural advantages...)}, 
% \jsc{we extend the recently explored technique of}
we employ self-distillation between the main branch and ad hoc single-modal branches to better train the {auxiliary} single-modal branches.}
% to show further performance gains on Active Learning.
% \djkim{(we should tone down contribution2. Might be confused that we firstly use self-distillation. ``novel usage of self-distillation?'')}
(3) {Through extensive experimentation, we show the effectiveness of our model on
%the VQA v2.0 dataset 
multiple VQA datasets
compared to various competing Active Learning methods.}
(4) {We show that our method is task and architecture agnostic by testing our method on the NTU RGB+D action recognition task~\cite{shahroudy2016ntu}.}
To the best of our knowledge, we are the first to create an Active Learning framework specifically tailored for the multi-modal task of VQA.
%{\setdefaultleftmargin{3mm}{}{}{}{}{}
%\begin{enumerate}
%    \item We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task
%    \item In order to better train the Active Learning model, we extend the recently explored technique of self-distillation to show further performance gains on Active Learning
%    \item Through extensive experimentation, we show the effectiveness of our model on the VQA v2.0 dataset compared to various competing Active Learning methods
%\end{enumerate}
%}


==> Legacy/unused_1_sec_intro_humantech.tex <==
%1) X is an important problem and core challenges
%2) Previous work on X has addressed these with Y, but the problems with this are Z.
%3) In this work we do W. Thorough explanation.
%4) Contributions, and experiments


%1) X is an important problem and core challenges
% \textbf{(Recently, deep active Learning has been studied extensively. Active Learning is important to resolve data issues in various deep learning tasks.)}
Recent successes of learning-based computer vision methods rely heavily on abundant annotated training examples, which may be prohibitively costly to label or impossible to obtain at large scale~\cite{deng2009imagenet}. 
In order 
to mitigate this drawback, Active Learning (AL)~\cite{cohn1996active} has been introduced to minimize the number of expensive labels for the supervised training of deep neural networks by selecting (or \emph{sampling}) a subset of informative samples from a large unlabeled collection of data~\cite{settles2009active,tong2001support}.
AL has shown high classification performance with low labeling costs for computer vision tasks such as image classification~\cite{beluch2018power,gal2017deep,li2013adaptive,sener2017active, yoo2019learning} and semantic segmentation~\cite{gorriz2017cost,kuo2018cost}. 

% do we need to explain active learning? ----------------------
% Active learning algorithms aim to minimize the number of expensive labels for supervised training of deep neural networks (DNNs) by selecting a subset of informative examples from a large unlabeled collection of data~\cite{tong2001support,settles2009active}.
% The subset is annotated by an oracle in semi-supervised setting and added to the training dataset in a single pool or, more often, in an iterative fashion. 
% The goal is to maximize prediction accuracy while minimizing the pool size and number of iterations.
% Active learning has been shown to require relatively fewer training instances when applied to computer vision tasks such as image classification~\cite{sener2017active,li2013adaptive,gal2017deep,beluch2018power} and semantic segmentation~\cite{yang2017suggestive,kuo2018cost,gorriz2017cost}.
% -------------------------------------------------------


% \textbf{(Traditional study has been only focused on limited applications, such as classification or detection. To the best of our knowledge, active learning on high-level tasks, such as VQA, has been rarely studied.)}


%2) Previous work on X has addressed these with Y, but the problems with this are Z.
More recently, AL has been shown to be a potential solution~\cite{tong2001support} 
% to maximize learning while reducing the data annotation cost 
for vision~\&~language tasks 
% like Visual Question Answering (VQA)~\cite{misra2018learning} 
% \djkim{(Maybe not mentioning VQA? Or maybe change the expression? Reviewers might ask to compare)} 
like image captioning~\cite{shen2019learning} that rely extensively on large, expensive, curated datasets~\cite{antol2015vqa,gurari2018vizwiz,krishna2017visual,zhu2016visual7w}. 
Nonetheless, applying existing AL strategies to these tasks do not result in the performance increase when compared to random sampling
% annotations
~\cite{figueroa2012active,mairesse2010phrase,settles2008active}. 
A key difference in vision~\&~language tasks is the presence of \emph{multi-modal} inputs.
% For example, the VQA task requires a model to take an image and question pair as an input to predict an answer to the question based on the image~\cite{antol2015vqa}.
% VQA takes two inputs with different modalities.
Previous AL works 
% such as~\cite{beluch2018power,gal2017deep,gorriz2017cost,kuo2018cost,li2013adaptive,sener2017active,yang2017suggestive, yoo2019learning} 
have focused more on single-modal inputs; hence, studies of AL with multi-modality is less prevalent. 
Since multi-modal tasks also suffer the same data issues, we turn our focus to the Visual Question Answering (VQA) task as it provides a simple multi-modal input, single output classification framework.
% we find the pertinence of studying AL algorithms.

% \djkim{(Why not dealing other vision\&language tasks? we need to specify to VQA in this paragraph.)}
% for these tasks and see potential for our method to be a segue for other multi-modal tasks.
% such as multi-modal action recognition, audio-visual tasks, visual grounding, \emph{etc}. 
% -----

% too wordy... maybe not necessary and wordy -------------
% are founded on the assumption that the input of the model is only a single modality; hence, studies in active learning using multi-modality is comparably less prevalent than single modal applications.
% the scenario for the model that takes multi-modal inputs has been barely studied.
% However, in the real scenario, there are numerous tasks that takes multi-modal input, such as visual question answering~\cite{}, multi-modal action recognition~\cite{},
% C audio-visual tasks~\cite{}, \etc.
% ------------------------------

% and can make a prediction. 

% However, that also makes us wonder how informative the each modality is to the prediction as even though the model might receive both modalities as inputs, it can focus only on a single modality.


% \djkim{(Practicality of the scenario, image-question ``pair'' as unlabeled sample. It is realistic enough! For example, VizWiz, blind people can obtain both visual and question at the same time. )}

% \djkim{(tone down about the bias issue. Reviewers might ask about works about bias in VQA.)}
\begin{figure}[t]
\centering
\vspace{-2mm}
%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_final}}
{\includegraphics[width=1\linewidth,keepaspectratio]{Figures/quantitative_VQA_new}}
%}
%\vspace{-2mm}
\caption{Comparison with existing approaches on the VQA v2.0 dataset. Reference is the best performance of the existing methods.
Our model shows the best performance among all the other methods by a large margin. Full dataset training shows 63.52\% accuracy, while ours at \emph{stage 10} shows 63.31\% accuracy.}
\vspace{-2mm}
\label{fig:quantitative}
\end{figure}

%3) In this work we do W. Thorough explanation.
In this work, we define a novel pool-based AL strategy to measure informativeness in AL for VQA
% for deep neural networks with multi-modal inputs 
in the form of \emph{mutual information} of the multiple inputs: %(or statistical distance) 
image and question.
% In this regime, the model has the privilege of information from two different modalities;
In this regime, we tackle the question of informativeness of each modality in VQA models
% {namely that of images and questions} 
as some studies have shown that VQA models are reliant on single modalities~\cite{goyal2017making,cadene2019rubi}.
To combat this, we leverage each modality separately using a multi-branch approach to evaluate the informativeness of each modality when sampling.
In this multi-branch model, the ``main'' branch relies on all present modalities and if a single-modal prediction $P(A|V)$ or $P(A|Q)$ is different from the ``main'' prediction $P(A|V,Q)$, it may signify that the missing modality is informative, where $A$, $V$, and $Q$ are the answer output, visual input, and question input respectively.


\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=0.9\linewidth,keepaspectratio]{Figures/architecture}
    % \vspace{-2mm}
    \caption{Illustration of our model architecture. Our model can be applied to any off-the-shelf VQA models (hence the area in green shows a generic VQA architecture) as our goal is to design ad hoc branches solely for the purpose of \emph{measuring uncertainty}. We add two auxiliary branches $g_v(\cdot)$ and $g_q(\cdot)$ that process the visual or question features exclusively to generate answers from a single modality. Along with the cross-entropy loss from ground truth answers, the single-modal branches are trained with knowledge distillation loss to follow the output from the multi-modal branch $g(\cdot)$.
    % original multi-modal answer prediction branch.
    In particular, $F(\cdot,\cdot)$ components (in black) are trained with \Eref{eqn:loss_main} while $g_v(\cdot)$ and $g_q(\cdot)$ (in red) are trained with \Eref{eqn:loss_v} and \Eref{eqn:loss_q} respectively. \
    % djkim{(Our model can be applied to any off-the-shelf VQA models. Our work is about designing good ad hoc branches to measure (only measure) the uncertainty.)(VQA architecture itself is not a concern in our work. The goal is to make a favorable \emph{uncertainty measure} and the auxiliary branches are only for the uncertainty measure! The branches don't affect the model training.)}
    }
    \vspace{-2mm}
    \label{fig:architecture}
\end{figure*}


Hence we propose a method that we call Single-Modal Entropic Measure (SMEM). 
Our method selects instances for labeling from the unlabeled data pool based on the differences among the predictions from the single-modal and ``main'' predictions while our network also learns to minimize the differences between these predictions.
We show that we can take the differences among the predictions from the single-modal and ``main'' predictions into account by simply computing the \emph{entropy of the single-modal} predictions.
In effect, we propose an uncertainty based sampling paradigm that enables simple inference without any ad hoc steps to measure uncertainty by relying on the multi-modal uncertainty instead of the simple and naive entropy of the main predictions.
% Our key contribution is the novel AL uncertainty sampling paradigm that estimates uncertainty via uncertainty measure instead of simple and naive single modal entropy.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
%~\jwcho{(wont they ask us to compare this if we add this?)}\djkim{(hmm... let's think about it)} and show the effectiveness of our strategy when compared to other existing AL approaches \jwcho{that do not include additional steps (like this? but more elegantly)}.
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
We demonstrate the efficacy of our approach on multiple VQA settings as VQA represents a challenging multi-modal task.
%, but also believe that our solution is potentially extendable to other multi-modal tasks while being easy to implement.
We also evaluate our method on another multi-modal task, action recognition, to show the generalizability of our approach while being easy to implement.



% In this multi-branch model, the 'main' branch relies on all present modalities for its output while the remaining branches (number depending on how many modalities are present), relies solely on individual modalities. Or method selects instances for labeling from the unlabeled pool based on the distances of the single-modal output and the multi-modal output. 
% In this mutual information based system, our model selects instances for labeling based on distances of the single-model and multi-modal outputs as the model learns to minimize the distance for more effective sampling.

% Our approach is extremely simple to implement, and it consistently improves the performance.

% We propose new acquisition function for AL.
% It is based on mutual information between the single modal output and the multimodal output.
% If a single modal output is different from the multimodal output, it means the missing modality is important.



% We introduce a pool-based active learning strategy which learns a similarity (statistical distance) between single modal output and multimodal output using multi-branch model via self-distillation~\cite{}.
% Self-distillation technique has been recently introduced for effective image classification with multiple branch.
% We extend this idea to multi-modal learning scenario to help active learning.
% Our method selects instances for labeling from the unlabeled pool that that has high distance between singlemodal output and multimodal output, and the model learns to minimize the distance for more effective sampling.



% \textbf{(In this regard, we propose a novel sampling strategy for active learning on VQA. In addition, we adopt self distillation technique in order to effetely train a target model.)}

% Instead of simply computing the multi-modal entropy, we propose to compute the mutual information, which is the entropy difference between multi-modal output and single-modal outputs.
% We believe this allows the model to learn the discrepancy between the multi-modal input and the single-modal inputs as the mutual information constantly being minimized in the training stage, ultimately aiding in better and more robust sampling.\djkim{(Maybe redundant paragraph? Merge with previous paragraph?)}


% It allows the model to learn the discrepancy between multi-modal input and single modal input.

In addition, we introduce a novel self-distillation technique~\cite{phuong2019distillation,zhang2019your} to help with mutual information sampling by forcing the single-modal branches to generate outputs similar to that of the ``main'' branch. 
Self-distillation has been recently introduced for effective image classification~\cite{phuong2019distillation,zhang2019your} with multiple branches via regularization.
We extend this idea to the multi-modal learning scenario, not as a regularizer, but to aid in AL with the motivation that if the discrepancy between the single- and multi-modal outputs is still large despite self-distillation, sampling that sample is highly likely to have large information gain.
We empirically show the significant performance gain of utilizing the self-distillation technique.

Through our experimentation, we show the effectiveness of our uncertainty sampling strategy on multiple VQA datasets including VQA v2.0~\cite{antol2015vqa}, VizWiz VQA~\cite{gurari2018vizwiz}, and VQA-CP2~\cite{goyal2017making}.
In addition, although we design our model with multi-modal inputs in mind (\emph{e.g.}, vision-language tasks), we also evaluate our model on NTU RGB+D dataset~\cite{shahroudy2016ntu} in order to show the extensibility of our approach.
% We observe that 
Our solution achieves favorable performance in VQA metrics~\cite{antol2015vqa} compared to existing sampling strategies~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning}, while being cost-efficient.
In particular, the proposed method is able to decrease labeling efforts by about 30\%.
% compared to prior methods.

Our main contributions are summarized as follows.
\setdefaultleftmargin{3mm}{}{}{}{}{}
\begin{itemize}
\item{We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task.}
\item{
% \jsc{In order to better train}
To better sample from the single-modal branches for Active Learning,
% For a more effective training of the 
% Active Learning 
% single-modal branches for Active Learning,
% \jwcho{(actually we are not training the ``active learning''  model, and this might be a little bit misleading, causing people to question our architectural advantages...)}, 
% \jsc{we extend the recently explored technique of}
we employ self-distillation between the main branch and ad hoc single-modal branches to better train the single-modal branches.}
% to show further performance gains on Active Learning.
% \djkim{(we should tone down contribution2. Might be confused that we firstly use self-distillation. ``novel usage of self-distillation?'')}
\item{Through extensive experimentation, we show the effectiveness of our model on
%the VQA v2.0 dataset 
multiple VQA datasets
compared to various competing Active Learning methods.}
\item{We show that our method is task and architecture agnostic by testing our method on the NTU RGB+D action recognition task~\cite{shahroudy2016ntu}.}
%{\setdefaultleftmargin{3mm}{}{}{}{}{}
%\begin{enumerate}
%    \item We propose a novel sampling criteria, that we call Single-Modal Entropic Measure (SMEM), based on mutual information for Active Learning for the Visual Question Answering task
%    \item In order to better train the Active Learning model, we extend the recently explored technique of self-distillation to show further performance gains on Active Learning
%    \item Through extensive experimentation, we show the effectiveness of our model on the VQA v2.0 dataset compared to various competing Active Learning methods
%\end{enumerate}
%}
\end{itemize}
\vspace{-2mm}

==> Legacy/unused_2_sec_related.tex <==

We explore the field of Active Learning (AL) and comment on how existing uncertainty measurements fail in environments of multi-modality.
% where we have multiple correct outputs. 
We place our work in context of VQA, as we believe it is highly representative manifestation of these environments. 
% Next, we dive into visual-semantic embedding, a practical solution to construct semantic spaces using
% visual priors. 
% Finally, we explore Bayesian uncertainty measurement techniques.

\noindent\textbf{Active Learning.} 
A typical AL setting starts with a small initial set of labeled data $\mathcal{D}\textsubscript{L}$ and a large set of unlabeled data $\mathcal{D}\textsubscript{U}$. 
Knowing that labeling data is costly and time consuming, the task is to minimize the number of samples to annotate from $\mathcal{D}\textsubscript{U}$ while maximizing performance on a given task~\cite{tong2001support}. 
AL strategies have been successfully applied to a wide number of machine learning tasks, including image recognition~\cite{joshi2009multi,sener2017active}, information extraction~\cite{culotta2005reducing,jones2003active,scheffer2001active}, and text categorization~\cite{hoi2006batch,lewis1994sequential}, with strategies including uncertainty-based sampling~\cite{collins2008towards,joshi2009multi} and information gain~\cite{houlsby2011bayesian}.
Others have introduced a theoretical dropout-based framework to measure uncertainty~\cite{gal2017deep,kendall2017uncertainties}.
Similar solutions have been adapted to NLP tasks such as Named Entity Recognition~\cite{shen2017deep} and Neural Semantic Parsing by adding Gaussian noise to network weights~\cite{dong2018confidence}. 
%In this paper, we empirically show how previous uncertainty sampling strategies do not perform better than random sampling in a VQA setting and propose a novel strategy that uses Bayesian uncertainty in a semantically structured embedding space.
Recently, AL has been explored in vision~\&~language tasks with varying degrees of success~\cite{chi2019justasknavigation,lin2017activelearningvqa,misra2018learning,shen2019learning}.


\noindent\textbf{Visual Question Answering.}
VQA systems expect an input image and a natural language question pair and attempt to output a correct answer~\cite{antol2015vqa}, and the system has received a considerable amount of attention in recent years with the development of several datasets proposed as benchmarks~\cite{antol2015vqa,goyal2017making,johnson2017clevr,krishna2017visual,malinowski2015ask,ren2015exploring,zhu2016visual7w} and of various models\cite{antol2015vqa,fukui2016multimodal,jabri2016revisiting,lu2016hierarchical,malinowski2015ask,wu2016ask,yang2016stacked,zhu2016visual7w}. 
To tackle the task, many have proposed architectures that encode and then merge the visual and textual information in order to classify the answers~\cite{jabri2016revisiting,ma2016learning,malinowski2015ask}.
Attention mechanisms have proven to be successful in this task~\cite{anderson2018bottom,lu2016hierarchical,shih2016look,xu2016ask}, and other works have focused on designing effective multi-modal feature fusion schemes~\cite{ben2017mutan,fukui2016multimodal,kim2017hadamard}. 
While the progress has been encouraging, such approaches require a large amount of labeled data.
% with a predefined, mutually exclusive set of answer categories. 
VQA models have also been shown to rely on priors and dataset biases~\cite{agrawal2016analyzevqa,agrawal2018don,cadene2019rubi,goyal2017making,jabri2016revisiting,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, and in the AL setting, we intend to exploit this trait.




% We explore a more realistic variant of VQA where models generate natural language answers, resulting in the generation of paraphrases.

%\noindent\textbf{Semantically structured embeddings.}
%Our key insight lies in moving uncertainty estimation from the model’s output space to a semantically structured internal embedding space. 
%Since we specifically study vision-language tasks, we build a visual-semantic space that combines both visual and textual information in order to create a unified latent representation. 
%This problem has been studied extensively in the last few years with work that involves jointly embedding images and text, at the word level~\cite{frome2013devise,kong2014you,joulin2016learning,matuszek2012joint,klein2015associating}, and sentence level~\cite{zitnick2013learning,karpathy2015deep,karpathy2014deep,chen2015mind,kiros2014unifying,reed2016learning}. 
%Visually grounded text representations have been applied to different tasks, including caption generation~\cite{kiros2014unifying,karpathy2015deep}, image retrieval~\cite{lin2014visual}, and visual question answering~\cite{malinowski2015ask}. 
%%Our approach is inspired by previous work~\cite{karpathy2014deep}, where we use image regions with their associated captions and adapt a margin objective to build the semantic space. 
%%We use the semantic space to enable a new active learning strategy.


%\noindent\textbf{Uncertainty.}
%As uncertainty estimation represents the most popular sampling strategy for active learning, we explore uncertainty estimation techniques developed for deep learning models. 
%Even though Deep Learning systems are performant, they remain uninterpretable, poor at quantifying predictive uncertainty, and overconfident in their predictions. 
%To mitigate this problem, Bayesian models have been proposed by placing a prior distribution over model weights [70, 53, 47]. 
%Yet, even though the problem is simple to formulate, deriving a posterior distribution for Deep Bayesian Neural Networks (BNN) is intractable which makes Bayesian inference difficult [18]. 
%Therefore, focus has shifted to approximating BNNs with variational inference. 
%Bayesian modeling of stochastic processes introduced new techniques into the field such as sampling-based and stochastic variational inference [6, 7]. 
%On the other hand, Monte-Carlo Dropout [19, 18] has empirically demonstrated comparable uncertainty estimation quality to variational inference [19]. 
%A model trained with dropout can be used as a Bayesian model by making multiple predictions while sampling different dropout masks for each forward propagation. 
%Estimating the posterior amounts to computing the mean and variance of the predictions. 
%While previous work has showed promise in classification and regression tasks [74, 18, 60], such methods have not been extended to language generation.
%In fact, most language-based uncertainty work adapts classification-based uncertainty techniques to language tasks, transforming the problem from an open language problem to a constrained closed problem [64, 22, 40, 24, 13]. 
%We propose a new sampling strategy that extends Monte-Carlo dropout uncertainty [18] to measure uncertainty in a semantic space.



%\noindent\textbf{Mutual Information in Deep Neural Networks.}
%asdfadf

==> Legacy/unused_2_sec_related_AAAI.tex <==

We explore the field of Active Learning (AL) 
% and comment on how existing uncertainty measurements fail 
in the environment of multi-modality
% where we have multiple correct outputs. 
and place our work in the context of VQA, as we believe it is a highly representative manifestation of this environment. 
% Next, we dive into visual-semantic embedding, a practical solution to construct semantic spaces using
% visual priors. 
% Finally, we explore Bayesian uncertainty measurement techniques.

\noindent\textbf{Active Learning.} 
% \djkim{(We should put more recent AL papers \cite{sinha2019variational,zhang2020state} somewhere)}
A typical AL setting starts with a small initial set of labeled data $\mathcal{D}\textsubscript{L}$ and a large set of unlabeled data $\mathcal{D}\textsubscript{U}$. 
Knowing that labeling data is costly and time consuming, the task is to minimize the number of samples to annotate from $\mathcal{D}\textsubscript{U}$ while maximizing performance on a given task~\cite{tong2001support}. 
AL strategies have been successfully applied to a wide number of machine learning tasks, including image recognition~\cite{joshi2009multi,sener2017active,yoo2019learning}, information extraction~\cite{culotta2005reducing,jones2003active,scheffer2001active}, and text categorization~\cite{hoi2006batch,lewis1994sequential}, with strategies including uncertainty-based sampling~\cite{collins2008towards,joshi2009multi} and information gain~\cite{houlsby2011bayesian}.
While others have introduced a theoretical dropout-based framework to measure uncertainty~\cite{gal2017deep,kendall2017uncertainties}, more recent works have leveraged latent space representations with the help of variational autoencoders and adversarial training for improved sampling~\cite{sinha2019variational,zhang2020state,shuo2020daal}.
However, we chose not to compare our method to these approaches as they require additional elaborately designed large networks to learn latent representation which have limited scalability to multi-modal tasks.%; thus we do not compare our method with these methods.
We also do not compare to methods that require multiple steps such as Monte-Carlo dropout or model ensemble (Query-by-Committee) %as we \js{(???)}
as they are hard to apply to recent large models for higher-level tasks.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
% Similar solutions have been adapted to NLP tasks such as named entity recognition~\cite{shen2017deep} and neural semantic parsing by adding Gaussian noise to network weights~\cite{dong2018confidence}. 
%In this paper, we empirically show how previous uncertainty sampling strategies do not perform better than random sampling in a VQA setting and propose a novel strategy that uses Bayesian uncertainty in a semantically structured embedding space.
Recently, AL has been explored in vision~\&~language tasks with varying degrees of success~\cite{chi2019justasknavigation,lin2017activelearningvqa,misra2018learning,shen2019learning}.
\djkim{(TODO: add more references suggested by reviewers)}

\noindent\textbf{Visual Question Answering.}
VQA systems expect an input image and a natural language question pair and attempt to output a correct answer~\cite{antol2015vqa}, and the system has received a considerable amount of attention due to its real world applicability in recent years with the development of several datasets proposed as benchmarks~\cite{goyal2017making,johnson2017clevr,krishna2017visual,zhu2016visual7w,gurari2018vizwiz} and much progress has been made with various models~\cite{fukui2016multimodal,lu2016hierarchical,yang2016stacked,kim2018bilinear}. 
To extend the real-world applicability of VQA, the team at VizWiz~\cite{gurari2018vizwiz} constructed a dataset where blind people provide both question and image, and then request an answer.
Motivated by current VQA setups~\cite{antol2015vqa,gurari2018vizwiz}, we define our AL problem as finding informative image-question pairs to request an answer.
%\djkim{(maybe the paragraph is not coherent enough?)}

\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=0.9\linewidth,keepaspectratio]{Figures/architecture}
    \vspace{-2mm}
    \caption{\djkim{(Our model can be applied to any off-the-shelf VQA models. Our work is about designing good ad-hoc branches to measure (only measure) the uncertainty.)} Illustration of our VQA model architecture. We add two auxiliary branches $g_v(\cdot)$ and $g_q(\cdot)$ that process the visual or question features exclusively to generate answers from a single modality. Along with the cross-entropy loss from ground truth answers, the single-modal branches are trained with knowledge distillation loss to follow the output from the multi-modal branch $g(\cdot)$.
    % original multi-modal answer prediction branch.
    In particular, $F(\cdot,\cdot)$ components (in black) are trained with \Eref{eqn:loss_main} while $g_v(\cdot)$ and $g_q(\cdot)$ (in red) are trained with \Eref{eqn:loss_v} and \Eref{eqn:loss_q} respectively. \djkim{(VQA architecture itself is not a concern in our work. The goal is to make a favorable \emph{uncertainty measure} and the auxiliary branches are only for the uncertainty measure! The branches don't affect the model training.)}}
    \vspace{-2mm}
    \label{fig:architecture}
\end{figure*}

% To tackle such tasks, many have proposed architectures that encode and then merge the visual and textual information in order to classify the answers~\cite{jabri2016revisiting,ma2016learning,malinowski2015ask}.


% Attention mechanisms have proven to be successful in this task~\cite{anderson2018bottom,lu2016hierarchical,shih2016look,xu2016ask}, and other works have focused on designing effective multi-modal feature fusion schemes~\cite{ben2017mutan,fukui2016multimodal,kim2017hadamard}. 
% While the progress has been encouraging, such approaches require a large amount of labeled data.
% \jwcho{(this might not be very neccessary as we do not actually deal with attention mechanisms, rather, I think it might be bteter to simply talk about some of the various similar tasks and why it is out of our scope)}

Similar works such as~\cite{teney2018visual} and~\cite{misra2018learning} have explored VQA in a setting similar to that of Active Learning where each setting has an oracle of sorts and tries to better train the models. 
However, although some settings may seem similar, the basic idea is different as~\cite{misra2018learning} achieves performance improvements by augmenting data with an additional network and~\cite{teney2018visual} focuses on meta learning tasks such as few shot and zero shot learning with VQA, 
%proving that it is out of scope with what we are trying to deal with in this paper. 
which is a task well out of scope from our problem definition.
In addition, VQA models have also been shown to rely on priors and dataset biases~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors,}, and we get inspiration to leverage individual modalities from~\cite{cadene2019rubi}, but where~\cite{cadene2019rubi} uses a question only branch for the purposes of reducing bias at test time, we use both question-only and image-only as completely independent branches to measure mutual information, while the branches have no affect on the training or performance of our model.

% which we try to explore in our AL setting. 

% \djkim{(add \cite{teney2018visual} in the related work?)}\jwcho{(meta, i feel that this is quite a bit different from the scope...)}




% We explore a more realistic variant of VQA where models generate natural language answers, resulting in the generation of paraphrases.

%\noindent\textbf{Semantically structured embeddings.}
%Our key insight lies in moving uncertainty estimation from the model’s output space to a semantically structured internal embedding space. 
%Since we specifically study vision-language tasks, we build a visual-semantic space that combines both visual and textual information in order to create a unified latent representation. 
%This problem has been studied extensively in the last few years with work that involves jointly embedding images and text, at the word level~\cite{frome2013devise,kong2014you,joulin2016learning,matuszek2012joint,klein2015associating}, and sentence level~\cite{zitnick2013learning,karpathy2015deep,karpathy2014deep,chen2015mind,kiros2014unifying,reed2016learning}. 
%Visually grounded text representations have been applied to different tasks, including caption generation~\cite{kiros2014unifying,karpathy2015deep}, image retrieval~\cite{lin2014visual}, and visual question answering~\cite{malinowski2015ask}. 
%%Our approach is inspired by previous work~\cite{karpathy2014deep}, where we use image regions with their associated captions and adapt a margin objective to build the semantic space. 
%%We use the semantic space to enable a new active learning strategy.


%\noindent\textbf{Uncertainty.}
%As uncertainty estimation represents the most popular sampling strategy for active learning, we explore uncertainty estimation techniques developed for deep learning models. 
%Even though Deep Learning systems are performant, they remain uninterpretable, poor at quantifying predictive uncertainty, and overconfident in their predictions. 
%To mitigate this problem, Bayesian models have been proposed by placing a prior distribution over model weights [70, 53, 47]. 
%Yet, even though the problem is simple to formulate, deriving a posterior distribution for Deep Bayesian Neural Networks (BNN) is intractable which makes Bayesian inference difficult [18]. 
%Therefore, focus has shifted to approximating BNNs with variational inference. 
%Bayesian modeling of stochastic processes introduced new techniques into the field such as sampling-based and stochastic variational inference [6, 7]. 
%On the other hand, Monte-Carlo Dropout [19, 18] has empirically demonstrated comparable uncertainty estimation quality to variational inference [19]. 
%A model trained with dropout can be used as a Bayesian model by making multiple predictions while sampling different dropout masks for each forward propagation. 
%Estimating the posterior amounts to computing the mean and variance of the predictions. 
%While previous work has showed promise in classification and regression tasks [74, 18, 60], such methods have not been extended to language generation.
%In fact, most language-based uncertainty work adapts classification-based uncertainty techniques to language tasks, transforming the problem from an open language problem to a constrained closed problem [64, 22, 40, 24, 13]. 
%We propose a new sampling strategy that extends Monte-Carlo dropout uncertainty [18] to measure uncertainty in a semantic space.



%\noindent\textbf{Mutual Information in Deep Neural Networks.}
%asdfadf



==> Legacy/unused_2_sec_related_ICML.tex <==

We explore the field of Active Learning (AL) 
% and comment on how existing uncertainty measurements fail 
in the environment of multi-modality
% where we have multiple correct outputs. 
and place our work in the context of VQA, as we believe it is a highly representative manifestation of this environment. 
% Next, we dive into visual-semantic embedding, a practical solution to construct semantic spaces using
% visual priors. 
% Finally, we explore Bayesian uncertainty measurement techniques.

\noindent\textbf{Active Learning.} 
% \djkim{(We should put more recent AL papers \cite{sinha2019variational,zhang2020state} somewhere)}
A typical AL setting starts with a small initial set of labeled data $\mathcal{D}\textsubscript{L}$ and a large set of unlabeled data $\mathcal{D}\textsubscript{U}$. 
Knowing that labeling data is costly and time consuming, the task is to minimize the number of samples to annotate from $\mathcal{D}\textsubscript{U}$ while maximizing performance on a given task~\cite{tong2001support}. 
AL strategies have been successfully applied to a wide number of machine learning tasks, including image recognition~\cite{joshi2009multi,sener2017active,yoo2019learning}, information extraction~\cite{culotta2005reducing,jones2003active,scheffer2001active}, and text categorization~\cite{hoi2006batch,lewis1994sequential}, with strategies including uncertainty-based sampling~\cite{collins2008towards,joshi2009multi} and information gain~\cite{houlsby2011bayesian}.
While others have introduced a theoretical dropout-based framework to measure uncertainty~\cite{gal2017deep,kendall2017uncertainties}, more recent works have leveraged latent space representations with the help of variational autoencoders and adversarial training for improved sampling~\cite{sinha2019variational,zhang2020state,shuo2020daal}.
%%%%%%%%%%%%%%%%%%
% However, we although we compare our method to these approaches,
% as they require additional elaborately designed large networks to learn latent representation which have limited scalability to multi-modal tasks.
%%%%%%%%%%%%%%
We do not compare to methods that require multiple steps such as Monte-Carlo dropout or model ensemble (Query-by-Committee) as they are hard to apply to recent large models for higher-level tasks.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
% Similar solutions have been adapted to NLP tasks such as named entity recognition~\cite{shen2017deep} and neural semantic parsing by adding Gaussian noise to network weights~\cite{dong2018confidence}. 
%In this paper, we empirically show how previous uncertainty sampling strategies do not perform better than random sampling in a VQA setting and propose a novel strategy that uses Bayesian uncertainty in a semantically structured embedding space.
Recently, AL has been explored in vision~\&~language tasks with varying degrees of success~\cite{chi2019justasknavigation,lin2017activelearningvqa,misra2018learning,shen2019learning}.
% \djkim{(TODO: add more references suggested by reviewers)}

\noindent\textbf{Visual Question Answering.}
VQA systems expect an input image and a natural language question pair and attempt to output a correct answer~\cite{antol2015vqa}, and the system has received a considerable amount of attention due to its real-world applicability in recent years with the development of several datasets proposed as benchmarks~\cite{goyal2017making,johnson2017clevr,krishna2017visual,zhu2016visual7w,gurari2018vizwiz} and much progress has been made with various models~\cite{fukui2016multimodal,lu2016hierarchical,yang2016stacked,kim2018bilinear}. 
To extend the real-world applicability of VQA, the team at VizWiz~\cite{gurari2018vizwiz} constructed a dataset where blind people provide both question and image, and then request an answer.
Motivated by current VQA setups~\cite{antol2015vqa,gurari2018vizwiz}, we define our AL problem as finding informative image-question pairs to request an answer.
%\djkim{(maybe the paragraph is not coherent enough?)}


% To tackle such tasks, many have proposed architectures that encode and then merge the visual and textual information in order to classify the answers~\cite{jabri2016revisiting,ma2016learning,malinowski2015ask}.


% Attention mechanisms have proven to be successful in this task~\cite{anderson2018bottom,lu2016hierarchical,shih2016look,xu2016ask}, and other works have focused on designing effective multi-modal feature fusion schemes~\cite{ben2017mutan,fukui2016multimodal,kim2017hadamard}. 
% While the progress has been encouraging, such approaches require a large amount of labeled data.
% \jwcho{(this might not be very neccessary as we do not actually deal with attention mechanisms, rather, I think it might be bteter to simply talk about some of the various similar tasks and why it is out of our scope)}

\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=0.9\linewidth,keepaspectratio]{Figures/architecture}
    % \vspace{-2mm}
    \caption{Illustration of our model architecture. Our model can be applied to any off-the-shelf VQA models (hence the area in green shows a generic VQA architecture) as our goal is to design ad hoc branches solely for the purpose of \emph{measuring uncertainty}. We add two auxiliary branches $g_v(\cdot)$ and $g_q(\cdot)$ that process the visual or question features exclusively to generate answers from a single modality. Along with the cross-entropy loss from ground truth answers, the single-modal branches are trained with knowledge distillation loss to follow the output from the multi-modal branch $g(\cdot)$.
    % original multi-modal answer prediction branch.
    In particular, $F(\cdot,\cdot)$ components (in black) are trained with \Eref{eqn:loss_main} while $g_v(\cdot)$ and $g_q(\cdot)$ (in red) are trained with \Eref{eqn:loss_v} and \Eref{eqn:loss_q} respectively. \
    % djkim{(Our model can be applied to any off-the-shelf VQA models. Our work is about designing good ad hoc branches to measure (only measure) the uncertainty.)(VQA architecture itself is not a concern in our work. The goal is to make a favorable \emph{uncertainty measure} and the auxiliary branches are only for the uncertainty measure! The branches don't affect the model training.)}
    }
    \vspace{-2mm}
    \label{fig:architecture}
\end{figure*}



Similar works such as~\cite{teney2018visual} and~\cite{misra2018learning} have explored VQA in a setting similar to that of AL where each setting has an oracle of sorts and tries to better train the models. 
However, although some settings may seem similar, the base idea is different as~\cite{misra2018learning} achieves performance improvements by augmenting data with an additional network and~\cite{teney2018visual} focuses on meta learning tasks such as few shot and zero shot learning with VQA, 
%proving that it is out of scope with what we are trying to deal with in this paper. 
which is a task well out of scope from our problem definition.
In addition, VQA models have also been shown to rely on priors and dataset biases~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors,clark2019dont}, and we get inspiration to leverage individual modalities from~\cite{cadene2019rubi}, but where~\cite{cadene2019rubi} uses a question only branch for the purposes of reducing bias at test time, we use both question-only and image-only as completely independent branches to measure mutual information, while the branches have no affect on the training or performance of our model. To the best of our knowledge, we are the first to leverage mutual information of individual modalities to measure uncertainty in an Active Learning VQA setting.

% which we try to explore in our AL setting. 

% \djkim{(add \cite{teney2018visual} in the related work?)}\jwcho{(meta, i feel that this is quite a bit different from the scope...)}




% We explore a more realistic variant of VQA where models generate natural language answers, resulting in the generation of paraphrases.

%\noindent\textbf{Semantically structured embeddings.}
%Our key insight lies in moving uncertainty estimation from the model’s output space to a semantically structured internal embedding space. 
%Since we specifically study vision-language tasks, we build a visual-semantic space that combines both visual and textual information in order to create a unified latent representation. 
%This problem has been studied extensively in the last few years with work that involves jointly embedding images and text, at the word level~\cite{frome2013devise,kong2014you,joulin2016learning,matuszek2012joint,klein2015associating}, and sentence level~\cite{zitnick2013learning,karpathy2015deep,karpathy2014deep,chen2015mind,kiros2014unifying,reed2016learning}. 
%Visually grounded text representations have been applied to different tasks, including caption generation~\cite{kiros2014unifying,karpathy2015deep}, image retrieval~\cite{lin2014visual}, and visual question answering~\cite{malinowski2015ask}. 
%%Our approach is inspired by previous work~\cite{karpathy2014deep}, where we use image regions with their associated captions and adapt a margin objective to build the semantic space. 
%%We use the semantic space to enable a new active learning strategy.


%\noindent\textbf{Uncertainty.}
%As uncertainty estimation represents the most popular sampling strategy for active learning, we explore uncertainty estimation techniques developed for deep learning models. 
%Even though Deep Learning systems are performant, they remain uninterpretable, poor at quantifying predictive uncertainty, and overconfident in their predictions. 
%To mitigate this problem, Bayesian models have been proposed by placing a prior distribution over model weights [70, 53, 47]. 
%Yet, even though the problem is simple to formulate, deriving a posterior distribution for Deep Bayesian Neural Networks (BNN) is intractable which makes Bayesian inference difficult [18]. 
%Therefore, focus has shifted to approximating BNNs with variational inference. 
%Bayesian modeling of stochastic processes introduced new techniques into the field such as sampling-based and stochastic variational inference [6, 7]. 
%On the other hand, Monte-Carlo Dropout [19, 18] has empirically demonstrated comparable uncertainty estimation quality to variational inference [19]. 
%A model trained with dropout can be used as a Bayesian model by making multiple predictions while sampling different dropout masks for each forward propagation. 
%Estimating the posterior amounts to computing the mean and variance of the predictions. 
%While previous work has showed promise in classification and regression tasks [74, 18, 60], such methods have not been extended to language generation.
%In fact, most language-based uncertainty work adapts classification-based uncertainty techniques to language tasks, transforming the problem from an open language problem to a constrained closed problem [64, 22, 40, 24, 13]. 
%We propose a new sampling strategy that extends Monte-Carlo dropout uncertainty [18] to measure uncertainty in a semantic space.



%\noindent\textbf{Mutual Information in Deep Neural Networks.}
%asdfadf



==> Legacy/unused_2_sec_related_humantech.tex <==

We explore the field of Active Learning (AL) 
% and comment on how existing uncertainty measurements fail 
in the environment of multi-modality
% where we have multiple correct outputs. 
and place our work in the context of VQA, as we believe it is a highly representative manifestation of this environment. 
% Next, we dive into visual-semantic embedding, a practical solution to construct semantic spaces using
% visual priors. 
% Finally, we explore Bayesian uncertainty measurement techniques.

\noindent\textbf{Active Learning.} 
% \djkim{(We should put more recent AL papers \cite{sinha2019variational,zhang2020state} somewhere)}
A typical AL setting starts with a small initial set of labeled data $\mathcal{D}\textsubscript{L}$ and a large set of unlabeled data $\mathcal{D}\textsubscript{U}$. 
Knowing that labeling data is costly and time consuming, the task is to minimize the number of samples to annotate from $\mathcal{D}\textsubscript{U}$ while maximizing performance on a given task~\cite{tong2001support}. 
AL strategies have been successfully applied to a wide number of machine learning tasks, including image recognition~\cite{joshi2009multi,sener2017active,yoo2019learning}, information extraction~\cite{culotta2005reducing,jones2003active,scheffer2001active}, and text categorization~\cite{hoi2006batch,lewis1994sequential}, with strategies including uncertainty-based sampling~\cite{collins2008towards,joshi2009multi} and information gain~\cite{houlsby2011bayesian}.
While others have introduced a theoretical dropout-based framework to measure uncertainty~\cite{gal2017deep,kendall2017uncertainties}, more recent works have leveraged latent space representations with the help of variational autoencoders and adversarial training for improved sampling~\cite{sinha2019variational,zhang2020state,shuo2020daal}.
%%%%%%%%%%%%%%%%%%
% However, we although we compare our method to these approaches,
% as they require additional elaborately designed large networks to learn latent representation which have limited scalability to multi-modal tasks.
%%%%%%%%%%%%%%
We also do not compare to methods that require multiple steps such as Monte-Carlo dropout or model ensemble (Query-by-Committee) %as we \js{(???)}
as they are hard to apply to recent large models for higher-level tasks.
% Our proposed method enables simple inference to measure uncertainty without any ad hoc steps (Monte-Carlo dropout) or model ensemble (Query-by-Committee)
% \djkim{which are hard be applied in recent large models for higher-level tasks. (Maybe move this sentence to related work section?)}
% Similar solutions have been adapted to NLP tasks such as named entity recognition~\cite{shen2017deep} and neural semantic parsing by adding Gaussian noise to network weights~\cite{dong2018confidence}. 
%In this paper, we empirically show how previous uncertainty sampling strategies do not perform better than random sampling in a VQA setting and propose a novel strategy that uses Bayesian uncertainty in a semantically structured embedding space.
Recently, AL has been explored in vision~\&~language tasks with varying degrees of success~\cite{chi2019justasknavigation,lin2017activelearningvqa,misra2018learning,shen2019learning}.
% \djkim{(TODO: add more references suggested by reviewers)}

\noindent\textbf{Visual Question Answering.}
VQA systems expect an input image and a natural language question pair and attempt to output a correct answer~\cite{antol2015vqa}, and the system has received a considerable amount of attention due to its real-world applicability in recent years with the development of several datasets proposed as benchmarks~\cite{goyal2017making,johnson2017clevr,krishna2017visual,zhu2016visual7w,gurari2018vizwiz} and much progress has been made with various models~\cite{fukui2016multimodal,lu2016hierarchical,yang2016stacked,kim2018bilinear}. 
To extend the real-world applicability of VQA, the team at VizWiz~\cite{gurari2018vizwiz} constructed a dataset where blind people provide both question and image, and then request an answer.
Motivated by current VQA setups~\cite{antol2015vqa,gurari2018vizwiz}, we define our AL problem as finding informative image-question pairs to request an answer.
%\djkim{(maybe the paragraph is not coherent enough?)}


% To tackle such tasks, many have proposed architectures that encode and then merge the visual and textual information in order to classify the answers~\cite{jabri2016revisiting,ma2016learning,malinowski2015ask}.


% Attention mechanisms have proven to be successful in this task~\cite{anderson2018bottom,lu2016hierarchical,shih2016look,xu2016ask}, and other works have focused on designing effective multi-modal feature fusion schemes~\cite{ben2017mutan,fukui2016multimodal,kim2017hadamard}. 
% While the progress has been encouraging, such approaches require a large amount of labeled data.
% \jwcho{(this might not be very neccessary as we do not actually deal with attention mechanisms, rather, I think it might be bteter to simply talk about some of the various similar tasks and why it is out of our scope)}

Similar works such as~\cite{teney2018visual} and~\cite{misra2018learning} have explored VQA in a setting similar to that of AL where each setting has an oracle of sorts and tries to better train the models. 
However, although some settings may seem similar, the base idea is different as~\cite{misra2018learning} achieves performance improvements by augmenting data with an additional network and~\cite{teney2018visual} focuses on meta learning tasks such as few shot and zero shot learning with VQA, 
%proving that it is out of scope with what we are trying to deal with in this paper. 
which is a task well out of scope from our problem definition.
In addition, VQA models have also been shown to rely on priors and dataset biases~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, and we get inspiration to leverage individual modalities from~\cite{cadene2019rubi}, but where~\cite{cadene2019rubi} uses a question only branch for the purposes of reducing bias at test time, we use both question-only and image-only as completely independent branches to measure mutual information, while the branches have no affect on the training or performance of our model.

% which we try to explore in our AL setting. 

% \djkim{(add \cite{teney2018visual} in the related work?)}\jwcho{(meta, i feel that this is quite a bit different from the scope...)}




% We explore a more realistic variant of VQA where models generate natural language answers, resulting in the generation of paraphrases.

%\noindent\textbf{Semantically structured embeddings.}
%Our key insight lies in moving uncertainty estimation from the model’s output space to a semantically structured internal embedding space. 
%Since we specifically study vision-language tasks, we build a visual-semantic space that combines both visual and textual information in order to create a unified latent representation. 
%This problem has been studied extensively in the last few years with work that involves jointly embedding images and text, at the word level~\cite{frome2013devise,kong2014you,joulin2016learning,matuszek2012joint,klein2015associating}, and sentence level~\cite{zitnick2013learning,karpathy2015deep,karpathy2014deep,chen2015mind,kiros2014unifying,reed2016learning}. 
%Visually grounded text representations have been applied to different tasks, including caption generation~\cite{kiros2014unifying,karpathy2015deep}, image retrieval~\cite{lin2014visual}, and visual question answering~\cite{malinowski2015ask}. 
%%Our approach is inspired by previous work~\cite{karpathy2014deep}, where we use image regions with their associated captions and adapt a margin objective to build the semantic space. 
%%We use the semantic space to enable a new active learning strategy.


%\noindent\textbf{Uncertainty.}
%As uncertainty estimation represents the most popular sampling strategy for active learning, we explore uncertainty estimation techniques developed for deep learning models. 
%Even though Deep Learning systems are performant, they remain uninterpretable, poor at quantifying predictive uncertainty, and overconfident in their predictions. 
%To mitigate this problem, Bayesian models have been proposed by placing a prior distribution over model weights [70, 53, 47]. 
%Yet, even though the problem is simple to formulate, deriving a posterior distribution for Deep Bayesian Neural Networks (BNN) is intractable which makes Bayesian inference difficult [18]. 
%Therefore, focus has shifted to approximating BNNs with variational inference. 
%Bayesian modeling of stochastic processes introduced new techniques into the field such as sampling-based and stochastic variational inference [6, 7]. 
%On the other hand, Monte-Carlo Dropout [19, 18] has empirically demonstrated comparable uncertainty estimation quality to variational inference [19]. 
%A model trained with dropout can be used as a Bayesian model by making multiple predictions while sampling different dropout masks for each forward propagation. 
%Estimating the posterior amounts to computing the mean and variance of the predictions. 
%While previous work has showed promise in classification and regression tasks [74, 18, 60], such methods have not been extended to language generation.
%In fact, most language-based uncertainty work adapts classification-based uncertainty techniques to language tasks, transforming the problem from an open language problem to a constrained closed problem [64, 22, 40, 24, 13]. 
%We propose a new sampling strategy that extends Monte-Carlo dropout uncertainty [18] to measure uncertainty in a semantic space.



%\noindent\textbf{Mutual Information in Deep Neural Networks.}
%asdfadf



==> Legacy/unused_3_sec_method.tex <==
Our Active Learning (AL) method, Single-Modal Entropic Measure (SMEM), for Visual Question Answering consists of two key components: (1) devising an efficient and effective sample acquisition function which takes the mutual information of the individual modalities into account,~\Sref{sec:method}, and (2) introducing a novel self-distillation technique for effectively training the individual auxiliary branches for better sampling with SMEM,~\Sref{sec:distillation}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio]{Figures/entropy_GT.pdf}
%     \caption{Illustration of how outputs from different branches can be viewed and how distance can be measured. (a) shows when all branches have similar outputs, (b) and (c) show cases where one output is similar to the main branch while the other is not. In order to get the most informative sample, our model searches for the ones that look like (d). (e) shows the legend}
%     \label{fig:entropy}
% \end{figure}


\begin{figure}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=1\linewidth,keepaspectratio]{Figures/architecture}
    \vspace{-4mm}
    \caption{Illustration of our model architecture. We add two auxiliary branches $g_v(\cdot)$ and $g_q(\cdot)$ that process the visual or question features exclusively to generate answers from a single modality. Along with the cross-entropy loss from ground truth answers, the single-modal branches are trained with knowledge distillation loss to follow the output from the multi-modal branch $g(\cdot)$.
    % original multi-modal answer prediction branch.
    In particular, $F(\cdot,\cdot)$ components (in black) are trained with \Eref{eqn:loss_main} while $g_v(\cdot)$ and $g_q(\cdot)$ (in red) are trained with \Eref{eqn:loss_v} and \Eref{eqn:loss_q} respectively.
    }
    \vspace{-2mm}
    \label{fig:architecture}
\end{figure}


\subsection{Visual Question Answering Baseline}

Given an image $V$ and question $Q$, the goal of the VQA task is to correctly predict an answer from the answer set $A\in\mathcal{A}$ (in a vectorized form, $\hat{\mathbf{y}}=F(V,Q)\in [0,1]^{|\mathcal{A}|}$), 
and we adapt one of the famous VQA state-of-the-art models as our base architecture~\cite{anderson2018bottom} where $F(\cdot,\cdot)$ is implemented via a combination of
% a deep neural network consisting of both 
convolutional and recurrent neural networks.
% \js{(Generally, any ML model but we used SOTA DL model?)}
% We adopt one of the famous V,QA state-of-the-art model~\cite{anderson2018bottom} as our base architecture.
Images and questions are mapped to feature vectors through convolutional ($f_v(\cdot)$) and recurrent ($f_q(\cdot)$) neural networks respectively: 
% to the form: 
% \js{(How? What is the mapping function? Learned?)}
\begin{equation}
    \mathbf{z}_v = f_v(V), \mathbf{z}_q = f_q(Q).
\end{equation}
Then following~\cite{anderson2018bottom}, $\mathbf{z}_v$ and $\mathbf{z}_q$ are combined via an additional sub-network $f_z(\cdot,\cdot)$ which includes attention and Hadamard product to generate joint representation:
\begin{equation}
    \mathbf{z}=f_z(\mathbf{z}_v,\mathbf{z}_q).
\end{equation}
Finally, $\mathbf{z}$ is fed through a fully-connected layer $g(\cdot)$ to predict $\hat{\mathbf{y}}$:
\begin{equation}
    \hat{\mathbf{y}}=g(\mathbf{z}).
\end{equation}
The goal for training a VQA model is to follow the conditional distribution of the target dataset:
\begin{equation}
    \hat{\mathbf{y}}=F(V,Q) \approx P(A|V,Q), 
\end{equation}
where $F(\cdot,\cdot)$ is the VQA model, and $P(\cdot)$ is the probability of the answer $A$ given image $V$ and question $Q$ predicted from $F(\cdot,\cdot)$.
% ($\hat{\mathbf{y}}^i = P(A=i|V,Q)$). 
Thus, the model is trained with Binary Cross-Entropy loss compared with ground truth $\mathbf{y}$:
\begin{equation}
    \mathcal{L}_{main} = BCE(\mathbf{y},\hat{\mathbf{y}}).
    \label{eqn:loss_main}
\end{equation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Learning with SMEM}%Mutual Information based Sampling Strategy}
\label{sec:method}
% \djkim{(we would need a reason why the mutual informatino of one of the modality $I(A;V|Q)$ and $I(A;Q|V)$ matters while not considering $I(A;QV)$.)}
% \djkim{(There should be definitions of $\mathcal{D}\textsubscript{U}$ and $\mathcal{D}\textsubscript{L}$ around here.)}
% In active learning, there exists a labeled set of $\mathcal{D}\textsubscript{L}$ image/question/answer tripletS that are used for training and a pool of $\mathcal{D}\textsubscript{U}$ triplets that the trained VQA model that will be sampled from.
The goal of AL is to find the best sample acquisition function $S(V,Q)$ that assigns a high score to \emph{informative} samples. In the AL setup, a labeled set $\mathcal{D}\textsubscript{L}$ is used to train a model, then after the model converges (end of a \emph{stage}), the model is used to sample from the unlabeled set $\mathcal{D}\textsubscript{U}$, then the chosen samples are given labels and added into the labeled set $\mathcal{D}\textsubscript{L}$ and removed from the unlabeled set $\mathcal{D}\textsubscript{U}$. This step is repeated several times depending on the number of stages (hyper-parameter).
In this paper, we define a novel acquisition function that takes \emph{mutual information} into account.
% Our approach exploits the multi-modality of the task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ as a sampling criteria instead of being grounded to only considering the final output representation $I(A; Y)$. 
Our approach exploits the multi-modality of this task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ individually %which are representations of image $V$ and question $Q$ respectively, 
to aid the sampling criteria instead of simply relying on $I(A;V,Q)$, the final output representation.
%, \djkim{whole input representation.}
%considering $I(A; V,Q)$ using the  %final output representation $Y$.
% Previous methods only consider the final output representation $\hat{Y}$. 
Since VQA has issues of relying on a single modality and of dataset bias~\cite{agrawal2016analyzevqa,agrawal2018don,cadene2019rubi,goyal2017making,jabri2016revisiting,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, sampling from a VQA model's output representation can make the model prone to selecting outliers or samples that are directly contrasting. 
% in avoiding overfitting and outlier sampling. 
% \djkim{(What would be the problem of the existing approaches theoretically?)}

Intuitively, if the value of mutual information, for example $I(A;V|Q)$, is high, the variable $V$ plays an important role in predicting the answer $A$.
In typical off-the-shelf models, directly computing the mutual information of individual modalities is difficult.
To this end, we add additional ad hoc branches to compute the mutual information which is described in the following subsection in detail. 
% Therefore, we choose to use mutual information in our sampling scheme.

% In order to measure the informativeness, we add additional branches that predict answer only from visual features as shown in \Fref{fig:architecture}. 
As shown in \Fref{fig:architecture}, we add additional branches that predict the answer exclusively from visual and question features to measure the informativeness of each modality.
The branches are also trained with cross-entropy loss with ground truth answers so that the output answer probability can approximate the conditional distribution of answers given cues such that $\mathbf{y}_v=g_v(\mathbf{z}_v) \approx P(A|V)$ for visual and $\mathbf{y}_q=g_q(\mathbf{z}_q) \approx P(A|Q)$ for question.

As we try to measure the informativeness of the given input visual question pair $(V,Q)$ through a proper acquisition function $S(V,Q)$, we can intuitively expect that the input cue $V$ or $Q$ may contain a considerable amount of information if the single-modal outputs $\mathbf{y}_v$ and $\mathbf{y}_q$ are considerably different from $\hat{\mathbf{y}}$. In this regard, we devise a novel acquisition function that takes into account the relation between the single-modal and multi-modal answer representations.





% \begin{equation}
%     Y_v=g_v(z_v) \approx p_\theta(y|v).
% \end{equation}

% Likewise, we can also define answer prediction only from a question feature:
% \begin{equation}
%     Y_q=g_q(z_q) \approx p_\theta(y|q).
% \end{equation}


% As our goal in this work is to leverage the three cues, $Y_v$, $Y_q$, and $\hat{Y}$ to effectively measure the informativeness of the given input visual-question pair $(V,Q)$ through a proper acquisition function $S(V,Q)$.
% Intuitively, if the single-modal outputs $Y_v$ and $Y_q$ are different enough from a multi-modal output $\hat{Y}$, one can expect the input cue $V$ or $Q$ may contain a considerable amount of information in order to predict a correct answer. In this regard, we devise a novel acquisition function that take the relation between the single-modal and multi-modal answer representations into account. \jwcho{(i really feel this paragraph and the one from line 111~119 redundant, but not, so must be changed... i cant think of a way yet)}

% \djkim{(possible tackle? other multi-modal tasks? maybe our idea is based on classification task)}


\noindent\textbf{Single-Modal Entropic Measure (SMEM).} %(our name???)
As our goal is to find the training data points that has high mutual information %with output answers 
$I(A;V|Q)$ and $I(A;Q|V)$,
according to the property of mutual information, the terms can be decomposed to the difference of entropy:
\begin{equation}
    I(A;V|Q) = H(A|Q) - H(A|V,Q) \approx H(Y_q) - H(\hat{Y}),
    \label{eqn:MI_Q}
\end{equation}
\begin{equation}
    I(A;Q|V) = H(A|V) - H(A|V,Q) \approx H(Y_v) - H(\hat{Y}),
    \label{eqn:MI_V}
\end{equation}
where $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ 
% \js{(H(\hat{Y})?)} 
is the entropy of a given distribution. As shown in the equations above, we see that mutual information easily be computed from the entropy values of the single-modal outputs and the multi-modal output.

On the other hand, if we modify \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can derive the equations:
\begin{equation}
    H(Y_q) \approx H(A|Q) = I(A;V|Q) + H(A|V,Q),
    \label{eqn:single-Q}
\end{equation}
\begin{equation}
    H(Y_v) \approx H(A|V) = I(A;Q|V) + H(A|V,Q),
    \label{eqn:single-V}
\end{equation}
where $H(Y_q)=-\sum_{i} \mathbf{y}_q^i\log \mathbf{y}_q^i$  and $H(Y_v)=-\sum_{i} \mathbf{y}_v^i\log \mathbf{y}_v^i$ . From \Eref{eqn:single-Q} and \Eref{eqn:single-V}, we can see that the entropy of the single-modal output is the sum of the mutual information and the entropy of the multi-modal output, and we want both values to be high when sampling.
% which are both we want to find samples with high values of.

In this regard, we propose an informativeness value to be the weighted sum of the single-modal entropy for image and question, \textbf{SMEM}:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v), 
    \label{eqn:student}
\end{equation}
where $0\leq \alpha \leq 1$  is a hyper-parameter that weights between visual and question scores.
Note that $0 \leq S(V,Q)\leq \log |\mathcal{A}|$, because $0 \leq H(\cdot) \leq \log |\mathcal{A}|$.





\begin{figure}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=1\linewidth,keepaspectratio]{Figures/jensenshanon.pdf}
    \vspace{-6mm}
    \caption{Illustration of differences of the outputs from $g(\cdot)$, $g_v(\cdot)$, and $g_q(\cdot)$.
    In our SMEM measure, which measures the difference between main output and the single-modal outputs, we give a higher score to (a) than (b) in the sampling stage. However, we can also intuitively expect (c) to be more informative than (b). Thus, we also propose to add Jensen-Shannon divergence between the two single-modal outputs in order to account for the distances between single-modal outputs.}
    \vspace{-2mm}
    \label{fig:jensenshanon}
\end{figure}



In addition, we also conjecture that as the information of the
% important information is not only information about the 
relationships between all single-modal and multi-modal outputs are important, the information of the relationship between the single-modal outputs is just as important.
As in \Fref{fig:jensenshanon} (a) and (b), even though the distance between single-modal outputs and the multi-modal output is fixed, the relationship between the three distributions can differ due to the distance between single-modal outputs.
In this regard, we also leverage \textbf{Jensen-Shannon divergence} as an additional sampling criterion:
\begin{equation}
    JSD(\mathbf{y}_v||\mathbf{y}_q) = (D_{KL}(\mathbf{y}_v||M)+D_{KL}(\mathbf{y}_q||M))/2, 
    \label{eqn:jsd}
\end{equation}
where  $M = (\mathbf{y}_v+\mathbf{y}_q)/2$. Therefore, our criterion can be modified by introducing an additional hyper-parameter $\beta \geq0$:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q).
    \label{eqn:addJSD}
\end{equation}
Note that $S(V,Q)\geq0$, because both entropy and Jensen-Shannon divergence are always non-negative.
We empirically found that adding $JSD(\mathbf{y}_v||\mathbf{y}_q)$ improved the active learning performance.



\noindent\textbf{Other possible approaches.} 
As the comparison target of our approach, we also test different measures for distribution discrepancy.
In the following paragraphs, we introduce several possible candidates to measure the distances between single-modal and multi-modal answer representations.

\textbf{\emph{(1) KL-Divergence (KLD)}} is defined as follows:
\begin{equation}
    D_{KL}(\mathbf{y}||\mathbf{y}_q) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_q)}, %= H(Y,Y_q) - H(\hat{Y}),
\end{equation} 
\begin{equation}
    D_{KL}(\mathbf{y}||\mathbf{y}_v) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_v)}. %= H(Y,Y_v) - H(\hat{Y}),
\end{equation} 
%where $H(Y,Y_q)$ and $H(Y,Y_v)$ are the cross-entropies of the single-modal answers compared to multi-modal answers.
Similar to our approach, by combining the two distance metrics via weighted sum, we have the KL-divergences:
\begin{equation}
    S(V,Q) = \alpha D_{KL}(\mathbf{y}||\mathbf{y}_q) + (1-\alpha) D_{KL}(\mathbf{y}||\mathbf{y}_v),
    \label{eqn:kld}
\end{equation}
where $\alpha$ is a hyper-parameter that weights between visual and question scores.
Note that $S(V,Q)\geq0$, because KL-divergence is always non-negative.

%\textbf{\emph{(2) Mutual information (MI)}} alone can also be used as informativeness measure.
%By combining \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can compute the combined version of mutual information values:
%\begin{equation}
%    R = \alpha (H(Y_q) - H(\hat{Y})) + (1-\alpha) (H(Y_v) - H(\hat{Y})).
%\end{equation}
%%Note that $R\geq0$, because mutual information is always non-negative.



\textbf{\emph{(2) Absolute Difference of KL-Divergence (AD-KLD)}} can also be used:
\begin{equation}
    S(V,Q) = |D_{KL}(\mathbf{y}||\mathbf{y}_q) - D_{KL}(\mathbf{y}||\mathbf{y}_v)|.
    \label{eqn:ad-kld}
\end{equation}
Although these methods have strong theoretical backing, we empirically show that for our problem, our proposed method shows the best performance.
% among the other options.



\noindent\textbf{Acquisition function of SMEM.}
After each stage, we utilize the trained model to sample the most informative visual-question pairs with respect to our acquisition function $S(V,Q)$.



%\noindent\textbf{Weighted sum with entropy.}
We empirically found that adding the entropy term of the multi-modal output additionally improved the performance.
In particular, our final acquisition function is defined as follows:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y}),
    \label{eqn:final}
\end{equation}
where $\gamma \geq0$ is the hyper-parameter that weights between the other functions and the entropy.
Note that $S(V,Q)\geq0$, because both entropy and Jensen-Shannon divergence are always non-negative.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-Distillation}
\label{sec:distillation}
The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are under the assumption that the classifiers $g_v(\cdot)$ and $g_q(\cdot)$ as well as $g(\cdot)$ are well trained to model the distribution of the labeled dataset.
Therefore, in order to satisfy the assumption, we need to better train $g_v(\cdot)$ and $g_q(\cdot)$.
To do so, we additionally propose the self-distillation~\cite{phuong2019distillation,zhang2019your} technique to work as a regularizer~\cite{phuong2019distillation,zhang2019your}.
Our insight is as follows: our acquisition function $S(V,Q)$ tries to find the sample that has a large difference between the teacher and the student. By adding knowledge distillation loss to directly minimize this difference, the easy samples will be forced to have a low $S(V,Q)$. In other words, if a sample gives a high $S(V,Q)$ value even after the explicit minimization of the $S(V,Q)$ score, the sample can be thought of a sample that is difficult and requires an oracle to label.
% \js{(One concern is whether mutual info calculation will still be effective with self distillation)}

Knowledge Distillation~\cite{hinton2015distilling} is defined as: training a ``student'' to follow a ``teacher'' model or representation.
Given a final output generated from a student model (in our case, $\mathbf{y}_v$ and $\mathbf{y}_q$) and an output from the teacher model (in our case, $\hat{\mathbf{y}}$), the student model learns the knowledge in the teacher's representation by forcing the student's representation to be similar to the teacher's.

% \begin{equation}
% 	\mathcal{L}_{distill}( \mathbf{y}_t,\mathbf{y}_s  ) = BCE(\mathbf{y}_t',\mathbf{y}_s'),
% 	\label{eq:loss_LWF}
% \end{equation}
% where
% \begin{equation}
% 	\\{y'}_k = \frac{(y_k)^{1/T}}{\sum_{k}^{}{(y_k)^{1/T}}}.
% 	\label{eqn:distillation}
% \end{equation}
% \djkim{(oh....eq(17) is for the distillation with CE loss, not BCE. We should remove eq(17))}
% where $y'_k$ is each individual output from the vector $\mathbf{y}$ of length $_k$ and $T$ is a hyperparameter \emph{Temperature}.
This approach suits our problem definition where the $g_v(\cdot)$ and $g_q(\cdot)$ can be student models and our $g(\cdot)$ can be the teacher model.
We believe that adding the
% As $g_v(\cdot)$ and $g_q(\cdot)$ are only trained on classification loss,
self-distillation loss in addition to the classification loss can aid in training $g_v(\cdot)$ and $g_q(\cdot)$ to improve our acquisition function directly. We empirically prove our approach through the sampling performance gain.
% that the self-distillation loss aids in overall performance gain. 

% While the theory is sound, if the network (especially visual/question branch) is not well trained enough, we cannot guarantee that the acquisition function $S(V,Q)$ to work properly.
% Therefore, we 
% propose to 
% add knowledge distillation loss to boost the active learning performance.
% \js{(active learning performance or learning performance?)}
% \js{(self distillation enforces all branches to predict similarly?)}

% Our insight is as follows.
% Our acquisition function $S(V,Q)$ is to find the sample that has large distance between teacher and student.
% If we add the knowledge distillation loss to directly minimize this distance, the easy samples will be forced to have low $S(V,Q)$ values.
% \jwcho{(i dont know if i like this word encouraged... can we use a stronger word like force? or isit too strong?)}
% \js{(enforced?)}
% In other words, if a sample gives high value for $S(V,Q)$ even though we tried to explicitly minimize the $S(V,Q)$ score, the sample is highly likely to require oracle to label.
% In a mathematical interpretation.....\djkim{(maybe generalization bound?)}



%The loss function to train auxiliary branches is defined as 
The auxiliary single-modal branches are trained with the following loss functions:
\begin{equation}
    \mathcal{L}_v =  BCE(\mathbf{y},\mathbf{y}_v)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_v),
    \label{eqn:loss_v}
\end{equation}
\begin{equation}
    \mathcal{L}_q = BCE(\mathbf{y},\mathbf{y}_q)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_q),
    \label{eqn:loss_q}
\end{equation}
where %$\mathcal{L}_{distill}(\cdot,\cdot)$ is the knowledge distillation loss~\cite{hinton2015distilling}.
%$\theta_v$ and $\theta_q$ are the parameter of the auxiliary single-modal branches $g_v(\cdot)$ and $g_q(\cdot)$ and 
$\lambda \geq0$ is a hyper-parameter to balance the loss weights.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Theoretical Properties}

% from introduction section. lets see where we can place this
% During the training phase, our model learns multiple branch of outputs which represents single-modal output and multi-modal output respectively.
% We additionally propose to use self-distillation framework~\cite{} for better training between single-modal and muti-modal outputs for single-modal output to predict answer as correct as multi-modal branch.


Re-examining our model, the training and sampling is reminiscent of Generative Adversarial Networks~\cite{goodfellow2014generative}, where the model is trained to produce the same output between single- and multi-modal, whereas in sampling, we label the data points that show a large gap between the two outputs.
% The strategy follows the intuition that if the output probability of the multi-modal and single-modal of the active learner is different, then it means that the missing sample is informative. \jwcho{(maybe here we can refer to the figure??)}
% \js{(Mentioning mini-max is understandable but, not sure if this can claim it is doing mini-max, because there is no 2-player aspect in loss function. Infact 2-players are doing the same thing, while HOPING that training is sufficient for prediction while insufficient for sampling.)}
% Therefore, instead of simply computing the entropy of the multi-modal output, we propose to use the entropy difference, which is the mutual information, to estimate the uncertainty of the unlabeled sample.
% With the proposed framework, we demonstrate the significant performance improvements in active learning setup.
% \djkim{(Let's move this details to the method section.)}
% --------------------------------------------------------

%\subsection{Temperature in Distillation Loss}









==> Legacy/unused_3_sec_method_AAAI.tex <==


Our Active Learning (AL) method, Single-Modal Entropic Measure (SMEM) for Visual Question Answering consists of two key components: (1) devising an efficient and effective sample acquisition function which takes the mutual information of the individual modalities into account and (2) introducing a novel self-distillation technique for effectively training the individual auxiliary branches for better sampling with SMEM.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio]{Figures/entropy_GT.pdf}
%     \caption{Illustration of how outputs from different branches can be viewed and how distance can be measured. (a) shows when all branches have similar outputs, (b) and (c) show cases where one output is similar to the main branch while the other is not. In order to get the most informative sample, our model searches for the ones that look like (d). (e) shows the legend}
%     \label{fig:entropy}
% \end{figure}





\subsection{Visual Question Answering Baseline}

Given an image $V$ and question $Q$, the goal of the VQA task is to correctly predict an answer from the answer set $A\in\mathcal{A}$ (in a vectorized form, $\hat{\mathbf{y}}=F(V,Q)\in [0,1]^{|\mathcal{A}|}$), 
and we adapt one of the famous VQA state-of-the-art models as our base architecture~\cite{anderson2018bottom} where $F(\cdot,\cdot)$ is implemented via a combination of
% a deep neural network consisting of both 
convolutional and recurrent neural networks.
% \js{(Generally, any ML model but we used SOTA DL model?)}
% We adopt one of the famous V,QA state-of-the-art model~\cite{anderson2018bottom} as our base architecture.
Images and questions are mapped to feature vectors through convolutional ($f_v(\cdot)$) and recurrent ($f_q(\cdot)$) neural networks respectively (\emph{i.e.}, $\mathbf{z}_v = f_v(V), \mathbf{z}_q = f_q(Q).$).
Then following~\cite{anderson2018bottom}, $\mathbf{z}_v$ and $\mathbf{z}_q$ are combined via an additional sub-network $f_z(\cdot,\cdot)$ which includes attention and Hadamard product to generate joint representation (\emph{i.e.}, $\mathbf{z}=f_z(\mathbf{z}_v,\mathbf{z}_q)$).
Finally, $\mathbf{z}$ is fed through a fully-connected layer $g(\cdot)$ to predict $\hat{\mathbf{y}}$ (\emph{i.e.}, $\hat{\mathbf{y}}=g(\mathbf{z})$).
The goal for training the VQA model is to follow the conditional distribution of the target dataset:
\begin{equation}
    \hat{\mathbf{y}}=F(V,Q) \approx P(A|V,Q), 
\end{equation}
where $F(\cdot,\cdot)$ is the VQA model, and $P(\cdot)$ is the probability of the answer $A$ given image $V$ and question $Q$ %predicted from $F(\cdot,\cdot)$.
that we want $F(\cdot,\cdot)$ to follow.
% ($\hat{\mathbf{y}}^i = P(A=i|V,Q)$). 
Thus, the model is trained with Binary Cross-Entropy loss compared with ground truth $\mathbf{y}$:
% \djkim{(and maybe this?)}
\begin{equation}
    \mathcal{L}_{main} = BCE(\mathbf{y},\hat{\mathbf{y}}).
    \label{eqn:loss_main}
\end{equation}



\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=.8\linewidth,keepaspectratio]{Figures/jensenshanon.pdf}
    \vspace{0mm}
    \caption{
    Illustration of differences of the outputs from $g(\cdot)$, $g_v(\cdot)$, and $g_q(\cdot)$.
    In our SMEM measure, which measures the difference between main output and the single-modal outputs, we give a higher score to (a) than (b) in the sampling stage. However, we can also intuitively expect (c) to be more informative than (b). Thus, we also propose to add Jensen-Shannon divergence between the two single-modal outputs in order to account for the discrepancies between single-modal outputs.}
    \vspace{-2mm}
    \label{fig:jensenshanon}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Learning with SMEM}%Mutual Information based Sampling Strategy}
\label{sec:method}
\djkim{(data-points are sampled from the fixed size unlabeled pool, not by checking all the (image-question) pairs.)}
% \djkim{(we need to mention that entropy is one of the powerful method, and we are adding mutual information upon entropy which is single-modal entropy)}
% \djkim{(we would need a reason why the mutual informatino of one of the modality $I(A;V|Q)$ and $I(A;Q|V)$ matters while not considering $I(A;QV)$.)}
% \djkim{(There should be definitions of $\mathcal{D}\textsubscript{U}$ and $\mathcal{D}\textsubscript{L}$ around here.)}
% In active learning, there exists a labeled set of $\mathcal{D}\textsubscript{L}$ image/question/answer tripletS that are used for training and a pool of $\mathcal{D}\textsubscript{U}$ triplets that the trained VQA model that will be sampled from.
The goal of AL is to find the best sample acquisition function $S(V,Q)$ that assigns a high score to \emph{informative} samples.
% (\emph{e.g.}, entropy $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ by defining uncertainty as informativeness). 
In the AL setup, a labeled set $\mathcal{D}\textsubscript{L}$ is used to train a model, then after the model converges (end of a \emph{stage}), the model is used to sample from the unlabeled set $\mathcal{D}\textsubscript{U}$, then the chosen samples are given labels and added into the labeled set $\mathcal{D}\textsubscript{L}$ and removed from the unlabeled set $\mathcal{D}\textsubscript{U}$. This step is repeated several times depending on the number of stages (hyper-parameter).
There are several ways to define the informativeness of a sample. For example, entropy, which is defined as $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$, does this by defining uncertainty as informativeness.
However, in this paper, we define a novel acquisition function that takes \emph{mutual information} into account.
% Our approach exploits the multi-modality of the task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ as a sampling criteria instead of being grounded to only considering the final output representation $I(A; Y)$. 
Our approach exploits the multi-modality of this task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ individually %which are representations of image $V$ and question $Q$ respectively, 
to aid the sampling criteria instead of simply relying on $I(A;V,Q)$, the final output representation.
%, \djkim{whole input representation.}
%considering $I(A; V,Q)$ using the  %final output representation $Y$.
% Previous methods only consider the final output representation $\hat{Y}$. 
Since VQA has issues on relying 
% shown to be reliant
on a single modality and dataset bias~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, sampling from a VQA model's output representation can make the model prone to selecting outliers or samples that are drastically different only in output representation space.
% in avoiding overfitting and outlier sampling. 
% \djkim{(What would be the problem of the existing approaches theoretically?)}

Intuitively, if the value of mutual information, for example $I(A;V|Q)$, is high, the variable $V$ plays an important role in predicting the answer $A$.
In a typical off-the-shelf model, directly computing the mutual information of individual modalities is difficult.
% To this end, we add additional ad hoc branches to compute the mutual information which is described in the following subsection in detail. 
% As shown in \Fref{fig:architecture}, 
In contrast, we add 
independent classification branches, as shown in \Fref{fig:architecture}, that predict the answer exclusively from visual and question single features to measure mutual information and the informativeness of each modality.\djkim{($\leftarrow$we should clarify these sentences. Our ultimate goal is to measure the uncertainty, and in order to implement that according to our formulation, we need to add additional single-modal branches.)}
The branches are detached from the model, meaning the gradients of the branches are cut off from the main model, which in turn means that the presence of the branch additions have no effect on the main model performance, and is trained with cross-entropy loss with ground truth answers so that the output answer probability can approximate the conditional distribution of answers given cues such that $\mathbf{y}_v=g_v(\mathbf{z}_v) \approx P(A|V)$ for visual and $\mathbf{y}_q=g_q(\mathbf{z}_q) \approx P(A|Q)$ for question.
\djkim{(note that the answer prediction from the single-modal classifiers don't have to be accurate because these outputs are only used for measuring uncertainty.)}

As we try to measure the informativeness of a given input visual question pair $(V,Q)$ through a given acquisition function $S(V,Q)$, we can intuitively expect that the input cue $V$ or $Q$ may contain a considerable amount of information if the single-modal outputs $\mathbf{y}_v$ and $\mathbf{y}_q$ are considerably different from $\hat{\mathbf{y}}$. 
%In addition, as entropy is a powerful metric for AL, where entropy is ($H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$). 
By measuring the uncertainty of the model predictions, we devise a novel acquisition function based on entropy that takes into account the relation between the single-modal and multi-modal answer representations and show significant performance gains.
% \djkim{(we can say that simple entropy is only for uncertainty, ours is uncertainty+mutual information!)}\jwcho{(got it!)}
% Since entropy is the most famous metric for AL, based on the core idea of entropy, we introduce a new metric that outperforms it. 
% \djkim{Entropy is the most famous metric for AL, but we introduce better way than the Entropy}



% \begin{equation}
%     Y_v=g_v(z_v) \approx p_\theta(y|v).
% \end{equation}

% Likewise, we can also define answer prediction only from a question feature:
% \begin{equation}
%     Y_q=g_q(z_q) \approx p_\theta(y|q).
% \end{equation}


% As our goal in this work is to leverage the three cues, $Y_v$, $Y_q$, and $\hat{Y}$ to effectively measure the informativeness of the given input visual-question pair $(V,Q)$ through a proper acquisition function $S(V,Q)$.
% Intuitively, if the single-modal outputs $Y_v$ and $Y_q$ are different enough from a multi-modal output $\hat{Y}$, one can expect the input cue $V$ or $Q$ may contain a considerable amount of information in order to predict a correct answer. In this regard, we devise a novel acquisition function that take the relation between the single-modal and multi-modal answer representations into account. \jwcho{(i really feel this paragraph and the one from line 111~119 redundant, but not, so must be changed... i cant think of a way yet)}

% \djkim{(possible tackle? other multi-modal tasks? maybe our idea is based on classification task)}


\noindent\textbf{Single-Modal Entropic Measure (SMEM).} %(our name???)
\djkim{(we should emphasize more that none of these methods effect the model training. All these methods are only for measuring the uncertainty.)}
Our goal is to find the training data points that have high mutual information %with output answers 
$I(A;V|Q)$ and $I(A;Q|V)$, and according to the property of mutual information, it can be decomposed into the difference of entropies:
\begin{equation}
    I(A;V|Q) = H(A|Q) - H(A|V,Q) \approx H(Y_q) - H(\hat{Y}),
    \label{eqn:MI_Q}
\end{equation}
\begin{equation}
    I(A;Q|V) = H(A|V) - H(A|V,Q) \approx H(Y_v) - H(\hat{Y}),
    \label{eqn:MI_V}
\end{equation}
where $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ 
is the entropy of a given distribution. 
As shown in the equations above, we see that mutual information is easily computed from the entropy values of the single-modal and multi-modal outputs.
\djkim{This is from the assumption that $H(A|V,Q)$, $H(A|Q)$, and $H(A|V)$ are modeled with $H(\hat{Y})$, $H(Y_q)$, and $H(Y_v)$ respectively (\ie~$H(A|V,Q) \approx H(\hat{Y})$, $H(A|Q)\approx H(Y_q)$, $ H(A|V)\approx H(Y_v)$)}.

% On the other hand, if we modify \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can derive the equations:

%On the other hand, 
In effect, \djkim{similarly,}
rearranging \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we get:
\begin{equation}
    H(Y_q) \approx H(A|Q) = I(A;V|Q) + H(A|V,Q),
    \label{eqn:single-Q}
\end{equation}
\begin{equation}
    H(Y_v) \approx H(A|V) = I(A;Q|V) + H(A|V,Q),
    \label{eqn:single-V}
\end{equation}
where $H(Y_q)=-\sum_{i} \mathbf{y}_q^i\log \mathbf{y}_q^i$  and $H(Y_v)=-\sum_{i} \mathbf{y}_v^i\log \mathbf{y}_v^i$ . From \Eref{eqn:single-Q} and \Eref{eqn:single-V}, we can see that the entropy of the single-modal output is the sum of the mutual information and the entropy of the multi-modal output, and we want both values to be high when sampling.
% which are both we want to find samples with high values of.
In other words,
% one can find training samples in terms of
both uncertainty and informativeness can be measured by simply computing the \emph{entropy of the single-modal output}.

In this regard, we propose an informativeness value to be the weighted sum of the single-modal entropy for image and question, \textbf{SMEM}:
%\djkim{(notation overload in $S(V,Q)$. maybe use different notation?)}
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v), 
    \label{eqn:student}
\end{equation}
where $0\leq \alpha \leq 1$  is a hyper-parameter that weights the relative importance of visual and question scores.
Note that $0 \leq S(V,Q)\leq \log |\mathcal{A}|$, because $0 \leq H(\cdot) \leq \log |\mathcal{A}|$.





In addition, we also conjecture that as the information of the
% important information is not only information about the 
relationships between all single-modal and multi-modal outputs are important, the information of the relationship between the single-modal outputs is just as important.
As in \Fref{fig:jensenshanon} (b) and (c), even though the distance between single-modal outputs and the multi-modal output is fixed, the relationship between the three distributions can differ due to the distance between single-modal outputs.
If we only leverage the distance between the single-modal and multi-modal outputs, (b) and (c) would give the same score, however, we can intuitively understand that (c) is more uncertain than (b) as the distance between the single-modal outputs is much greater.
In order to measure this distance between the single-modal outputs on top of the distances between the single-modal and multi-modal outputs, we propose to also leverage \textbf{Jensen-Shannon divergence} (JSD) as an additional sampling criterion:
% \djkim{(more techinical explanation about the effectiveness of JSD if possible)}
\begin{equation}
    JSD(\mathbf{y}_v||\mathbf{y}_q) = (D_{KL}(\mathbf{y}_v||M)+D_{KL}(\mathbf{y}_q||M))/2, 
    \label{eqn:jsd}
\end{equation}
where  $M = (\mathbf{y}_v+\mathbf{y}_q)/2$. 
The addition of the JSD in the sampling criterion forces the sampler to find samples that have a large divergence between each single-modal output, ultimately increasing the maximum distance among all 3 points.
Therefore, our criterion can be modified by introducing an additional hyper-parameter $\beta \geq0$:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q).
    \label{eqn:addJSD}
\end{equation}
Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.
We empirically found that adding $JSD(\mathbf{y}_v||\mathbf{y}_q)$ improved the active learning performance.
The introduction and comparison with other possible approaches can be found in the supplementary material.


% \noindent\textbf{Other possible approaches.} \jwcho{(I feel it might be possible to move this to the supplementary section?)}\djkim{(If we can show VQA CP result in the main paper, let's move this to the supplementary.)}
% As the comparison target of our approach, we also test different measures for distribution discrepancy.
% In the following paragraphs, we introduce several possible candidates to measure the distances between single-modal and multi-modal answer representations.

% \textbf{\emph{(1) KL-Divergence (KLD)}} is defined as follows:
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_q) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_q)}, %= H(Y,Y_q) - H(\hat{Y}),
% \end{equation} 
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_v) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_v)}. %= H(Y,Y_v) - H(\hat{Y}),
% \end{equation} 
% %where $H(Y,Y_q)$ and $H(Y,Y_v)$ are the cross-entropies of the single-modal answers compared to multi-modal answers.
% Similar to our approach, by combining the two distance metrics via weighted sum, we have the KL-divergences:
% \begin{equation}
%     S(V,Q) = \alpha D_{KL}(\mathbf{y}||\mathbf{y}_q) + (1-\alpha) D_{KL}(\mathbf{y}||\mathbf{y}_v),
%     \label{eqn:kld}
% \end{equation}
% where $\alpha$ is a hyper-parameter that weighs between visual and question scores.
% Note that $S(V,Q)\geq0$, because KL-divergence is always non-negative.

%\textbf{\emph{(2) Mutual information (MI)}} alone can also be used as informativeness measure.
%By combining \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can compute the combined version of mutual information values:
%\begin{equation}
%    R = \alpha (H(Y_q) - H(\hat{Y})) + (1-\alpha) (H(Y_v) - H(\hat{Y})).
%\end{equation}
%%Note that $R\geq0$, because mutual information is always non-negative.



% \textbf{\emph{(2) Absolute Difference of KL-Divergence (AD-KLD)}} can also be used:
% \begin{equation}
%     S(V,Q) = |D_{KL}(\mathbf{y}||\mathbf{y}_q) - D_{KL}(\mathbf{y}||\mathbf{y}_v)|.
%     \label{eqn:ad-kld}
% \end{equation}
% Although these methods have strong theoretical backing, we empirically show that for our problem, our proposed method shows the best performance.
% among the other options.



\noindent\textbf{Acquisition function of SMEM.}
After each stage, we utilize the trained model to sample the most informative visual-question pairs with respect to $S(V,Q)$.



%\noindent\textbf{Weighted sum with entropy.}
We empirically found that adding the entropy term of the multi-modal output further improved the performance.
In particular, our final acquisition function is defined as follows:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y}),
    \label{eqn:final}
\end{equation}
where $\gamma \geq0$ is the hyper-parameter that weights between the other functions and the entropy.
Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-Distillation}
\label{sec:distillation}
\djkim{(different from previous we don't use self-distillation as regularizer. Our self-distillation doesn't effect the model training, but it is only to measure the uncertainty.)}
% \djkim{(emphasize that the effect of shaping the output distribution (and uncertainty represented therein) in a manner similar across the
% modalities/full model such that the entropy measures are more reliable to perform comparisons across modalities/full model.)}
% \jwcho{(yes)}

% The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are under the assumption that the classifiers $g_v(\cdot)$, $g_q(\cdot)$, and $g(\cdot)$ are sufficiently trained for modeling the distribution of the labeled dataset, 
% expecting that the single-modal classifiers will model the distribution similar to that of the multi-modal classifiers.
% \djkim{$\rightarrow$ expecting that single-modal classifiers will model the distribution similar to that of multi-modal classifiers especially if the visual input is conditionally independent to answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).}

The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are expecting that the single-modal classifiers will model the distribution similar to that of the multi-modal classifiers especially if the visual input is conditionally independent to answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).
In order to satisfy this assumption, 
% we need to better train 
%we need to best try to ensure 
training should enforce the $g_v(\cdot)$ and $g_q(\cdot)$ models to resemble the output distribution as close to $g(\cdot)$ as possible.
To do so, we additionally propose the self-distillation~\cite{phuong2019distillation,zhang2019your} technique to work as a regularizer~\cite{phuong2019distillation,zhang2019your}. \djkim{(we don't use it as a regularizer!)}
Our insight is that, as our acquisition function $S(V,Q)$ tries to find the sample that has a large difference between the multi-modal output (as teacher) and the single-modal output (as student), the knowledge distillation loss tries to directly minimize this difference. 
This in turn causes the easy samples to have a low $S(V,Q)$. 
In other words, if a sample gives a high $S(V,Q)$ value even after the explicit minimization of the $S(V,Q)$ score meaning the single-modal classifiers have difficulty following the output distribution of the multi-modal classifier, the sample can be thought of as a sample that is difficult or affected by both modalities and thus requires an oracle to be labeled.

Knowledge Distillation~\cite{hinton2015distilling} is defined as: training a ``student'' to follow a ``teacher'' model or representation.
Given a final output generated from a student model (in our case, $\mathbf{y}_v$ and $\mathbf{y}_q$) and an output from the teacher model (in our case, $\hat{\mathbf{y}}$), the student model learns the knowledge from the teacher's representation by forcing the student's representation to be similar to the teacher's.

% \begin{equation}
% 	\mathcal{L}_{distill}( \mathbf{y}_t,\mathbf{y}_s  ) = BCE(\mathbf{y}_t',\mathbf{y}_s'),
% 	\label{eq:loss_LWF}
% \end{equation}
% where
% \begin{equation}
% 	\\{y'}_k = \frac{(y_k)^{1/T}}{\sum_{k}^{}{(y_k)^{1/T}}}.
% 	\label{eqn:distillation}
% \end{equation}
% \djkim{(oh....eq(17) is for the distillation with CE loss, not BCE. We should remove eq(17))}
% where $y'_k$ is each individual output from the vector $\mathbf{y}$ of length $_k$ and $T$ is a hyperparameter \emph{Temperature}.
This approach suits our problem definition where the $g_v(\cdot)$ and $g_q(\cdot)$ can be student models and our $g(\cdot)$ can be the teacher model.
By adding the
% As $g_v(\cdot)$ and $g_q(\cdot)$ are only trained on classification loss,
self-distillation loss in addition to the classification loss can aid in training $g_v(\cdot)$ and $g_q(\cdot)$ to improve our acquisition function directly. We empirically prove our approach through the sampling performance gain.
% that the self-distillation loss aids in overall performance gain. 

% While the theory is sound, if the network (especially visual/question branch) is not well trained enough, we cannot guarantee that the acquisition function $S(V,Q)$ to work properly.
% Therefore, we 
% propose to 
% add knowledge distillation loss to boost the active learning performance.
% \js{(active learning performance or learning performance?)}
% \js{(self distillation enforces all branches to predict similarly?)}

% Our insight is as follows.
% Our acquisition function $S(V,Q)$ is to find the sample that has large distance between teacher and student.
% If we add the knowledge distillation loss to directly minimize this distance, the easy samples will be forced to have low $S(V,Q)$ values.
% \jwcho{(i dont know if i like this word encouraged... can we use a stronger word like force? or isit too strong?)}
% \js{(enforced?)}
% In other words, if a sample gives high value for $S(V,Q)$ even though we tried to explicitly minimize the $S(V,Q)$ score, the sample is highly likely to require oracle to label.
% In a mathematical interpretation.....\djkim{(maybe generalization bound?)}



%The loss function to train auxiliary branches is defined as 
The auxiliary single-modal branches are trained with the following loss functions:
\begin{equation}
    \mathcal{L}_v =  BCE(\mathbf{y},\mathbf{y}_v)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_v),
    \label{eqn:loss_v}
\end{equation}
\begin{equation}
    \mathcal{L}_q = BCE(\mathbf{y},\mathbf{y}_q)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_q),
    \label{eqn:loss_q}
\end{equation}
where %$\mathcal{L}_{distill}(\cdot,\cdot)$ is the knowledge distillation loss~\cite{hinton2015distilling}.
%$\theta_v$ and $\theta_q$ are the parameter of the auxiliary single-modal branches $g_v(\cdot)$ and $g_q(\cdot)$ and 
$\lambda \geq0$ is a hyper-parameter to balance the loss weights.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Theoretical Properties}

% from introduction section. lets see where we can place this
% During the training phase, our model learns multiple branch of outputs which represents single-modal output and multi-modal output respectively.
% We additionally propose to use self-distillation framework~\cite{} for better training between single-modal and muti-modal outputs for single-modal output to predict answer as correct as multi-modal branch.


Re-examining our model, the training and sampling is reminiscent of Generative Adversarial Networks~\cite{goodfellow2014generative}, where the model is trained to produce the same output between single- and multi-modal, whereas in sampling, we label the data points that show a large gap between the two outputs.
\djkim{(We shall remove this paragraph for re-submission)}
% The strategy follows the intuition that if the output probability of the multi-modal and single-modal of the active learner is different, then it means that the missing sample is informative. \jwcho{(maybe here we can refer to the figure??)}
% \js{(Mentioning mini-max is understandable but, not sure if this can claim it is doing mini-max, because there is no 2-player aspect in loss function. Infact 2-players are doing the same thing, while HOPING that training is sufficient for prediction while insufficient for sampling.)}
% Therefore, instead of simply computing the entropy of the multi-modal output, we propose to use the entropy difference, which is the mutual information, to estimate the uncertainty of the unlabeled sample.
% With the proposed framework, we demonstrate the significant performance improvements in active learning setup.
% \djkim{(Let's move this details to the method section.)}
% --------------------------------------------------------

%\subsection{Temperature in Distillation Loss}









==> Legacy/unused_3_sec_method_ICML.tex <==
% \begin{figure*}[t]
% \vspace{-2mm}
%     \centering
%     \includegraphics[width=0.9\linewidth,keepaspectratio]{Figures/architecture}
%     % \vspace{-2mm}
%     \caption{Illustration of our model architecture. Our model can be applied to any off-the-shelf VQA models (hence the area in green shows a generic VQA architecture) as our goal is to design ad hoc branches solely for the purpose of \emph{measuring uncertainty}. We add two auxiliary branches $g_v(\cdot)$ and $g_q(\cdot)$ that process the visual or question features exclusively to generate answers from a single modality. Along with the cross-entropy loss from ground truth answers, the single-modal branches are trained with knowledge distillation loss to follow the output from the multi-modal branch $g(\cdot)$.
%     % original multi-modal answer prediction branch.
%     In particular, $F(\cdot,\cdot)$ components (in black) are trained with \Eref{eqn:loss_main} while $g_v(\cdot)$ and $g_q(\cdot)$ (in red) are trained with \Eref{eqn:loss_v} and \Eref{eqn:loss_q} respectively. \
%     % djkim{(Our model can be applied to any off-the-shelf VQA models. Our work is about designing good ad hoc branches to measure (only measure) the uncertainty.)(VQA architecture itself is not a concern in our work. The goal is to make a favorable \emph{uncertainty measure} and the auxiliary branches are only for the uncertainty measure! The branches don't affect the model training.)}
%     }
%     \vspace{-2mm}
%     \label{fig:architecture}
% \end{figure*}

Our Active Learning (AL) method, Single-Modal Entropic Measure (SMEM) for Visual Question Answering consists of two key components: (1) devising an efficient and effective sample acquisition function which takes the mutual information of the individual modalities into account and (2) introducing a novel usage for the self-distillation technique for effectively training the
% individual 
auxiliary branches for a more effective sampling using SMEM.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio]{Figures/entropy_GT.pdf}
%     \caption{Illustration of how outputs from different branches can be viewed and how distance can be measured. (a) shows when all branches have similar outputs, (b) and (c) show cases where one output is similar to the main branch while the other is not. In order to get the most informative sample, our model searches for the ones that look like (d). (e) shows the legend}
%     \label{fig:entropy}
% \end{figure}





\subsection{Visual Question Answering Baseline}

Given an image $V$ and question $Q$ pair, the goal of the VQA task is to correctly predict an answer from the answer set $A\in\mathcal{A}$ (in a vectorized form, $\hat{\mathbf{y}}=F(V,Q)\in [0,1]^{|\mathcal{A}|}$), 
and we adapt one of the famous VQA state-of-the-art models as our base architecture~\cite{anderson2018bottom} where $F(\cdot,\cdot)$ is implemented via a combination of
% a deep neural network consisting of both 
convolutional and recurrent neural networks.
% \js{(Generally, any ML model but we used SOTA DL model?)}
% We adopt one of the famous V,QA state-of-the-art model~\cite{anderson2018bottom} as our base architecture.
Images and questions are mapped to feature vectors through convolutional ($f_v(\cdot)$) and recurrent ($f_q(\cdot)$) neural networks respectively (\emph{i.e.}, $\mathbf{z}_v = f_v(V), \mathbf{z}_q = f_q(Q).$).
Then following~\cite{anderson2018bottom}, $\mathbf{z}_v$ and $\mathbf{z}_q$ are combined via an additional sub-network $f_z(\cdot,\cdot)$ which includes attention and Hadamard product to generate joint representation (\emph{i.e.}, $\mathbf{z}=f_z(\mathbf{z}_v,\mathbf{z}_q)$).
Finally, $\mathbf{z}$ is fed through a fully-connected layer $g(\cdot)$ to predict $\hat{\mathbf{y}}$ (\emph{i.e.}, $\hat{\mathbf{y}}=g(\mathbf{z})$).
The goal for training the VQA model is to follow the conditional distribution of the target dataset:
% \vspace{-3mm}
\begin{equation}
    \hat{\mathbf{y}}=F(V,Q) \approx P(A|V,Q), 
\end{equation}
% \vspace{-1mm}
where $F(\cdot,\cdot)$ is the VQA model, and $P(\cdot)$ is the probability of the answer $A$ given image $V$ and question $Q$ %predicted from $F(\cdot,\cdot)$.
that we want $F(\cdot,\cdot)$ to follow.
% ($\hat{\mathbf{y}}^i = P(A=i|V,Q)$). 
Thus, the model is trained with Binary Cross-Entropy loss compared with ground truth $\mathbf{y}$:
% \djkim{(and maybe this?)}
% \vspace{-1mm}
\begin{equation}
    \mathcal{L}_{main} = BCE(\mathbf{y},\hat{\mathbf{y}}).
    \label{eqn:loss_main}
\end{equation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Learning with SMEM}%Mutual Information based Sampling Strategy}
\label{sec:method}
% \djkim{(data-points are sampled from the fixed size unlabeled pool, not by checking all the (image-question) pairs.)}
% \djkim{(we need to mention that entropy is one of the powerful method, and we are adding mutual information upon entropy which is single-modal entropy)}
% \djkim{(we would need a reason why the mutual informatino of one of the modality $I(A;V|Q)$ and $I(A;Q|V)$ matters while not considering $I(A;QV)$.)}
% \djkim{(There should be definitions of $\mathcal{D}\textsubscript{U}$ and $\mathcal{D}\textsubscript{L}$ around here.)}
% In active learning, there exists a labeled set of $\mathcal{D}\textsubscript{L}$ image/question/answer tripletS that are used for training and a pool of $\mathcal{D}\textsubscript{U}$ triplets that the trained VQA model that will be sampled from.
The goal of AL is to find the best sample acquisition function $S(V,Q)$ that assigns a high score to \emph{informative} samples.
% (\emph{e.g.}, entropy $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ by defining uncertainty as informativeness). 
In the AL setup, a labeled set $\mathcal{D}\textsubscript{L}$ is used to train a model, then after the model converges (end of a \emph{stage}), the model is used to sample from the unlabeled set $\mathcal{D}\textsubscript{U}$, then the chosen samples are given labels and added into the labeled set $\mathcal{D}\textsubscript{L}$ and removed from the unlabeled set $\mathcal{D}\textsubscript{U}$. This step is repeated several times depending on the number of stages (hyper-parameter).
There are several ways to define the informativeness of a sample. For example, entropy, which is defined as $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$, does this by defining uncertainty as informativeness.
However, in this paper, we define a novel acquisition function that takes \emph{mutual information} into account.
% Our approach exploits the multi-modality of the task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ as a sampling criteria instead of being grounded to only considering the final output representation $I(A; Y)$. 
Our approach exploits the multi-modality of this task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ individually %which are representations of image $V$ and question $Q$ respectively, 
to aid the sampling criteria instead of simply relying on $I(A;V,Q)$, the final output representation.
%, \djkim{whole input representation.}
%considering $I(A; V,Q)$ using the  %final output representation $Y$.
% Previous methods only consider the final output representation $\hat{Y}$. 
Since VQA has issues on relying 
% shown to be reliant
on a single modality and dataset bias~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, sampling from a VQA model's output representation can make the model prone to selecting outliers or heavily biased samples.
% or samples that are drastically different only in output representation space.

% in avoiding overfitting and outlier sampling. 
% \djkim{(What would be the problem of the existing approaches theoretically?)}

Intuitively, if the value of mutual information, for example $I(A;V|Q)$, is high, the variable $V$ plays an important role in predicting the answer $A$.
% In a typical off-the-shelf model, directly computing the mutual information of individual modalities is difficult.
% As it is difficult to compute the mutual information of individual modalities of typical off-the-shelf models, we 
% In order to measure the uncertainty of each single-modal input, we add 
% In contrast, we add 
In order to compute mutual information of individual modalities, we
add auxiliary independent classification branches, as shown in \Fref{fig:architecture}, that predict the answer exclusively from individual visual and question features.
% to measure mutual information and the informativeness of each modality.
% \djkim{($\leftarrow$we should clarify these sentences. Our ultimate goal is to measure the uncertainty, and in order to implement that according to our formulation, we need to add additional single-modal branches.)}
The branches are detached from the model, 
% meaning the gradients of the branches do not flow into the main model, 
meaning that the presence of the branches have no effect on the main model performance and \emph{does not act as a regularizer} of any kind.
The branches are trained with cross-entropy loss with ground truth answers so that the output answer probability can approximate the conditional distribution of answers given cues such that $\mathbf{y}_v=g_v(\mathbf{z}_v) \approx P(A|V)$ for visual and $\mathbf{y}_q=g_q(\mathbf{z}_q) \approx P(A|Q)$ for question, note however that the answer predictions from the single-modal classifiers do not have to be accurate as their purpose is only to measure uncertainty.
% \djkim{(note that the answer prediction from the single-modal classifiers don't have to be accurate because these outputs are only used for measuring uncertainty.)}

As we try to measure the informativeness of a given input visual question pair $(V,Q)$ through a given acquisition function $S(V,Q)$, we can intuitively expect that the input cue $V$ or $Q$ may contain a considerable amount of information if the single-modal outputs $\mathbf{y}_v$ and $\mathbf{y}_q$ are considerably different from $\hat{\mathbf{y}}$. 
%In addition, as entropy is a powerful metric for AL, where entropy is ($H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$). 
By measuring the uncertainty of the model predictions, we devise a novel acquisition function based on entropy that takes into account the relation between the single-modal and multi-modal answer representations and show significant performance gains.
% \djkim{(we can say that simple entropy is only for uncertainty, ours is uncertainty+mutual information!)}\jwcho{(got it!)}
% Since entropy is the most famous metric for AL, based on the core idea of entropy, we introduce a new metric that outperforms it. 
% \djkim{Entropy is the most famous metric for AL, but we introduce better way than the Entropy}


\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=.8\linewidth,keepaspectratio]{Figures/jensenshanon.pdf}
    \vspace{-2mm}
    \caption{
    Illustration of differences of the outputs from $g(\cdot)$, $g_v(\cdot)$, and $g_q(\cdot)$.
    % SMEM
    % , which measures the difference between main output and the single-modal outputs, we
    % gives a higher score to (a) than (b) in the sampling stage as it measures the difference between the main output and single-modal outputs.
    Since we can intuitively expect (c) to be more informative than (b), we propose to add Jensen-Shannon divergence between the two single-modal outputs in order to account for the discrepancies between single-modal outputs. Ultimately, SMEM gives a higher score to (a) than (b) in the sampling stage.}
    \vspace{-2mm}
    \label{fig:jensenshanon}
\end{figure*}



% \begin{equation}
%     Y_v=g_v(z_v) \approx p_\theta(y|v).
% \end{equation}

% Likewise, we can also define answer prediction only from a question feature:
% \begin{equation}
%     Y_q=g_q(z_q) \approx p_\theta(y|q).
% \end{equation}


% As our goal in this work is to leverage the three cues, $Y_v$, $Y_q$, and $\hat{Y}$ to effectively measure the informativeness of the given input visual-question pair $(V,Q)$ through a proper acquisition function $S(V,Q)$.
% Intuitively, if the single-modal outputs $Y_v$ and $Y_q$ are different enough from a multi-modal output $\hat{Y}$, one can expect the input cue $V$ or $Q$ may contain a considerable amount of information in order to predict a correct answer. In this regard, we devise a novel acquisition function that take the relation between the single-modal and multi-modal answer representations into account. \jwcho{(i really feel this paragraph and the one from line 111~119 redundant, but not, so must be changed... i cant think of a way yet)}

% \djkim{(possible tackle? other multi-modal tasks? maybe our idea is based on classification task)}


\noindent\textbf{Single-Modal Entropic Measure (SMEM).} %(our name???)
% \djkim{(we should emphasize more that none of these methods effect the model training. All these methods are only for measuring the uncertainty.)}
Our goal is to find the training data points that have high mutual information %with output answers 
$I(A;V|Q)$ and $I(A;Q|V)$, and according to the property of mutual information, it can be decomposed into the difference of entropies:
\begin{equation}
    I(A;V|Q) = H(A|Q) - H(A|V,Q) \approx H(Y_q) - H(\hat{Y}),
    \label{eqn:MI_Q}
\end{equation}
\vspace{-2mm}
\begin{equation}
    I(A;Q|V) = H(A|V) - H(A|V,Q) \approx H(Y_v) - H(\hat{Y}),
    \label{eqn:MI_V}
\end{equation}
where $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ 
is the entropy of a given distribution. 
As shown in the equations above, we see that mutual information is easily computed from the entropy values of the single-modal and multi-modal outputs.
This is from the assumption that $H(A|V,Q)$, $H(A|Q)$, and $H(A|V)$ are modeled with $H(\hat{Y})$, $H(Y_q)$, and $H(Y_v)$ respectively (\ie~$H(A|V,Q) \approx H(\hat{Y})$, $H(A|Q)\approx H(Y_q)$, $ H(A|V)\approx H(Y_v)$).

% On the other hand, if we modify \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can derive the equations:

%On the other hand, 
Similarly,
rearranging \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we get:
\begin{equation}
    H(Y_q) \approx H(A|Q) = I(A;V|Q) + H(A|V,Q),
    \label{eqn:single-Q}
\end{equation}
\vspace{-5mm}
\begin{equation}
    H(Y_v) \approx H(A|V) = I(A;Q|V) + H(A|V,Q),
    \label{eqn:single-V}
\end{equation}
where $H(Y_q)=-\sum_{i} \mathbf{y}_q^i\log \mathbf{y}_q^i$  and $H(Y_v)=-\sum_{i} \mathbf{y}_v^i\log \mathbf{y}_v^i$ . From \Eref{eqn:single-Q} and \Eref{eqn:single-V}, we can see that the entropy of the single-modal output is the sum of the mutual information and the entropy of the multi-modal output, and we want both values to be high when sampling.
% which are both we want to find samples with high values of.
In other words,
% one can find training samples in terms of
both uncertainty and informativeness can be measured by simply computing the \emph{entropy of the single-modal output}.

In this regard, we propose an informativeness value to be the weighted sum of the single-modal entropy for image and question, \textbf{SMEM}:
%\djkim{(notation overload in $S(V,Q)$. maybe use different notation?)}
% \vspace{-3mm}
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v), 
    \label{eqn:student}
\end{equation}
where $0\leq \alpha \leq 1$  is a hyper-parameter that weights the relative importance of visual and question scores.
Note that $0 \leq S(V,Q)\leq \log |\mathcal{A}|$, because $0 \leq H(\cdot) \leq \log |\mathcal{A}|$.




In addition, we also conjecture that as the information of the
% important information is not only information about the 
relationships between all single-modal and multi-modal outputs are important, the information of the relationship between the single-modal outputs is just as important.
As in \Fref{fig:jensenshanon} (b) and (c), even though the distance between single-modal outputs and the multi-modal output is fixed, the relationship between the three distributions can differ due to the distance between single-modal outputs.
If we only leverage the distance between the single-modal and multi-modal outputs, (b) and (c) would give the same score, however, we can intuitively understand that (c) is more uncertain than (b) as the distance between the single-modal outputs is much greater.
In order to measure this distance between the single-modal outputs on top of the distances between the single-modal and multi-modal outputs, we propose to also leverage \textbf{Jensen-Shannon divergence} (JSD) as an additional sampling criterion:
% \djkim{(more techinical explanation about the effectiveness of JSD if possible)}
\begin{equation}
    JSD(\mathbf{y}_v||\mathbf{y}_q) = (D_{KL}(\mathbf{y}_v||M)+D_{KL}(\mathbf{y}_q||M))/2, 
    \label{eqn:jsd}
\end{equation}
where  $M = (\mathbf{y}_v+\mathbf{y}_q)/2$. 
The addition of JSD in the sampling criterion forces the sampler to find samples with a large divergence between single-modal outputs, ultimately increasing the maximum distance among all three points.


\noindent\textbf{Final Acquisition function of SMEM.} 
% After each AL stage, we utilize the trained model to sample the most informative visual-question pairs with respect to $S(V,Q)$. 
Therefore, we decide on our final sampling criterion as:
% modified by introducing an additional hyper-parameter $\beta \geq0$:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q),
    \label{eqn:addJSD}
\end{equation}
where we introduce an additional weight hyper-parameter $\beta \geq0$.
Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.
% We empirically found that adding $JSD(\mathbf{y}_v||\mathbf{y}_q)$ improved the active learning performance. \jwcho{(maybe not the best addition)}
The introduction and comparison with other possible approaches can be found in the supplementary material.


% \noindent\textbf{Other possible approaches.} \jwcho{(I feel it might be possible to move this to the supplementary section?)}\djkim{(If we can show VQA CP result in the main paper, let's move this to the supplementary.)}
% As the comparison target of our approach, we also test different measures for distribution discrepancy.
% In the following paragraphs, we introduce several possible candidates to measure the distances between single-modal and multi-modal answer representations.

% \textbf{\emph{(1) KL-Divergence (KLD)}} is defined as follows:
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_q) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_q)}, %= H(Y,Y_q) - H(\hat{Y}),
% \end{equation} 
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_v) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_v)}. %= H(Y,Y_v) - H(\hat{Y}),
% \end{equation} 
% %where $H(Y,Y_q)$ and $H(Y,Y_v)$ are the cross-entropies of the single-modal answers compared to multi-modal answers.
% Similar to our approach, by combining the two distance metrics via weighted sum, we have the KL-divergences:
% \begin{equation}
%     S(V,Q) = \alpha D_{KL}(\mathbf{y}||\mathbf{y}_q) + (1-\alpha) D_{KL}(\mathbf{y}||\mathbf{y}_v),
%     \label{eqn:kld}
% \end{equation}
% where $\alpha$ is a hyper-parameter that weighs between visual and question scores.
% Note that $S(V,Q)\geq0$, because KL-divergence is always non-negative.

%\textbf{\emph{(2) Mutual information (MI)}} alone can also be used as informativeness measure.
%By combining \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can compute the combined version of mutual information values:
%\begin{equation}
%    R = \alpha (H(Y_q) - H(\hat{Y})) + (1-\alpha) (H(Y_v) - H(\hat{Y})).
%\end{equation}
%%Note that $R\geq0$, because mutual information is always non-negative.



% \textbf{\emph{(2) Absolute Difference of KL-Divergence (AD-KLD)}} can also be used:
% \begin{equation}
%     S(V,Q) = |D_{KL}(\mathbf{y}||\mathbf{y}_q) - D_{KL}(\mathbf{y}||\mathbf{y}_v)|.
%     \label{eqn:ad-kld}
% \end{equation}
% Although these methods have strong theoretical backing, we empirically show that for our problem, our proposed method shows the best performance.
% among the other options.



% \noindent\textbf{Acquisition function of SMEM.}

We also empirically found that adding the entropy term of the multi-modal output further improved the performance: $S(V,Q)+ \gamma H(\hat{Y}),$
where $\gamma \geq0$ is the hyper-parameter that weights between $S(V,Q)$ and the entropy.
Note that $S(V,Q)+ \gamma H(\hat{Y})\geq0$, because both $S(V,Q)$ and $H(\hat{Y})$ are always non-negative.




%\noindent\textbf{Weighted sum with entropy.}
% We empirically found that adding the entropy term of the multi-modal output further improved the performance.
% In particular, our final acquisition function is defined as follows:
% \vspace{-3mm}
% \begin{equation}
%     S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y}),
%     \label{eqn:final}
% \end{equation}
% where $\gamma \geq0$ is the hyper-parameter that weights between the other functions and the entropy.
% Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training Auxiliary Branches with Self-Distillation}
\label{sec:distillation}
% \djkim{(different from previous we don't use self-distillation as regularizer. Our self-distillation doesn't effect the model training, but it is only to measure the uncertainty.)}
% \djkim{(emphasize that the effect of shaping the output distribution (and uncertainty represented therein) in a manner similar across the
% modalities/full model such that the entropy measures are more reliable to perform comparisons across modalities/full model.)}
% \jwcho{(yes)}

% The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are under the assumption that the classifiers $g_v(\cdot)$, $g_q(\cdot)$, and $g(\cdot)$ are sufficiently trained for modeling the distribution of the labeled dataset, 
% expecting that the single-modal classifiers will model the distribution similar to that of the multi-modal classifiers.
% \djkim{$\rightarrow$ expecting that single-modal classifiers will model the distribution similar to that of multi-modal classifiers especially if the visual input is conditionally independent to answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).}

\Eref{eqn:single-Q} and \Eref{eqn:single-V} are set on the basis that the single-modal classifiers' output distribution will be similar to that of the multi-modal classifier's especially if the visual input is conditionally independent on answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).
In order to satisfy this assumption, 
% we need to better train 
%we need to best try to ensure 
$g_v(\cdot)$ and $g_q(\cdot)$'s outputs distribution should be trained to resemble $g(\cdot)$'s output distribution as closely as possible.
To do so, we additionally utilize the self-distillation technique to explicitly train the auxiliary single-modal classifiers to mimic the ``main'' classifier's distribution~\cite{phuong2019distillation,zhang2019your}. Note that as the single-modal classifiers are detached, this self-distillation technique has no effect on the performance of the model and \emph{does not act as a regularizer}.
Our insight is, our acquisition function $S(V,Q)$ tries to find the sample that has a large difference between the multi-modal output (as teacher) and the single-modal output (as student), and the knowledge distillation loss tries to directly minimize this difference. 
This causes the easy samples to have a low $S(V,Q)$. 
In other words, if a sample gives a high $S(V,Q)$ value even after the explicit minimization of the $S(V,Q)$ score meaning the single-modal classifiers have difficulty following the output distribution of the multi-modal classifier, the sample can be thought of as a sample that is difficult or affected by both modalities and thus requires an oracle to be labeled.

Knowledge Distillation~\cite{hinton2015distilling} is defined as: training a ``student'' to follow a ``teacher'' model or representation.
Given a final output generated from a student model (in our case, $\mathbf{y}_v$ and $\mathbf{y}_q$) and an output from the teacher model (in our case, $\hat{\mathbf{y}}$), the student model learns the knowledge from the teacher's representation by forcing the student's representation to be similar to the teacher's.
% In our approach, we define $g_v(\cdot)$ and $g_q(\cdot)$ as student models while $g(\cdot)$ is defined as the teacher. 
To this end, we add the self-distillation loss in addition to the classification loss in training $g_v(\cdot)$ and $g_q(\cdot)$ to improve our acquisition function directly. 
% We empirically prove our approach through the sampling performance gain.
% that the self-distillation loss aids in overall performance gain. 
The auxiliary single-modal branches are trained with the following loss functions:
\begin{equation}
    \mathcal{L}_v =  BCE(\mathbf{y},\mathbf{y}_v)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_v),
    \label{eqn:loss_v}
\end{equation}
% \vspace{-4mm}
\begin{equation}
    \mathcal{L}_q = BCE(\mathbf{y},\mathbf{y}_q)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_q),
    \label{eqn:loss_q}
\end{equation}
where %$\mathcal{L}_{distill}(\cdot,\cdot)$ is the knowledge distillation loss~\cite{hinton2015distilling}.
%$\theta_v$ and $\theta_q$ are the parameter of the auxiliary single-modal branches $g_v(\cdot)$ and $g_q(\cdot)$ and 
$\lambda \geq0$ is a loss weight hyper-parameter.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Theoretical Properties}

% from introduction section. lets see where we can place this
% During the training phase, our model learns multiple branch of outputs which represents single-modal output and multi-modal output respectively.
% We additionally propose to use self-distillation framework~\cite{} for better training between single-modal and muti-modal outputs for single-modal output to predict answer as correct as multi-modal branch.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Re-examining our model, the training and sampling is reminiscent of Generative Adversarial Networks~\cite{goodfellow2014generative}, where the model is trained to produce the same output between single- and multi-modal, whereas in sampling, we label the data points that show a large gap between the two outputs.
% \djkim{(We shall remove this paragraph for re-submission)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% The strategy follows the intuition that if the output probability of the multi-modal and single-modal of the active learner is different, then it means that the missing sample is informative. \jwcho{(maybe here we can refer to the figure??)}
% \js{(Mentioning mini-max is understandable but, not sure if this can claim it is doing mini-max, because there is no 2-player aspect in loss function. Infact 2-players are doing the same thing, while HOPING that training is sufficient for prediction while insufficient for sampling.)}
% Therefore, instead of simply computing the entropy of the multi-modal output, we propose to use the entropy difference, which is the mutual information, to estimate the uncertainty of the unlabeled sample.
% With the proposed framework, we demonstrate the significant performance improvements in active learning setup.
% \djkim{(Let's move this details to the method section.)}
% --------------------------------------------------------

%\subsection{Temperature in Distillation Loss}




==> Legacy/unused_3_sec_method_humantech.tex <==


Our Active Learning (AL) method, Single-Modal Entropic Measure (SMEM) for Visual Question Answering consists of two key components: (1) devising an efficient and effective sample acquisition function which takes the mutual information of the individual modalities into account and (2) introducing a novel usage for the self-distillation technique for effectively training the individual auxiliary branches for better sampling with SMEM.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio]{Figures/entropy_GT.pdf}
%     \caption{Illustration of how outputs from different branches can be viewed and how distance can be measured. (a) shows when all branches have similar outputs, (b) and (c) show cases where one output is similar to the main branch while the other is not. In order to get the most informative sample, our model searches for the ones that look like (d). (e) shows the legend}
%     \label{fig:entropy}
% \end{figure}





\subsection{Visual Question Answering Baseline}

Given an image $V$ and question $Q$ pair, the goal of the VQA task is to correctly predict an answer from the answer set $A\in\mathcal{A}$ (in a vectorized form, $\hat{\mathbf{y}}=F(V,Q)\in [0,1]^{|\mathcal{A}|}$), 
and we adapt one of the famous VQA state-of-the-art models as our base architecture~\cite{anderson2018bottom} where $F(\cdot,\cdot)$ is implemented via a combination of
% a deep neural network consisting of both 
convolutional and recurrent neural networks.
% \js{(Generally, any ML model but we used SOTA DL model?)}
% We adopt one of the famous V,QA state-of-the-art model~\cite{anderson2018bottom} as our base architecture.
Images and questions are mapped to feature vectors through convolutional ($f_v(\cdot)$) and recurrent ($f_q(\cdot)$) neural networks respectively (\emph{i.e.}, $\mathbf{z}_v = f_v(V), \mathbf{z}_q = f_q(Q).$).
Then following~\cite{anderson2018bottom}, $\mathbf{z}_v$ and $\mathbf{z}_q$ are combined via an additional sub-network $f_z(\cdot,\cdot)$ which includes attention and Hadamard product to generate joint representation (\emph{i.e.}, $\mathbf{z}=f_z(\mathbf{z}_v,\mathbf{z}_q)$).
Finally, $\mathbf{z}$ is fed through a fully-connected layer $g(\cdot)$ to predict $\hat{\mathbf{y}}$ (\emph{i.e.}, $\hat{\mathbf{y}}=g(\mathbf{z})$).
The goal for training the VQA model is to follow the conditional distribution of the target dataset:
\begin{equation}
    \hat{\mathbf{y}}=F(V,Q) \approx P(A|V,Q), 
\end{equation}
where $F(\cdot,\cdot)$ is the VQA model, and $P(\cdot)$ is the probability of the answer $A$ given image $V$ and question $Q$ %predicted from $F(\cdot,\cdot)$.
that we want $F(\cdot,\cdot)$ to follow.
% ($\hat{\mathbf{y}}^i = P(A=i|V,Q)$). 
Thus, the model is trained with Binary Cross-Entropy loss compared with ground truth $\mathbf{y}$:
% \djkim{(and maybe this?)}
\begin{equation}
    \mathcal{L}_{main} = BCE(\mathbf{y},\hat{\mathbf{y}}).
    \label{eqn:loss_main}
\end{equation}



\begin{figure*}[t]
\vspace{-2mm}
    \centering
    \includegraphics[width=.8\linewidth,keepaspectratio]{Figures/jensenshanon.pdf}
    \vspace{0mm}
    \caption{
    Illustration of differences of the outputs from $g(\cdot)$, $g_v(\cdot)$, and $g_q(\cdot)$.
    In our SMEM measure, which measures the difference between main output and the single-modal outputs, we give a higher score to (a) than (b) in the sampling stage. However, we can also intuitively expect (c) to be more informative than (b). Thus, we also propose to add Jensen-Shannon divergence between the two single-modal outputs in order to account for the discrepancies between single-modal outputs.}
    \vspace{-2mm}
    \label{fig:jensenshanon}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Learning with SMEM}%Mutual Information based Sampling Strategy}
\label{sec:method}
% \djkim{(data-points are sampled from the fixed size unlabeled pool, not by checking all the (image-question) pairs.)}
% \djkim{(we need to mention that entropy is one of the powerful method, and we are adding mutual information upon entropy which is single-modal entropy)}
% \djkim{(we would need a reason why the mutual informatino of one of the modality $I(A;V|Q)$ and $I(A;Q|V)$ matters while not considering $I(A;QV)$.)}
% \djkim{(There should be definitions of $\mathcal{D}\textsubscript{U}$ and $\mathcal{D}\textsubscript{L}$ around here.)}
% In active learning, there exists a labeled set of $\mathcal{D}\textsubscript{L}$ image/question/answer tripletS that are used for training and a pool of $\mathcal{D}\textsubscript{U}$ triplets that the trained VQA model that will be sampled from.
The goal of AL is to find the best sample acquisition function $S(V,Q)$ that assigns a high score to \emph{informative} samples.
% (\emph{e.g.}, entropy $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ by defining uncertainty as informativeness). 
In the AL setup, a labeled set $\mathcal{D}\textsubscript{L}$ is used to train a model, then after the model converges (end of a \emph{stage}), the model is used to sample from the unlabeled set $\mathcal{D}\textsubscript{U}$, then the chosen samples are given labels and added into the labeled set $\mathcal{D}\textsubscript{L}$ and removed from the unlabeled set $\mathcal{D}\textsubscript{U}$. This step is repeated several times depending on the number of stages (hyper-parameter).
There are several ways to define the informativeness of a sample. For example, entropy, which is defined as $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$, does this by defining uncertainty as informativeness.
However, in this paper, we define a novel acquisition function that takes \emph{mutual information} into account.
% Our approach exploits the multi-modality of the task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ as a sampling criteria instead of being grounded to only considering the final output representation $I(A; Y)$. 
Our approach exploits the multi-modality of this task and directly measures the mutual information $I(A;V|Q)$ and $I(A;Q|V)$ individually %which are representations of image $V$ and question $Q$ respectively, 
to aid the sampling criteria instead of simply relying on $I(A;V,Q)$, the final output representation.
%, \djkim{whole input representation.}
%considering $I(A; V,Q)$ using the  %final output representation $Y$.
% Previous methods only consider the final output representation $\hat{Y}$. 
Since VQA has issues on relying 
% shown to be reliant
on a single modality and dataset bias~\cite{agrawal2018don,cadene2019rubi,goyal2017making,manjunatha2018explicitbiasvqa,ramakrishnan2018overcomingpriors}, sampling from a VQA model's output representation can make the model prone to selecting outliers or samples that are drastically different only in output representation space.
% in avoiding overfitting and outlier sampling. 
% \djkim{(What would be the problem of the existing approaches theoretically?)}

Intuitively, if the value of mutual information, for example $I(A;V|Q)$, is high, the variable $V$ plays an important role in predicting the answer $A$.
In a typical off-the-shelf model, directly computing the mutual information of individual modalities is difficult.
% To this end, we add additional ad hoc branches to compute the mutual information which is described in the following subsection in detail. 
% As shown in \Fref{fig:architecture}, 
In order to measure the uncertainty of each single-modal input, we add 
% In contrast, we add 
independent classification branches, as shown in \Fref{fig:architecture}, that predict the answer exclusively from visual and question single features.
% to measure mutual information and the informativeness of each modality.
% \djkim{($\leftarrow$we should clarify these sentences. Our ultimate goal is to measure the uncertainty, and in order to implement that according to our formulation, we need to add additional single-modal branches.)}
The branches are detached from the model, meaning the gradients of the branches are cut off from the main model, which in turn means that the presence of the branch additions have no effect on the main model performance, and is trained with cross-entropy loss with ground truth answers so that the output answer probability can approximate the conditional distribution of answers given cues such that $\mathbf{y}_v=g_v(\mathbf{z}_v) \approx P(A|V)$ for visual and $\mathbf{y}_q=g_q(\mathbf{z}_q) \approx P(A|Q)$ for question, note however that the answer predictions from the single-modal classifiers do not have to be accurate as their purpose is only to measure uncertainty.
% \djkim{(note that the answer prediction from the single-modal classifiers don't have to be accurate because these outputs are only used for measuring uncertainty.)}

As we try to measure the informativeness of a given input visual question pair $(V,Q)$ through a given acquisition function $S(V,Q)$, we can intuitively expect that the input cue $V$ or $Q$ may contain a considerable amount of information if the single-modal outputs $\mathbf{y}_v$ and $\mathbf{y}_q$ are considerably different from $\hat{\mathbf{y}}$. 
%In addition, as entropy is a powerful metric for AL, where entropy is ($H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$). 
By measuring the uncertainty of the model predictions, we devise a novel acquisition function based on entropy that takes into account the relation between the single-modal and multi-modal answer representations and show significant performance gains.
% \djkim{(we can say that simple entropy is only for uncertainty, ours is uncertainty+mutual information!)}\jwcho{(got it!)}
% Since entropy is the most famous metric for AL, based on the core idea of entropy, we introduce a new metric that outperforms it. 
% \djkim{Entropy is the most famous metric for AL, but we introduce better way than the Entropy}



% \begin{equation}
%     Y_v=g_v(z_v) \approx p_\theta(y|v).
% \end{equation}

% Likewise, we can also define answer prediction only from a question feature:
% \begin{equation}
%     Y_q=g_q(z_q) \approx p_\theta(y|q).
% \end{equation}


% As our goal in this work is to leverage the three cues, $Y_v$, $Y_q$, and $\hat{Y}$ to effectively measure the informativeness of the given input visual-question pair $(V,Q)$ through a proper acquisition function $S(V,Q)$.
% Intuitively, if the single-modal outputs $Y_v$ and $Y_q$ are different enough from a multi-modal output $\hat{Y}$, one can expect the input cue $V$ or $Q$ may contain a considerable amount of information in order to predict a correct answer. In this regard, we devise a novel acquisition function that take the relation between the single-modal and multi-modal answer representations into account. \jwcho{(i really feel this paragraph and the one from line 111~119 redundant, but not, so must be changed... i cant think of a way yet)}

% \djkim{(possible tackle? other multi-modal tasks? maybe our idea is based on classification task)}


\noindent\textbf{Single-Modal Entropic Measure (SMEM).} %(our name???)
% \djkim{(we should emphasize more that none of these methods effect the model training. All these methods are only for measuring the uncertainty.)}
Our goal is to find the training data points that have high mutual information %with output answers 
$I(A;V|Q)$ and $I(A;Q|V)$, and according to the property of mutual information, it can be decomposed into the difference of entropies:
\begin{equation}
    I(A;V|Q) = H(A|Q) - H(A|V,Q) \approx H(Y_q) - H(\hat{Y}),
    \label{eqn:MI_Q}
\end{equation}
\begin{equation}
    I(A;Q|V) = H(A|V) - H(A|V,Q) \approx H(Y_v) - H(\hat{Y}),
    \label{eqn:MI_V}
\end{equation}
where $H(\hat{Y})=-\sum_{i} \hat{\mathbf{y}}^i\log \hat{\mathbf{y}}^i$ 
is the entropy of a given distribution. 
As shown in the equations above, we see that mutual information is easily computed from the entropy values of the single-modal and multi-modal outputs.
This is from the assumption that $H(A|V,Q)$, $H(A|Q)$, and $H(A|V)$ are modeled with $H(\hat{Y})$, $H(Y_q)$, and $H(Y_v)$ respectively (\ie~$H(A|V,Q) \approx H(\hat{Y})$, $H(A|Q)\approx H(Y_q)$, $ H(A|V)\approx H(Y_v)$).

% On the other hand, if we modify \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can derive the equations:

%On the other hand, 
Similarly,
rearranging \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we get:
\begin{equation}
    H(Y_q) \approx H(A|Q) = I(A;V|Q) + H(A|V,Q),
    \label{eqn:single-Q}
\end{equation}
\begin{equation}
    H(Y_v) \approx H(A|V) = I(A;Q|V) + H(A|V,Q),
    \label{eqn:single-V}
\end{equation}
where $H(Y_q)=-\sum_{i} \mathbf{y}_q^i\log \mathbf{y}_q^i$  and $H(Y_v)=-\sum_{i} \mathbf{y}_v^i\log \mathbf{y}_v^i$ . From \Eref{eqn:single-Q} and \Eref{eqn:single-V}, we can see that the entropy of the single-modal output is the sum of the mutual information and the entropy of the multi-modal output, and we want both values to be high when sampling.
% which are both we want to find samples with high values of.
In other words,
% one can find training samples in terms of
both uncertainty and informativeness can be measured by simply computing the \emph{entropy of the single-modal output}.

In this regard, we propose an informativeness value to be the weighted sum of the single-modal entropy for image and question, \textbf{SMEM}:
%\djkim{(notation overload in $S(V,Q)$. maybe use different notation?)}
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v), 
    \label{eqn:student}
\end{equation}
where $0\leq \alpha \leq 1$  is a hyper-parameter that weights the relative importance of visual and question scores.
Note that $0 \leq S(V,Q)\leq \log |\mathcal{A}|$, because $0 \leq H(\cdot) \leq \log |\mathcal{A}|$.





In addition, we also conjecture that as the information of the
% important information is not only information about the 
relationships between all single-modal and multi-modal outputs are important, the information of the relationship between the single-modal outputs is just as important.
As in \Fref{fig:jensenshanon} (b) and (c), even though the distance between single-modal outputs and the multi-modal output is fixed, the relationship between the three distributions can differ due to the distance between single-modal outputs.
If we only leverage the distance between the single-modal and multi-modal outputs, (b) and (c) would give the same score, however, we can intuitively understand that (c) is more uncertain than (b) as the distance between the single-modal outputs is much greater.
In order to measure this distance between the single-modal outputs on top of the distances between the single-modal and multi-modal outputs, we propose to also leverage \textbf{Jensen-Shannon divergence} (JSD) as an additional sampling criterion:
% \djkim{(more techinical explanation about the effectiveness of JSD if possible)}
\begin{equation}
    JSD(\mathbf{y}_v||\mathbf{y}_q) = (D_{KL}(\mathbf{y}_v||M)+D_{KL}(\mathbf{y}_q||M))/2, 
    \label{eqn:jsd}
\end{equation}
where  $M = (\mathbf{y}_v+\mathbf{y}_q)/2$. 
The addition of the JSD in the sampling criterion forces the sampler to find samples that have a large divergence between each single-modal output, ultimately increasing the maximum distance among all 3 points.
Therefore, our criterion can be modified by introducing an additional hyper-parameter $\beta \geq0$:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q).
    \label{eqn:addJSD}
\end{equation}
Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.
We empirically found that adding $JSD(\mathbf{y}_v||\mathbf{y}_q)$ improved the active learning performance.
The introduction and comparison with other possible approaches can be found in the supplementary material.


% \noindent\textbf{Other possible approaches.} \jwcho{(I feel it might be possible to move this to the supplementary section?)}\djkim{(If we can show VQA CP result in the main paper, let's move this to the supplementary.)}
% As the comparison target of our approach, we also test different measures for distribution discrepancy.
% In the following paragraphs, we introduce several possible candidates to measure the distances between single-modal and multi-modal answer representations.

% \textbf{\emph{(1) KL-Divergence (KLD)}} is defined as follows:
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_q) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_q)}, %= H(Y,Y_q) - H(\hat{Y}),
% \end{equation} 
% \begin{equation}
%     D_{KL}(\mathbf{y}||\mathbf{y}_v) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_v)}. %= H(Y,Y_v) - H(\hat{Y}),
% \end{equation} 
% %where $H(Y,Y_q)$ and $H(Y,Y_v)$ are the cross-entropies of the single-modal answers compared to multi-modal answers.
% Similar to our approach, by combining the two distance metrics via weighted sum, we have the KL-divergences:
% \begin{equation}
%     S(V,Q) = \alpha D_{KL}(\mathbf{y}||\mathbf{y}_q) + (1-\alpha) D_{KL}(\mathbf{y}||\mathbf{y}_v),
%     \label{eqn:kld}
% \end{equation}
% where $\alpha$ is a hyper-parameter that weighs between visual and question scores.
% Note that $S(V,Q)\geq0$, because KL-divergence is always non-negative.

%\textbf{\emph{(2) Mutual information (MI)}} alone can also be used as informativeness measure.
%By combining \Eref{eqn:MI_Q} and \Eref{eqn:MI_V}, we can compute the combined version of mutual information values:
%\begin{equation}
%    R = \alpha (H(Y_q) - H(\hat{Y})) + (1-\alpha) (H(Y_v) - H(\hat{Y})).
%\end{equation}
%%Note that $R\geq0$, because mutual information is always non-negative.



% \textbf{\emph{(2) Absolute Difference of KL-Divergence (AD-KLD)}} can also be used:
% \begin{equation}
%     S(V,Q) = |D_{KL}(\mathbf{y}||\mathbf{y}_q) - D_{KL}(\mathbf{y}||\mathbf{y}_v)|.
%     \label{eqn:ad-kld}
% \end{equation}
% Although these methods have strong theoretical backing, we empirically show that for our problem, our proposed method shows the best performance.
% among the other options.



\noindent\textbf{Acquisition function of SMEM.}
After each stage, we utilize the trained model to sample the most informative visual-question pairs with respect to $S(V,Q)$.



%\noindent\textbf{Weighted sum with entropy.}
We empirically found that adding the entropy term of the multi-modal output further improved the performance.
In particular, our final acquisition function is defined as follows:
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y}),
    \label{eqn:final}
\end{equation}
where $\gamma \geq0$ is the hyper-parameter that weights between the other functions and the entropy.
Note that $S(V,Q)\geq0$, because both entropy and JSD are always non-negative.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[t]
\SetAlgoLined
\KwIn{Labeled pool $\mathcal{D}\textsubscript{L}$, Initialized models $g_v(\cdot), g_q(\cdot),\text{ and }F(\cdot,\cdot)$ with parameters $\theta_v$,$\theta_q$,\text{ and }$\theta$ respectively}
\KwIn{Hyper-parameters : learning rate $\eta$, maximum number of epoches $MaxEpoch$}
\KwOut{$g_v(\cdot), g_q(\cdot),\text{ and }F(\cdot,\cdot)$ with trained $\theta_v$,$\theta_q$,\text{ and }$\theta$}
\Begin{
    \For{$e=1$ to MaxEpoch}{
    sample $(X,Y)\in\mathcal{D}\textsubscript{L}$\;
    Compute $\mathcal{L}_{main}$\;
    Compute $\mathcal{L}_v$\;
    Compute $\mathcal{L}_q$\;
    Update the model parameters:\\
    $\theta \leftarrow \theta - \eta \nabla \mathcal{L}_{main}$\\
    $\theta_v \leftarrow \theta_v - \eta \nabla \mathcal{L}_{v}$\\
    $\theta_q \leftarrow \theta_q - \eta \nabla \mathcal{L}_{q}$\\
    }
}
\caption{Training Our Model with Self-distillation}
\label{alg:training}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-Distillation}
\label{sec:distillation}
% \djkim{(different from previous we don't use self-distillation as regularizer. Our self-distillation doesn't effect the model training, but it is only to measure the uncertainty.)}
% \djkim{(emphasize that the effect of shaping the output distribution (and uncertainty represented therein) in a manner similar across the
% modalities/full model such that the entropy measures are more reliable to perform comparisons across modalities/full model.)}
% \jwcho{(yes)}

% The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are under the assumption that the classifiers $g_v(\cdot)$, $g_q(\cdot)$, and $g(\cdot)$ are sufficiently trained for modeling the distribution of the labeled dataset, 
% expecting that the single-modal classifiers will model the distribution similar to that of the multi-modal classifiers.
% \djkim{$\rightarrow$ expecting that single-modal classifiers will model the distribution similar to that of multi-modal classifiers especially if the visual input is conditionally independent to answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).}

The \Eref{eqn:single-Q} and \Eref{eqn:single-V} are expecting that the single-modal classifiers will model the distribution similar to that of the multi-modal classifiers especially if the visual input is conditionally independent on answers given a question (\emph{i.e.}, $P(A|VQ)\approx P(A|Q)$) or vice versa (\emph{i.e.}, $P(A|VQ)\approx P(A|V)$).
In order to satisfy this assumption, 
% we need to better train 
%we need to best try to ensure 
training should enforce the $g_v(\cdot)$ and $g_q(\cdot)$ models to resemble the output distribution as close to $g(\cdot)$ as possible.
To do so, we additionally propose the self-distillation~\cite{phuong2019distillation,zhang2019your} technique to explicitly train the single-modal classifiers to mimic the ``main'' classifier's distribution~\cite{phuong2019distillation,zhang2019your}. Note that as the single-modal classifiers are detached, this self-distillation technique has no effect on the performance of the model.
% \djkim{(we don't use it as a regularizer!)}
Our insight is that, as our acquisition function $S(V,Q)$ tries to find the sample that has a large difference between the multi-modal output (as teacher) and the single-modal output (as student), the knowledge distillation loss tries to directly minimize this difference. 
This in turn causes the easy samples to have a low $S(V,Q)$. 
In other words, if a sample gives a high $S(V,Q)$ value even after the explicit minimization of the $S(V,Q)$ score meaning the single-modal classifiers have difficulty following the output distribution of the multi-modal classifier, the sample can be thought of as a sample that is difficult or affected by both modalities and thus requires an oracle to be labeled.

Knowledge Distillation~\cite{hinton2015distilling} is defined as: training a ``student'' to follow a ``teacher'' model or representation.
Given a final output generated from a student model (in our case, $\mathbf{y}_v$ and $\mathbf{y}_q$) and an output from the teacher model (in our case, $\hat{\mathbf{y}}$), the student model learns the knowledge from the teacher's representation by forcing the student's representation to be similar to the teacher's.
% \begin{equation}
% 	\mathcal{L}_{distill}( \mathbf{y}_t,\mathbf{y}_s  ) = BCE(\mathbf{y}_t',\mathbf{y}_s'),
% 	\label{eq:loss_LWF}
% \end{equation}
% where
% \begin{equation}
% 	\\{y'}_k = \frac{(y_k)^{1/T}}{\sum_{k}^{}{(y_k)^{1/T}}}.
% 	\label{eqn:distillation}
% \end{equation}
% \djkim{(oh....eq(17) is for the distillation with CE loss, not BCE. We should remove eq(17))}
% where $y'_k$ is each individual output from the vector $\mathbf{y}$ of length $_k$ and $T$ is a hyperparameter \emph{Temperature}.
This approach suits our problem definition where the $g_v(\cdot)$ and $g_q(\cdot)$ can be student models and our $g(\cdot)$ can be the teacher model.
By adding the
% As $g_v(\cdot)$ and $g_q(\cdot)$ are only trained on classification loss,
self-distillation loss in addition to the classification loss can aid in training $g_v(\cdot)$ and $g_q(\cdot)$ to improve our acquisition function directly. We empirically prove our approach through the sampling performance gain.
% that the self-distillation loss aids in overall performance gain. 

% While the theory is sound, if the network (especially visual/question branch) is not well trained enough, we cannot guarantee that the acquisition function $S(V,Q)$ to work properly.
% Therefore, we 
% propose to 
% add knowledge distillation loss to boost the active learning performance.
% \js{(active learning performance or learning performance?)}
% \js{(self distillation enforces all branches to predict similarly?)}

% Our insight is as follows.
% Our acquisition function $S(V,Q)$ is to find the sample that has large distance between teacher and student.
% If we add the knowledge distillation loss to directly minimize this distance, the easy samples will be forced to have low $S(V,Q)$ values.
% \jwcho{(i dont know if i like this word encouraged... can we use a stronger word like force? or isit too strong?)}
% \js{(enforced?)}
% In other words, if a sample gives high value for $S(V,Q)$ even though we tried to explicitly minimize the $S(V,Q)$ score, the sample is highly likely to require oracle to label.
% In a mathematical interpretation.....\djkim{(maybe generalization bound?)}





%The loss function to train auxiliary branches is defined as 
The auxiliary single-modal branches are trained with the following loss functions:
\begin{equation}
    \mathcal{L}_v =  BCE(\mathbf{y},\mathbf{y}_v)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_v),
    \label{eqn:loss_v}
\end{equation}
\begin{equation}
    \mathcal{L}_q = BCE(\mathbf{y},\mathbf{y}_q)+\lambda BCE(\hat{\mathbf{y}},\mathbf{y}_q),
    \label{eqn:loss_q}
\end{equation}
where %$\mathcal{L}_{distill}(\cdot,\cdot)$ is the knowledge distillation loss~\cite{hinton2015distilling}.
%$\theta_v$ and $\theta_q$ are the parameter of the auxiliary single-modal branches $g_v(\cdot)$ and $g_q(\cdot)$ and 
$\lambda \geq0$ is a hyper-parameter to balance the loss weights.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Theoretical Properties}

% from introduction section. lets see where we can place this
% During the training phase, our model learns multiple branch of outputs which represents single-modal output and multi-modal output respectively.
% We additionally propose to use self-distillation framework~\cite{} for better training between single-modal and muti-modal outputs for single-modal output to predict answer as correct as multi-modal branch.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Re-examining our model, the training and sampling is reminiscent of Generative Adversarial Networks~\cite{goodfellow2014generative}, where the model is trained to produce the same output between single- and multi-modal, whereas in sampling, we label the data points that show a large gap between the two outputs.
% \djkim{(We shall remove this paragraph for re-submission)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% The strategy follows the intuition that if the output probability of the multi-modal and single-modal of the active learner is different, then it means that the missing sample is informative. \jwcho{(maybe here we can refer to the figure??)}
% \js{(Mentioning mini-max is understandable but, not sure if this can claim it is doing mini-max, because there is no 2-player aspect in loss function. Infact 2-players are doing the same thing, while HOPING that training is sufficient for prediction while insufficient for sampling.)}
% Therefore, instead of simply computing the entropy of the multi-modal output, we propose to use the entropy difference, which is the mutual information, to estimate the uncertainty of the unlabeled sample.
% With the proposed framework, we demonstrate the significant performance improvements in active learning setup.
% \djkim{(Let's move this details to the method section.)}
% --------------------------------------------------------

%\subsection{Temperature in Distillation Loss}



\noindent\textbf{Description of the Training and Sampling Procedure.}
The detailed description of the algorithms for training our model and sampling are shown in \Aref{alg:training} and \Aref{alg:sampling} respectively.







\begin{algorithm}[t]
\SetAlgoLined
\KwIn{Labeled pool $\mathcal{D}\textsubscript{L}$, Unlabeled pool $\mathcal{D}\textsubscript{U}$, Number of samples collecting for each stage $b$, Models $g_v(\cdot), g_q(\cdot),\text{ and }F(\cdot,\cdot)$ }
\KwOut{Updated $\mathcal{D}\textsubscript{L}$ and $\mathcal{D}\textsubscript{U}$}
\Begin{
    From $\mathcal{D}\textsubscript{U}$, collect a set of samples $\{X^s\}$ with 
    $\max_b S(V,Q) = \max_b{ \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y})}$\;
    $\{(X^s,Y^s)\} = ORACLE(\{X^s\})$\;
    $\mathcal{D}\textsubscript{L} \leftarrow \mathcal{D}\textsubscript{L} \cup \{(X^s,Y^s)\}$\;
    $\mathcal{D}\textsubscript{U} \leftarrow \mathcal{D}\textsubscript{U} - \{X^s\}$\;
}
 \caption{Our Proposed Sampling Strategy with Single-Modal Entropic Measure (SMEM)}
 \label{alg:sampling}
\end{algorithm}

==> Legacy/unused_4_sec_experiment.tex <==
In this section, we describe the experimental setups, competing methods, and provide performance evaluations of the proposed methods with both quantitative and qualitative results.

% \begin{figure}[t]
% \centering
% \vspace{-2mm}
% %\resizebox{1\linewidth}{!}{%
% {\includegraphics[width=0.4\linewidth,keepaspectratio]{Figures/quantitative_final}}
% %}
% %\vspace{-2mm}
% \caption{Comparison with existing approaches. Reference is the best performance of the existing methods.
% Our model shows the best performance among all the other methods by a large margin.}
% \vspace{-2mm}
% \label{fig:quantitative}
% \end{figure}

\subsection{Experimental Setup}
\noindent\textbf{Dataset and metric.}
We evaluate our method on VQA 2.0 dataset~\cite{antol2015vqa}, which consists of 1.1M data points (visual-question-answer triplets), with 444K/214K/448K for train/val/test respectively.
Each image is set up with at least 3 questions and 10 answers per question and thus contains 204K images, 1.1M questions, 11.1M answers.
As for evaluation, we utilize the VQA accuracy metric~\cite{antol2015vqa}.


\noindent\textbf{Active Learning setup.}
For the Active Learning (AL) setup, labeled set $\mathcal{D}\textsubscript{L}$ with a size of 40,000 out of 443,757 training data points is initialized randomly, and our model is trained until the training loss converges.
After converging, which marks the end of the first stage, we use this model to collect the samples from the unlabeled dataset $\mathcal{D}\textsubscript{U}$ according to an acquisition function $S(V,Q)$.
For every stage, we sample the next 40,000 data points from the unlabeled dataset and add them to the labeled dataset.
After increasing the labeled set, we re-train our model using the resulting labeled set, and repeat the previous steps (marking the subsequent stages), increasing the dataset and training the model for 10 iterations, resulting in a final $\mathcal{D}\textsubscript{L}$ size of 400,000 data points.



\noindent\textbf{Implementation details.}
%\subsection{Details of Network Architecture}
The base network architecture we adopt for this VQA task is identical to that of~\cite{anderson2018bottom}, with modifications to the classifier layer as we include 3 different classifiers. 
Full implementation details can be found in the supplementary section.
% Model architecture implementation details can be found in the supplementary section of this paper.
The changes we make to the model is that we add two additional classifier layers which takes the single modalities as its input as shown in~\Fref{fig:architecture} as $g_v(\cdot)$ and $g_q(\cdot)$ respectively. These classifiers are identical to the model's original classifier, $g(\cdot)$, and the difference is that while $g(\cdot)$ takes in the input of $\mathbf{z}$ as shown in equation (2), classifiers $g_v(\cdot)$ takes in $\mathbf{z}\textsubscript{v}$ and $g_q(\cdot)$ takes in $\mathbf{z}\textsubscript{q}$. 
Because we use identical classifiers, our method does not significantly increase parameters or calculation costs, making it cost-effective.
More detail is in the supplementary material.

% -------------------------- move to supple? ---------------------------------
% Following the model from~\cite{anderson2018bottom}, we make use of the pre-extracted image features from Mask-RCNN~\cite{he2017mask} for the visual input and Glove6B~\cite{pennington2014glove} embedding with a GRU~\cite{chung2014empirical} to process the question features. Then, the features are attended using the modified version of the attention proposed in~\cite{anderson2018bottom}~\footnote{The modified version of the attention proposed in~\cite{anderson2018bottom} is found on this github link: https://github.com/hengyuan-hu/bottom-up-attention-vqa}.
% Following this, a classifier layer is used to classify the outputs. In addition to the classifier layer which takes the attended features as its input, we create 2 more classifier layers which takes the single modalities as its input as shown in~\ref{fig:architecture} as $g{\_}v(\cdot)$ and $g{\_}q(\cdot)$ respectively. These classifiers have the same exact properties as $g(\cdot)$, the only difference is that while $g(\cdot)$ takes in the input of $Z$ as shown in equation (2), classifiers $g{\_}v(\cdot)$ takes in $Z\textsubscript{v}$ and $g{\_}q(\cdot)$ takes in $Z\textsubscript{q}$. 
% \djkim{(maybe move this to the supplementary?)}
% ----------------------------------------------------------------------------





\noindent\textbf{Baseline approaches.}
In order to demonstrate the effectiveness of our method, we compare the performance of our model to widely used sample acquisition approaches~\cite{culotta2005reducing,scheffer2001active,shen2017deep}:
{\setdefaultleftmargin{3mm}{}{}{}{}{}
\begin{itemize}
    \item \textbf{\emph{Random}} passive learning strategy that queries points following a uniformly random distribution.
    \item \textbf{\emph{Entropy}~\cite{shen2017deep}} queries instances that maximize the entropy of a model's output: $S(V,Q)=H(\hat{Y})$.
    \item \textbf{\emph{Margin}~\cite{scheffer2001active}} queries instances with the least margin between the output probabilities for the two most likely generated answers of a model: $S(V,Q)=1 + \hat{\mathbf{y}}^1-\hat{\mathbf{y}}^2$, where $\hat{\mathbf{y}}^1$ and $\hat{\mathbf{y}}^2$ are the probability of the first and second most confident model's responses.
    \item \textbf{\emph{Least Confident (LC)}~\cite{culotta2005reducing}} queries instances for which a model has the least confidence in its most likely generated sequence: $S(V,Q)=1-\hat{\mathbf{y}}^*$, where $\hat{\mathbf{y}}^*$ is the probability of the most confident model's response.
\end{itemize}
}

\begin{table}[t]
\vspace{-2mm}
\centering
\caption{Ablation study of our method. Our final method (the last row) shows the best performance among the variants of our methods in most of the Active Learning stages.}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{ ccc|cccccccccc }
    \hline
    \textbf{\emph{+JSD}}&\textbf{\emph{+Distillation}}&\textbf{\emph{+Entropy}}&1&2&3&4&5&6&7&8&9&10\\
    \hline
    $\times$&$\times$&$\times$        &50.52	&54.06	&55.59	&56.85	&57.7	&58.55	&59.06	&59.52	&59.93	&60.12\\%&50.33	&54.05	&\textbf{55.96}	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
    $\checkmark$&$\times$&$\times$      &50.81	&53.92	&55.55	&56.78	&57.69	&58.32	&58.94	&59.33	&59.64	&60.02\\
    $\times$&$\checkmark$&$\times$      &50.27	&54.10	&55.77	&57.08	&57.89	&58.52	&59.03	&59.46	&59.89	&60.20\\
    $\checkmark$&$\checkmark$&$\times$    &50.77	&54.08	&55.78	&57.02	&57.90	&58.60	&59.13	&59.63	&59.91	&60.24\\
    $\times$&$\times$&$\checkmark$      &50.65	&53.97	&55.42	&56.65	&57.63	&58.51	&59.27	&59.82	&60.20	&60.36\\
    $\checkmark$&$\times$&$\checkmark$    &49.94	&53.61	&55.45	&56.75	&57.77	&58.61	&59.47	&60.04	&60.39	&60.53\\
    $\times$&$\checkmark$&$\checkmark$    &50.39	&53.98	&\textbf{55.92}	&\textbf{57.21}	&58.05	&58.84	&59.54	&60.09	&60.50	&60.61\\
    $\checkmark$&$\checkmark$&$\checkmark$ &{50.03}	&\textbf{54.13}	&{55.71}	&{56.99}	&\textbf{58.06}	&\textbf{58.85}	&\textbf{59.66}	&\textbf{60.21}	&\textbf{60.61}	&\textbf{60.81}\\
    \hline
\end{tabular}
}

\vspace{-2mm}
\label{table:ablation_ours}
\end{table}



\begin{figure}[b]
\vspace{-4mm}
\centering
%\resizebox{1\linewidth}{!}{%
\subfigure[Vanilla]{\includegraphics[width=0.32\linewidth]{Figures/ablation_plain}}
\subfigure[+Distillation]{\includegraphics[width=0.32\linewidth]{Figures/ablation+distillation}}
\subfigure[+Distillation+Entropy]{\includegraphics[width=0.32\linewidth]{Figures/ablation+distillation+entropy}}
%}
\vspace{-2mm}
\caption{Comparison between different measuring methods. 
Ours is the SMEM + JSD in all graphs above. 
(a):without anything, (b):with distillation loss, and (c):with both distillation loss and entropy. }
\vspace{-2mm}
\label{fig:ablation}
\end{figure}



\subsection{Quantitative Results}


\noindent\textbf{Comparison with existing approaches.}
We compare our final method to existing AL methods~\cite{culotta2005reducing,scheffer2001active,shen2017deep} that do not consider multi-modality in \Fref{fig:quantitative}.
Among the existing methods, \textbf{\emph{Margin}} and \textbf{\emph{Least Confident(LC)}} show similarly poor performance, while \textbf{\emph{Random}} and \textbf{\emph{Entropy}} show better performance in the early stage and the late stage respectively. 
Between \textbf{\emph{Random}} and \textbf{\emph{Entropy}}, \textbf{\emph{Random}} shows a higher score in the early stage.
Moreover, our proposed method shows the best performance compared to all the counterparts by a large margin in all stages.
Note that the best among the existing approaches achieved 59.28\% accuracy when using 400,000 training samples, which is similar performance of our model trained with 240,000 training samples, signifying that our method SMEM can save about 40\% of the human labeling effort compared to existing approaches.



\noindent\textbf{Ablation study.}
Here, we introduce variants of our sampling methods.
\textbf{{\emph{KL-Divergence (KLD)}}} is described in \Eref{eqn:kld}. %\djkim{(multimodal1,2)}
\textbf{\emph{Jensen-Shannon Divergence only (JSD)}} is the baseline that is sampled by only using Jensen-Shannon divergence described in \Eref{eqn:jsd}. %\djkim{(multimodal3)}
\textbf{\emph{Absolute Difference of KL-Divergence (AD-KLD)}} is described in \Eref{eqn:ad-kld}. %\djkim{(multimodal6)}
\textbf{\emph{Mutual Information (MI)}} is the baseline that is sampled by only using mutual information: $S(V,Q) = \alpha I(A;V|Q) + (1-\alpha) I(A;Q|V)$. %\djkim{(multimodal7,8)}
\textbf{\emph{Single-Modal Entropic Measure (SMEM) or (Ours)}} is our proposed method either before or after adding entropy term as described in \Eref{eqn:addJSD} or \Eref{eqn:final}.  %\djkim{(multimodalV,Q)}



In addition, we also perform an analysis on each of the components of our final method.
\textbf{\emph{+Distillation}} is for the proposed self-distillation loss described in \Sref{sec:distillation}.
\textbf{\emph{+Entropy}} indicates the additional entropy term of the main branch output $H(\hat{Y})$ which changes our acquisition function from \Eref{eqn:addJSD} to \Eref{eqn:final}.
\textbf{\emph{+Jensen-Shannon Divergence (+JSD)}} is the additional Jensen-Shannon divergence term which changes our acquisition function from \Eref{eqn:student} to \Eref{eqn:addJSD}.



The ablation study results are illustrated in \Fref{fig:ablation}.
We compare the AL performance of our model with other design choices for distribution discrepancy measures.
We draw the training curves for three different setups: (a) without distillation or entropy, (b) adding distillation loss only, and (c) adding distillation loss and entropy.
Each setup shows its strengths in different areas of the AL stages.
In (a), ours shows the best performance in the early stages with less data while \textbf{\emph{KLD}} shows better performance in the later stages as more data is accumulated.
In (b), ours shows the best performance with less data while \textbf{\emph{MI}} shows better performance as more data is accumulated.
In (c), we show that by taking the main entropy into account, our model shows the best performance compared to all the other design choices throughout all given stages.






\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=.8\linewidth]{Figures/qualitative}
   \vspace{-2mm}
   \caption{Qualitative result of the Top-1 prediction of our model for every Active Learning stage.}
\label{fig:qualitative}
\vspace{-2mm}
\end{figure}

Finally, we perform an ablation study on each of the components of our SMEM method, and we show the results in~\Tref{table:ablation_ours}.
Since the first stage is randomly initialized, comparison in the first stage is meaningless.
% Because the first stage does not involves sample acquisition, 
% we do not compare the model in the first stage.
\textbf{\emph{+JSD}} improves the performance when we use \textbf{\emph{+Entropy}}.
\textbf{\emph{+Distillation}} improves the performance when we use either \textbf{\emph{+JSD}} or \textbf{\emph{+Entropy}}.
Moreover, \textbf{\emph{+Entropy}} improves the performance when we use \textbf{\emph{+Distillation}}.
Among all the baselines, our final setups (which includes all \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, and \textbf{\emph{+Entropy}}) shows the best performance in most of the stages.


\subsection{Qualitative Results}
\Fref{fig:qualitative} shows the qualitative results of our model for every AL stage. 
For each stage, we show the Top-1 predicted answer colored in blue if correct and red if not correct.
As the AL stages progress, the model is trained to generate increasingly accurate answers.
More qualitative results can be found in the supplementary material.

% \subsection{Additional Analysis}



%\subsection{Effects of Distillation Temperature}

% Through various results and hyper-parameter tuning, there has been differing effects of temperature on the model. One of the biggest trends we can see is that as the temperature on the teacher model is increased in relation to that of the student model, although the final accuracies do get higher, the initial accuracies suffer. This can be thought of as a trade-off or a in some ways destructive in the early stages where there are not too much data in the dataset, causing the model to be easily affected by the gradients of the other classifiers. % maybe <- not sure



%\begin{table}[h]
%\centering
%\caption{Ablation Study. Comparison between the variations of our approach.}
%\resizebox{1\linewidth}{!}{%
%\begin{tabular}{ l|cccccccccc }
%    \hline
%    &1&2&3&4&5&6&7&8&9&10\\
%    \hline
%    \textbf{\emph{KLD}}                                         &50.63  &53.60	&55.66	&56.77	&58.09	&58.71	&59.30	&59.69  &60.09  &60.39\\
%    \textbf{\emph{KLD+Distillation}}                            &50.43	&53.78	&55.48	&56.72	&57.55	&58.47	&59.14	&59.79	&60.28	&60.62\\
%    \textbf{\emph{KLD+Distillation+Entropy}}                    &50.47	&53.66	&55.57	&56.91	&57.81	&58.73	&59.54	&60.10	&60.41	&60.74\\
%    \hline
%    \textbf{\emph{JSD}}                                         &50.59	&53.36	&55.08	&56.47	&57.25	&58.34	&58.94	&59.42	&59.89	&60.20\\
%    \textbf{\emph{JSD+Distillation}}                            &50.36	&53.35	&55.37	&56.46	&57.57	&58.37	&58.90	&59.32	&59.75	&60.12\\
%    \textbf{\emph{JSD+Distillation+Entropy}}                    &50.72	&53.97	&55.63	&56.92	&57.95	&58.99	&59.78	&60.30	&60.63	&60.74\\
%    \hline
%    \textbf{\emph{MI}}                                          &50.96	&53.77	&55.56	&56.73	&57.64	&58.47	&59.03	&59.53	&59.91	&60.19\\
%    \textbf{\emph{MI+Distillation}}                             &50.44	&53.40	&54.96	&56.14	&56.98	&57.96	&58.82	&59.55	&60.15	&60.49\\
%    \textbf{\emph{MI+Distillation+Entropy}}                     &50.32	&53.63	&55.29	&56.47	&57.53	&58.30	&59.22	&59.76	&60.11	&60.57\\
%    \hline
%    \textbf{\emph{\djkim{(NAME?)} (Ours)}}                      &50.33	&54.05	&55.96	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
%    \textbf{\emph{\djkim{(NAME?)}+Distillation (Ours)}}         &50.40	&54.04	&56.06	&57.27	&58.14	&58.89	&59.61	&60.22	&60.42	&60.61\\
%    \textbf{\emph{\djkim{(NAME?)}+Distillation+Entropy (Ours)}} &50.53	&54.34	&56.25	&57.41	&58.28	&59.07	&59.71	&60.31	&60.62	&60.81\\
%    \hline
%\end{tabular}
%}
%\label{table:ablation}
%\end{table}













%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_ours.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study of our method.}
%\label{fig:ablation_ours}
%\end{figure}

%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_operation.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study with different ways to combine multimodal7 and multimodal 8. Multiplication shows %the best performance among the various options.}
%\label{fig:operation}
%\end{figure}


%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_temperature.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study with different temperature.}
%\label{fig:temperature}
%\end{figure}








==> Legacy/unused_4_sec_experiment_AAAI.tex <==
In this section, we describe the experimental setups, competing methods, and provide performance evaluations of the proposed methods.
\djkim{TODO : add results of additional baselines (VAAL, SRAAL, and maybe core-set?)}

\begin{figure}[t]
\centering
\vspace{-2mm}
%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_final}}
{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_VQA_new}}
%}
%\vspace{-2mm}
\caption{Comparison with existing approaches on the VQA v2.0 dataset. Reference is the best performance of the existing methods.
Our model shows the best performance among all the other methods by a large margin.}
\vspace{-2mm}
\label{fig:quantitative}
\end{figure}


\begin{table*}[t]
\vspace{-2mm}
\centering
\caption{Ablation study of our method. Our final method (the last row) shows the best performance among the variants of our methods in most of the Active Learning stages.%\djkim{(Justification to use Table. Mention that it is the same as Figures but more fine-grained values)}
}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{ c|ccc|cccccccccc }
    \hline
    Method&\textbf{\emph{+JSD}}&\textbf{\emph{+Distillation}}&\textbf{\emph{+Entropy}}&1&2&3&4&5&6&7&8&9&10\\
    \hline
    %Random&&&&50.42&53.93&	55.38&	56.72&	57.45&	57.93&	58.26&	58.49&	59.20&	59.33\\
    %Entropy&&&&50.16&	52.66&	54.24&	55.62&	56.59&	57.20&	58.19&	58.61&	59.28&	59.04\\
    Random&&&&50.56	&54.55	&55.93	&56.91	&58.59	&59.46	&60.27	&60.34	&61.11	&61.21\\
    Entropy&&&&50.74	&54.07	&55.49	&56.51	&58.21	&58.67	&60.30	&61.25	&61.50	&61.59\\
    \hline

    %\multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$        &50.52	&54.06	&55.59	&56.85	&57.70	&58.55	&59.06	&59.52	&59.93	&60.12\\%&50.33	&54.05	&\textbf{55.96}	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
    %&$\checkmark$&$\times$&$\times$      &50.81	&53.92	&55.55	&56.78	&57.69	&58.32	&58.94	&59.33	&59.64	&60.02\\
    %&$\times$&$\checkmark$&$\times$      &50.27	&54.10	&55.77	&57.08	&57.89	&58.52	&59.03	&59.46	&59.89	&60.20\\
    %&$\checkmark$&$\checkmark$&$\times$    &50.77	&54.08	&55.78	&57.02	&57.90	&58.60	&59.13	&59.63	&59.91	&60.24\\
    %&$\times$&$\times$&$\checkmark$      &50.65	&53.97	&55.42	&56.65	&57.63	&58.51	&59.27	&59.82	&60.20	&60.36\\
    %&$\checkmark$&$\times$&$\checkmark$    &49.94	&53.61	&55.45	&56.75	&57.77	&58.61	&59.47	&60.04	&60.39	&60.53\\
    %&$\times$&$\checkmark$&$\checkmark$    &50.39	&53.98	&\textbf{55.92}	&\textbf{57.21}	&58.05	&58.84	&59.54	&60.09	&60.50	&60.61\\
    %&$\checkmark$&$\checkmark$&$\checkmark$ &{50.03}	&\textbf{54.13}	&{55.71}	&{56.99}	&\textbf{58.06}	&\textbf{58.85}	&\textbf{59.66}	&\textbf{60.21}	&\textbf{60.61}	&\textbf{60.81}\\
    
    
    \multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$  &49.91	&54.34	&56.80	&58.21	&59.53	&60.62	&61.20	&62.02	&62.60	&63.10\\
    &$\checkmark$&$\times$&$\times$                             &50.10	&54.11	&56.14	&57.89	&59.21	&60.20	&61.24	&61.86	&62.55	&63.11\\
    &$\times$&$\checkmark$&$\times$                             &50.49	&54.36	&56.79	&\textbf{58.30}	&59.42	&60.49	&61.05	&62.00	&62.45	&62.92\\
    &$\checkmark$&$\checkmark$&$\times$                         &50.30	&54.35	&56.29	&58.08	&59.20	&60.27	&61.14	&61.79	&62.51	&63.06\\
    &$\times$&$\times$&$\checkmark$                             &50.32	&54.61	&56.81	&58.29	&59.34	&60.41	&61.61	&62.40	&62.94	&63.22\\
    &$\checkmark$&$\times$&$\checkmark$                         &50.23	&54.44	&56.63	&58.22	&59.13	&60.42	&61.67	&\textbf{62.47}	&62.94	&63.26\\
    &$\times$&$\checkmark$&$\checkmark$                         &50.43	&54.30	&56.76	&58.25	&59.44	&60.32	&61.55	&62.45	&62.97	&63.29\\
    &$\checkmark$&$\checkmark$&$\checkmark$                     &50.51	&\textbf{54.86}	&\textbf{56.82}	&\textbf{58.30}	&\textbf{59.55}	&\textbf{60.63}	&\textbf{61.74}	&\textbf{62.47}	&\textbf{63.00}	&\textbf{63.31}\\
    
    \hline
\end{tabular}
}

%\vspace{-2mm}
\label{table:ablation_ours}
\end{table*}





 \subsection{Experimental Setup for VQA v2.0 Dataset}
%\subsection{Experiments on VQA v2.0}
\noindent\textbf{Dataset and metric.}
We evaluate our method on VQA v2.0 dataset~\cite{antol2015vqa}, which consists of 1.1M data points (visual-question-answer triplets), with 444K/214K/448K for train/val/test respectively.
Each image is set up with at least 3 questions and 10 answers per question and thus contains 204K images, 1.1M questions, 11.1M answers.
As for evaluation, we utilize the VQA accuracy metric~\cite{antol2015vqa}.


\noindent\textbf{Active Learning setup.}
For the Active Learning (AL) setup, labeled set $\mathcal{D}\textsubscript{L}$ with a size of 40,000 out of 443,757 training data points \djkim{(as most of the existing AL works set 10\% of the full dataset as the budget)} is initialized randomly, and our model is trained until the training loss converges.
After converging, which marks the end of the first stage, we use this model to collect the samples from the unlabeled dataset $\mathcal{D}\textsubscript{U}$ according to an acquisition function $S(V,Q)$.
For every stage, we sample the next 40,000 data points from the unlabeled dataset and add them to the labeled dataset.
After increasing the labeled set, we train a newly initialized model using the resulting labeled set, and repeat the previous steps (marking the subsequent stages), increasing the dataset and training models for 10 iterations, resulting in a final $\mathcal{D}\textsubscript{L}$ size of 400,000 data points.



\noindent\textbf{Implementation details.}
%\subsection{Details of Network Architecture}
The base network architecture we adopt for this VQA task is identical to that of~\cite{anderson2018bottom}, with modifications to the classifier layer as we include 3 different classifiers. 
Full implementation details can be found in the supplementary section.
% Model architecture implementation details can be found in the supplementary section of this paper.
The only changes we make to the model is two additional classifier layers which takes the single modalities as its input as shown in~\Fref{fig:architecture} as $g_v(\cdot)$ and $g_q(\cdot)$ respectively. These classifiers are identical to the model's original classifier, $g(\cdot)$, and the difference is that while $g(\cdot)$ takes in the input of $\mathbf{z}$ as shown in equation (2), classifiers $g_v(\cdot)$ takes in $\mathbf{z}\textsubscript{v}$ and $g_q(\cdot)$ takes in $\mathbf{z}\textsubscript{q}$. 
Because we use identical classifiers, our method does not significantly increase parameters or calculation costs, making it cost-effective. In addition to this, we detach the classifiers from the model so the presence of the classifiers do not affect the performance of the model at all.
More details can be found in the supplementary material along with qualitative results on the VQA v2.0 dataset.
% -------------------------- move to supple? ---------------------------------
% Following the model from~\cite{anderson2018bottom}, we make use of the pre-extracted image features from Mask-RCNN~\cite{he2017mask} for the visual input and Glove6B~\cite{pennington2014glove} embedding with a GRU~\cite{chung2014empirical} to process the question features. Then, the features are attended using the modified version of the attention proposed in~\cite{anderson2018bottom}~\footnote{The modified version of the attention proposed in~\cite{anderson2018bottom} is found on this github link: https://github.com/hengyuan-hu/bottom-up-attention-vqa}.
% Following this, a classifier layer is used to classify the outputs. In addition to the classifier layer which takes the attended features as its input, we create 2 more classifier layers which takes the single modalities as its input as shown in~\ref{fig:architecture} as $g{\_}v(\cdot)$ and $g{\_}q(\cdot)$ respectively. These classifiers have the same exact properties as $g(\cdot)$, the only difference is that while $g(\cdot)$ takes in the input of $Z$ as shown in equation (2), classifiers $g{\_}v(\cdot)$ takes in $Z\textsubscript{v}$ and $g{\_}q(\cdot)$ takes in $Z\textsubscript{q}$. 
% \djkim{(maybe move this to the supplementary?)}
% ------------------------------------------------------------------------


\noindent\textbf{Baseline approaches.}
In order to demonstrate the effectiveness of our method, we compare the performance of our model to widely used sample acquisition approaches~\cite{culotta2005reducing,scheffer2001active,shen2017deep} as well as the recent deep Active Learning method~\cite{yoo2019learning}:%\djkim{(Require explanation why we don't use VAAL or SAAL etc.)}~\jwcho{(tried to answer in related works. maybe that is a good enough explanation)}
{\setdefaultleftmargin{3mm}{}{}{}{}{}
\begin{itemize}
    \item \textbf{\emph{Random}} passive learning strategy that queries points following a uniformly random distribution.
    \item \textbf{\emph{Entropy}~\cite{shen2017deep}} queries instances that maximize the entropy of a model's output: $S(V,Q)=H(\hat{Y})$.
    \item \textbf{\emph{Margin}~\cite{scheffer2001active}} queries instances with the least margin between the output probabilities for the two most likely generated answers of a model: $S(V,Q)=1 + \hat{\mathbf{y}}^1-\hat{\mathbf{y}}^2$, where $\hat{\mathbf{y}}^1$ and $\hat{\mathbf{y}}^2$ are the probability of the first and second most confident model's responses.
    \item \textbf{\emph{Least Confident (LC)}~\cite{culotta2005reducing}} queries instances for which a model has the least confidence in its most likely generated sequence: $S(V,Q)=1-\hat{\mathbf{y}}^*$, where $\hat{\mathbf{y}}^*$ is the probability of the most confident model's response.
    \item \textbf{\emph{Learning Loss (LL)}~\cite{yoo2019learning}} adds a loss prediction module which measures how much a sample would affect the loss if sampled.
\end{itemize}
}





\subsection{Results on VQA v2.0 Dataset}\djkim{(TODO:update the explanation about VAAL and SRAAL)}
% \djkim{(TODO : The improvements might be incremental. Need to improve.)}

%\djkim{(The reason why LC and margin are worse than random? Because the number of the classes are extremely large. Also, long-tailed distribution can be a problem.)}

% \djkim{(TODO : compare with ``Learning by asking Questions'' and ``VQA as meta-learning'', ``Learning loss for AC''. Maybe ``Core-set approach'' and ``query-by-committe''?)}

%\djkim{(TODO : other VQA datasets, CLEVER? VQAcp? VizWiz?)}

% \djkim{(TODO : different VQA architecture, CNN+LSTM, or BAN. Compare the gain from architecture and AL $\rightarrow$maybe we can't. the performance gain from the architecture is more than that from AL.)}

\noindent\textbf{Comparison with existing approaches.}
We compare our final method to existing AL methods~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning} that do not originally consider multi-modality in \Fref{fig:quantitative}.
Among the existing methods, \textbf{\emph{Margin}} and \textbf{\emph{Least Confident(LC)}} show similarly poor performance, while \textbf{\emph{Random}} and \textbf{\emph{Entropy}} show better performance in the early stage and the late stage respectively. 
We conjecture that the poor performance of \textbf{\emph{Margin}} and \textbf{\emph{LC}} is due to the large number of classes. In VQA v2.0 dataset, there are 3129 number of candidate classes, even after cutting out redundant classes and answers that appear less than 9 times, which is noticeably larger than typical image classification datasets (\emph{i.e.}, ImageNet). The large number of classes can also cause the long-tailed distribution problem which makes AL with conventional approaches difficult. In particular, the model predictions might be dominated to major classes; thus regarding only the most confident class (\textbf{\emph{LC}}) or second (\textbf{\emph{Margin}}) might lead to biased acquisition to major classes.
Between \textbf{\emph{Random}} and \textbf{\emph{Entropy}},
%\jwcho{(might need to change based on graph)}
\textbf{\emph{Random}} shows a higher score in the early stage, and \textbf{\emph{Entropy}} surpasses \textbf{\emph{Random}} in the later stages.
%\jwcho{\emph{LL} shows some kind of performance etc etc etc}
A recent approach, \textbf{\emph{LL}}, shows similar performance to \textbf{\emph{Random}} and \textbf{\emph{Entropy}} in VQA task.
Moreover, our proposed method shows the best performance compared to all the counterparts by a large margin in all stages.
Note that the best among the existing approaches achieved 59.28\% accuracy when using 400K training samples, which is similar performance of our model trained with 240K training samples, signifying that our method SMEM can save about 30\% of the human labeling effort compared to existing approaches.



\noindent\textbf{Ablation study.}
We perform an ablation study on each of the  components of our final method.
% In addition, we also perform an analysis on each of the components of our final method.
\textbf{\emph{+Distillation}} is for the proposed self-distillation loss described 
% in \Sref{sec:distillation}.
previously.
\textbf{\emph{+Entropy}} indicates the additional entropy term of the ``main'' branch output $H(\hat{Y})$ which changes our acquisition function from \Eref{eqn:addJSD} to \Eref{eqn:final}.
\textbf{\emph{+Jensen-Shannon Divergence (+JSD)}} is the additional JSD term which changes our acquisition function from \Eref{eqn:student} to \Eref{eqn:addJSD}.



% Finally, we perform an ablation study on each of the components of our SMEM method, and we show the
\Tref{table:ablation_ours} shows the fine-grained performance changes caused by the auxiliary terms, \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, \textbf{\emph{+Entropy}}.
We include traditional approaches, \textbf{\emph{Random}} and \textbf{\emph{Entropy}}, to compare with our methods. 
Although the performance improvements from each auxiliary terms might be seem marginal, we emphasize that the performance gain between \textbf{\emph{Entropy}} and our proposed SMEM model is noticeable.
Note that our model without any auxiliary terms already shows favorable performance at AL stages.
Since the first stage is randomly initialized, comparison in the first stage is meaningless.
\djkim{Although each change seems to make marginal difference, by adding all the terms, the performance gap between the one with none of the terms and all the terms become noticable.}
% Because the first stage does not involves sample acquisition, 
% we do not compare the model in the first stage.
%\djkim{(WE should change this part according to the updated result.)}
%\textbf{\emph{+JSD}} improves the performance when we use \textbf{\emph{+Entropy}}.
\textbf{\emph{+Entropy}} improves the performance consistently.
\textbf{\emph{+Distillation}} improves the performance when we use either \textbf{\emph{+JSD}} or \textbf{\emph{+Entropy}}.
%Moreover, \textbf{\emph{+Entropy}} improves the performance when we use \textbf{\emph{+Distillation}}.
Moreover, \textbf{\emph{+JSD}} improves the performance when we use both \textbf{\emph{+Distillation}} and \textbf{\emph{+Entropy}}.
Among all the baselines, our final setups (which includes all \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, and \textbf{\emph{+Entropy}}) shows the best performance in all stages.




\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/VizWiz.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VizWiz Dataset. Our proposed method shows the best performance in most of the sampling stages.}
\label{fig:VizWiz}
\vspace{-2mm}
\end{figure}

\subsection{Results on VizWiz VQA Dataset}

To demonstrate the effectiveness of our method, we also evaluate our method on another VQA dataset, the VizWiz VQA~\cite{gurari2018vizwiz} dataset, that is arguably more difficult.
The VizWiz dataset contains 19,425 train image/question pairs and we sample 1,900 image/question pairs per stage with the final stage ending at 19,000 image/question pairs.
For architecture, we use a variant of~\cite{yang2016stacked}\footnote{https://github.com/DenisDsh/VizWiz-VQA-PyTorch}.

We use the same baselines as the previous subsection, and experimental results are shown in \Fref{fig:VizWiz}.
As VizWiz is a more challenging dataset than VQA v2.0 dataset, %we have these and these and these results....
all the baselines show similarly lower performance overall.
One interesting observation is that, different from the other experiments, \textbf{\emph{LC}} shows better performance than \textbf{\emph{Random}} baseline.
Note that, among the baselines, our proposed method shows the best performance in most of the sampling stages.





\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/CP2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VQA-CP2 Dataset. Our model shows favorable performance compared to the baseline approaches in most of the stages.}
\label{fig:VQA-CP2}
\vspace{-2mm}
\end{figure}

\subsection{Results on VQA-CP2 Dataset}
We also evaluate our method the VQA-CP2~\cite{goyal2017making} dataset, which has a different data distribution between training and test splits.
VQA-CP2 is usually used to evaluate the robustness in uni-modal bias in VQA models.
As VQA-CP2 is a rearrangement of the VQA v2.0 dataset, the VQA-CP2 dataset size is similar yet slightly different and contains 438K train image/question pairs and we sample 40K image/question pairs per stage with the final stage ending at 400K image/question pairs.
We use the same network architecture from~\cite{anderson2018bottom} and we use the same baselines as VQA v2.0.

The experimental results on VQA-CP2 dataset is shown in \Fref{fig:VQA-CP2}.
Among the existing approaches, \textbf{\emph{Entropy}} shows the best performance.
Our model shows the highest peak performance and we can see an interesting case where \textbf{\emph{Entropy}} also peaks above the Reference.
We can conclude that our method is robust for modality bias as well.
Note that when tested on all 438K training data, the model performance showed to be 39.91\% (denoted by Reference in \Fref{fig:VQA-CP2}) which is lower than the performance of \emph{\textbf{Entropy}} and \emph{\textbf{Ours} trained with the subset of the training data}. 
%but using some of the Active Learning methods such as \emph{\textbf{Entropy}} and \emph{\textbf{Ours}} 
This
shows that by elaborately sampling some of the meaningful data, we are able to surpass the performance from the full dataset. We believe that this finding opens up interesting possible future research ideas.


\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/NTU.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the NTU RGB+D Action Recognition Dataset. Although our method is designed specifically for VQA task, our method consistently outperforms all the existing approaches in every sampling stage in terms of action recognition accuracy.}
\label{fig:NTU}
\vspace{-2mm}
\end{figure}

\subsection{Results on NTU Action Recognition Dataset}
Although our model is designed specifically for a model with multi-modal input (\emph{e.g.}, vision-language tasks), we also evaluate our model on one of the popular multi-modal action recognition datasets, NTU RGB+D dataset~\cite{shahroudy2016ntu}, in order to show the extensibility of our approach.
We show through experiments the effectiveness of our approach,
% Although the motivation for our work comes from multi-modal inputs and show through experiments the effectiveness of our approach, \jwcho{redundant}
and we believe that this method can be expanded to experiments that use multiple inputs. 

We %experiment on
use the model from~\cite{li2018co} with the NTU RGB+D dataset~\cite{shahroudy2016ntu} which leverages multiple views or subjects with the same action class and trains the network for improved performance.
The dataset processing used in the implementation of~\cite{li2018co} makes use of 37,646 pairs of inputs and we sample 3,000 at each stage, ending at 30,000 pairs at the last stage. 
We followed the cross-subject evaluation~\cite{shahroudy2016ntu} that splits the 40 subjects into training and testing sets.
We apply our method on the subject dataset and treat each subject as a single modality and train additional classifiers similar to the VQA settings. 

We use the same baselines as the previous subsection, and show experimental results in \Fref{fig:NTU}.
%We create the base active learning baselines and show through~\Fref{fig:NTU} 
% the effectiveness of our approach on this setting as well. 
%and demonstrate that 
Note that the gap between \textbf{\emph{Margin}} or \textbf{\emph{LC}} and the other baselines is larger than that of the previous experiments.
Among \textbf{\emph{Random}}, \textbf{\emph{Entropy}}, and \textbf{\emph{LL}}, and \textbf{\emph{LL}} shows the best performance in the early stages, and \textbf{\emph{Entropy}} shows the best performance in the later stages.
Moreover, compared to the baseline approaches, our method shows favorable performance 
%compared to the baseline approaches 
for all sampling stages in the NTU RGB+D dataset as well.
The effectiveness of our approach opens up the possibilities of applying our method on other kinds of datasets and tasks where multiple inputs maybe used whether they are of the same modality of not.




% \djkim{(Analysis suggestion : what would be the score like if the totally unrelated image-question pair?)}
% \djkim{(Or maybe draw t-SNE?)}
% \subsection{Additional Analysis}



%\subsection{Effects of Distillation Temperature}

% Through various results and hyper-parameter tuning, there has been differing effects of temperature on the model. One of the biggest trends we can see is that as the temperature on the teacher model is increased in relation to that of the student model, although the final accuracies do get higher, the initial accuracies suffer. This can be thought of as a trade-off or a in some ways destructive in the early stages where there are not too much data in the dataset, causing the model to be easily affected by the gradients of the other classifiers. % maybe <- not sure



%\begin{table}[h]
%\centering
%\caption{Ablation Study. Comparison between the variations of our approach.}
%\resizebox{1\linewidth}{!}{%
%\begin{tabular}{ l|cccccccccc }
%    \hline
%    &1&2&3&4&5&6&7&8&9&10\\
%    \hline
%    \textbf{\emph{KLD}}                                         &50.63  &53.60	&55.66	&56.77	&58.09	&58.71	&59.30	&59.69  &60.09  &60.39\\
%    \textbf{\emph{KLD+Distillation}}                            &50.43	&53.78	&55.48	&56.72	&57.55	&58.47	&59.14	&59.79	&60.28	&60.62\\
%    \textbf{\emph{KLD+Distillation+Entropy}}                    &50.47	&53.66	&55.57	&56.91	&57.81	&58.73	&59.54	&60.10	&60.41	&60.74\\
%    \hline
%    \textbf{\emph{JSD}}                                         &50.59	&53.36	&55.08	&56.47	&57.25	&58.34	&58.94	&59.42	&59.89	&60.20\\
%    \textbf{\emph{JSD+Distillation}}                            &50.36	&53.35	&55.37	&56.46	&57.57	&58.37	&58.90	&59.32	&59.75	&60.12\\
%    \textbf{\emph{JSD+Distillation+Entropy}}                    &50.72	&53.97	&55.63	&56.92	&57.95	&58.99	&59.78	&60.30	&60.63	&60.74\\
%    \hline
%    \textbf{\emph{MI}}                                          &50.96	&53.77	&55.56	&56.73	&57.64	&58.47	&59.03	&59.53	&59.91	&60.19\\
%    \textbf{\emph{MI+Distillation}}                             &50.44	&53.40	&54.96	&56.14	&56.98	&57.96	&58.82	&59.55	&60.15	&60.49\\
%    \textbf{\emph{MI+Distillation+Entropy}}                     &50.32	&53.63	&55.29	&56.47	&57.53	&58.30	&59.22	&59.76	&60.11	&60.57\\
%    \hline
%    \textbf{\emph{\djkim{(NAME?)} (Ours)}}                      &50.33	&54.05	&55.96	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
%    \textbf{\emph{\djkim{(NAME?)}+Distillation (Ours)}}         &50.40	&54.04	&56.06	&57.27	&58.14	&58.89	&59.61	&60.22	&60.42	&60.61\\
%    \textbf{\emph{\djkim{(NAME?)}+Distillation+Entropy (Ours)}} &50.53	&54.34	&56.25	&57.41	&58.28	&59.07	&59.71	&60.31	&60.62	&60.81\\
%    \hline
%\end{tabular}
%}
%\label{table:ablation}
%\end{table}













%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_ours.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study of our method.}
%\label{fig:ablation_ours}
%\end{figure}

%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_operation.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study with different ways to combine multimodal7 and multimodal 8. Multiplication shows %the best performance among the various options.}
%\label{fig:operation}
%\end{figure}


%\begin{figure}[ht]
%\centering
%%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=0.5\linewidth,keepaspectratio]{Figures/ablation_temperature.pdf}}
%%}
%%\vspace{-2mm}
%\caption{Ablation study with different temperature.}
%\label{fig:temperature}
%\end{figure}








==> Legacy/unused_4_sec_experiment_ICML.tex <==
In this section, we describe the experimental setups, competing methods, and provide performance evaluations of the proposed methods.
% \djkim{TODO : add results of additional baselines (VAAL, SRAAL, and maybe core-set?)}












\subsection{Experimental Setup for VQA v2.0 Dataset}
%\subsection{Experiments on VQA v2.0}
\noindent\textbf{Dataset and metric.}
We evaluate our method on VQA v2.0 dataset~\cite{antol2015vqa}, which consists of 1.1M data points (visual-question-answer triplets), with 444K/214K/448K for train/val/test respectively.
Each image is set up with at least 3 questions and 10 answers per question and thus contains 204K images, 1.1M questions, 11.1M answers.
As for evaluation, we utilize the VQA accuracy metric~\cite{antol2015vqa}.


\noindent\textbf{Active Learning setup.}
For the Active Learning (AL) setup, labeled set $\mathcal{D}\textsubscript{L}$ with a size of 40,000 out of 443,757 training data points, which is roughly 10\% of the full dataset,
% \djkim{(as most of the existing AL works set 10\% of the full dataset as the budget)} 
is initialized randomly, and our model is trained until the training loss converges.
After converging, which marks the end of the first stage, we use this model to collect samples from the unlabeled dataset $\mathcal{D}\textsubscript{U}$ according to an acquisition function $S(V,Q)$.
For every stage, we sample the next 40,000 data points from the unlabeled dataset and add them to the labeled dataset.
After increasing the labeled set, we train a newly initialized model using the resulting labeled set, and repeat the previous steps (marking the subsequent stages), increasing the dataset and training models for 10 iterations, resulting in a final $\mathcal{D}\textsubscript{L}$ size of 400,000 data points.



\noindent\textbf{Implementation details.}
%\subsection{Details of Network Architecture}
The base network architecture we adopt for this VQA task is identical to that of~\cite{anderson2018bottom}, with modifications to the classifier layer as we include two additional classifiers. 
Full implementation details can be found in the supplementary section.
% Model architecture implementation details can be found in the supplementary section of this paper.
The only changes we make to the model is two additional classifier layers which takes the single modalities as its input as shown in~\Fref{fig:architecture} as $g_v(\cdot)$ and $g_q(\cdot)$ respectively. These classifiers are identical to the model's original classifier, $g(\cdot)$, and the difference is that while $g(\cdot)$ takes in the input of $\mathbf{z}$ as shown in equation (2), classifiers $g_v(\cdot)$ takes in $\mathbf{z}\textsubscript{v}$ and $g_q(\cdot)$ takes in $\mathbf{z}\textsubscript{q}$. 
Because we use identical classifiers, our method does not significantly increase parameters or calculation costs, making it cost-effective. In addition to this, we detach the classifiers from the model so the presence of the classifiers do not affect the performance of the model at all.
More details can be found in the supplementary material along with qualitative results on the VQA v2.0 dataset.
% -------------------------- move to supple? ---------------------------------
% Following the model from~\cite{anderson2018bottom}, we make use of the pre-extracted image features from Mask-RCNN~\cite{he2017mask} for the visual input and Glove6B~\cite{pennington2014glove} embedding with a GRU~\cite{chung2014empirical} to process the question features. Then, the features are attended using the modified version of the attention proposed in~\cite{anderson2018bottom}~\footnote{The modified version of the attention proposed in~\cite{anderson2018bottom} is found on this github link: https://github.com/hengyuan-hu/bottom-up-attention-vqa}.
% Following this, a classifier layer is used to classify the outputs. In addition to the classifier layer which takes the attended features as its input, we create 2 more classifier layers which takes the single modalities as its input as shown in~\ref{fig:architecture} as $g{\_}v(\cdot)$ and $g{\_}q(\cdot)$ respectively. These classifiers have the same exact properties as $g(\cdot)$, the only difference is that while $g(\cdot)$ takes in the input of $Z$ as shown in equation (2), classifiers $g{\_}v(\cdot)$ takes in $Z\textsubscript{v}$ and $g{\_}q(\cdot)$ takes in $Z\textsubscript{q}$. 
% \djkim{(maybe move this to the supplementary?)}
% ------------------------------------------------------------------------





\noindent\textbf{Baseline approaches.}
In order to demonstrate the effectiveness of our method, we compare the performance of our model to widely used sample acquisition approaches~\cite{culotta2005reducing,scheffer2001active,shen2017deep} as well as the recent deep AL methods~\cite{sinha2019variational,yoo2019learning,zhang2020state}:%\djkim{(Require explanation why we don't use VAAL or SAAL etc.)}~\jwcho{(tried to answer in related works. maybe that is a good enough explanation)}
{\setdefaultleftmargin{3mm}{}{}{}{}{}
\begin{itemize}
    % \vspace{-4mm}
    \item \textbf{\emph{Random}} passive learning strategy that queries points following a uniformly random distribution.
    % \vspace{-2mm}
    \item \textbf{\emph{Entropy}~\cite{shen2017deep}} queries instances that maximize the entropy of a model's output: $S(V,Q)=H(\hat{Y})$.
    % \vspace{-6mm}
    \item \textbf{\emph{Margin}~\cite{scheffer2001active}} queries instances with the least margin between the output probabilities for the two most likely generated answers of a model: $S(V,Q)=1 + \hat{\mathbf{y}}^1-\hat{\mathbf{y}}^2$, where $\hat{\mathbf{y}}^1$ and $\hat{\mathbf{y}}^2$ are the probability of the first and second most confident model's responses.
    % \vspace{-3mm}
    \item \textbf{\emph{Least Confident (LC)}~\cite{culotta2005reducing}} queries instances for which a model has the least confidence in its most likely generated sequence: $S(V,Q)=1-\hat{\mathbf{y}}^*$, where $\hat{\mathbf{y}}^*$ is the probability of the most confident model's response.
    % \vspace{-3mm}
    \item \textbf{\emph{Learning Loss (LL)}~\cite{yoo2019learning}} adds a loss prediction module which measures how much a sample would affect the loss if sampled.
    % \vspace{-3mm}
    \item \textbf{\emph{Variational Adversarial Active Learning (VAAL)}~\cite{sinha2019variational}} adds a VAE to generate a latent space and discriminate between labeled and unlabeled samples.
    % \vspace{-3mm}
    \item \textbf{\emph{State Relabeling Adversarial Active Learning (SRAAL)}~\cite{zhang2020state}} is similar to VAAL, but also leverages the uncertainty of the task model to discriminate samples.
    % \vspace{-3mm}
\end{itemize}
}

% \begin{figure}[t]
% \centering
% \vspace{-2mm}
% %\resizebox{1\linewidth}{!}{%
% %{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_final}}
% {\includegraphics[width=1\linewidth,keepaspectratio]{Figures/quantitative_VQA_new}}
% %}
% %\vspace{-2mm}
% \caption{Comparison with existing approaches on the VQA v2.0 dataset. Reference is the best performance of the existing methods.
% Our model shows the best performance among all the other methods by a large margin.}
% \vspace{-2mm}
% \label{fig:quantitative}
% \end{figure}


\begin{figure}[t]
\centering
\vspace{0mm}
%\resizebox{1\linewidth}{!}{%
%{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_final}}
{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_VQA_new}}
%}
%\vspace{-2mm}
\caption{Comparison with existing approaches on the VQA v2.0 dataset. Reference is the best performance of the existing methods.
Our model shows the best performance among all the other methods by a large margin. Full dataset training shows 63.52\% accuracy, while ours at \emph{stage 10} shows 63.31\% accuracy.}
\vspace{-2mm}
\label{fig:quantitative}
\end{figure}


\begin{table*}[t]
\vspace{0mm}
\centering
\caption{Ablation study of our method. Our final method (the last row) shows the best performance among the variants of our methods in most of the Active Learning stages.%\djkim{(Justification to use Table. Mention that it is the same as Figures but more fine-grained values)}
}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{ c|ccc|cccccccccc }
    \hline
    Method&\textbf{\emph{+JSD}}&\textbf{\emph{+Distillation}}&\textbf{\emph{+Entropy}}&1&2&3&4&5&6&7&8&9&10\\
    \hline
    %Random&&&&50.42&53.93&	55.38&	56.72&	57.45&	57.93&	58.26&	58.49&	59.20&	59.33\\
    %Entropy&&&&50.16&	52.66&	54.24&	55.62&	56.59&	57.20&	58.19&	58.61&	59.28&	59.04\\
    Random&&&&50.56	&54.55	&55.93	&56.91	&58.59	&59.46	&60.27	&60.34	&61.11	&61.21\\
    Entropy&&&&50.74	&54.07	&55.49	&56.51	&58.21	&58.67	&60.30	&61.25	&61.50	&61.59\\
    \hline

    %\multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$        &50.52	&54.06	&55.59	&56.85	&57.70	&58.55	&59.06	&59.52	&59.93	&60.12\\%&50.33	&54.05	&\textbf{55.96}	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
    %&$\checkmark$&$\times$&$\times$      &50.81	&53.92	&55.55	&56.78	&57.69	&58.32	&58.94	&59.33	&59.64	&60.02\\
    %&$\times$&$\checkmark$&$\times$      &50.27	&54.10	&55.77	&57.08	&57.89	&58.52	&59.03	&59.46	&59.89	&60.20\\
    %&$\checkmark$&$\checkmark$&$\times$    &50.77	&54.08	&55.78	&57.02	&57.90	&58.60	&59.13	&59.63	&59.91	&60.24\\
    %&$\times$&$\times$&$\checkmark$      &50.65	&53.97	&55.42	&56.65	&57.63	&58.51	&59.27	&59.82	&60.20	&60.36\\
    %&$\checkmark$&$\times$&$\checkmark$    &49.94	&53.61	&55.45	&56.75	&57.77	&58.61	&59.47	&60.04	&60.39	&60.53\\
    %&$\times$&$\checkmark$&$\checkmark$    &50.39	&53.98	&\textbf{55.92}	&\textbf{57.21}	&58.05	&58.84	&59.54	&60.09	&60.50	&60.61\\
    %&$\checkmark$&$\checkmark$&$\checkmark$ &{50.03}	&\textbf{54.13}	&{55.71}	&{56.99}	&\textbf{58.06}	&\textbf{58.85}	&\textbf{59.66}	&\textbf{60.21}	&\textbf{60.61}	&\textbf{60.81}\\
    
    
    \multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$  &49.91	&54.34	&56.80	&58.21	&59.53	&60.62	&61.20	&62.02	&62.60	&63.10\\
    &$\checkmark$&$\times$&$\times$                             &50.10	&54.11	&56.14	&57.89	&59.21	&60.20	&61.24	&61.86	&62.55	&63.11\\
    &$\times$&$\checkmark$&$\times$                             &50.49	&54.36	&56.79	&\textbf{58.30}	&59.42	&60.49	&61.05	&62.00	&62.45	&62.92\\
    &$\checkmark$&$\checkmark$&$\times$                         &50.30	&54.35	&56.29	&58.08	&59.20	&60.27	&61.14	&61.79	&62.51	&63.06\\
    &$\times$&$\times$&$\checkmark$                             &50.32	&54.61	&56.81	&58.29	&59.34	&60.41	&61.61	&62.40	&62.94	&63.22\\
    &$\checkmark$&$\times$&$\checkmark$                         &50.23	&54.44	&56.63	&58.22	&59.13	&60.42	&61.67	&\textbf{62.47}	&62.94	&63.26\\
    &$\times$&$\checkmark$&$\checkmark$                         &50.43	&54.30	&56.76	&58.25	&59.44	&60.32	&61.55	&62.45	&62.97	&63.29\\
    &$\checkmark$&$\checkmark$&$\checkmark$                     &50.51	&\textbf{54.86}	&\textbf{56.82}	&\textbf{58.30}	&\textbf{59.55}	&\textbf{60.63}	&\textbf{61.74}	&\textbf{62.47}	&\textbf{63.00}	&\textbf{63.31}\\
    
    \hline
\end{tabular}
}

%\vspace{-2mm}
\label{table:ablation_ours}
\end{table*}


\subsection{Results on VQA v2.0 Dataset}
% \djkim{(TODO : The improvements might be incremental. Need to improve.)}

%\djkim{(The reason why LC and margin are worse than random? Because the number of the classes are extremely large. Also, long-tailed distribution can be a problem.)}

% \djkim{(TODO : compare with ``Learning by asking Questions'' and ``VQA as meta-learning'', ``Learning loss for AC''. Maybe ``Core-set approach'' and ``query-by-committe''?)}

%\djkim{(TODO : other VQA datasets, CLEVER? VQAcp? VizWiz?)}

% \djkim{(TODO : different VQA architecture, CNN+LSTM, or BAN. Compare the gain from architecture and AL $\rightarrow$maybe we can't. the performance gain from the architecture is more than that from AL.)}

\noindent\textbf{Comparison with existing approaches.}
We compare our final method to existing AL methods~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning} that do not originally consider multi-modality in \Fref{fig:quantitative}.
Among the existing methods, \textbf{\emph{Margin}} and \textbf{\emph{Least Confident(LC)}} show similarly poor performance, while \textbf{\emph{Random}} and \textbf{\emph{Entropy}} show better performance in the early stage and the late stage respectively. 
We conjecture that the poor performance of \textbf{\emph{Margin}} and \textbf{\emph{LC}} is due to the large number of classes. In VQA v2.0 dataset, there are 3129 number of candidate classes, even after cutting out redundant classes and answers that appear less than 9 times, which is noticeably larger than typical image classification datasets (\emph{i.e.}, ImageNet). The large number of classes can also cause the long-tailed distribution problem which makes AL with conventional approaches difficult. In particular, the model predictions might be dominated to major classes; thus regarding only the most confident class (\textbf{\emph{LC}}) or second (\textbf{\emph{Margin}}) might lead to biased acquisition to major classes.
Between \textbf{\emph{Random}} and \textbf{\emph{Entropy}},
\textbf{\emph{Random}} shows a higher score in the early stage, and \textbf{\emph{Entropy}} surpasses \textbf{\emph{Random}} in the later stages.
%A recent approach, \textbf{\emph{LL}}, shows
Note that recent state-of-the-art Active Learning methods, \textbf{\emph{LL}}, \textbf{\emph{VAAL}}, \textbf{\emph{VRAAL}}, show similar performance to \textbf{\emph{Random}} and \textbf{\emph{Entropy}} in VQA task.
Moreover, our proposed method shows the best performance compared to all the counterparts by a large margin in all stages.
Note that the best among the existing approaches achieved 59.28\% accuracy when using 400K training samples, which is similar performance of our model trained with 240K training samples, signifying that our method SMEM can save about 30\% of the human labeling effort compared to existing approaches.






\noindent\textbf{Ablation study.}
We perform an ablation study on each of the  components of our final method.
% In addition, we also perform an analysis on each of the components of our final method.
\textbf{\emph{+Distillation}} is for the proposed self-distillation loss described 
% in \Sref{sec:distillation}.
previously.
\textbf{\emph{+Jensen-Shannon Divergence (+JSD)}} is the additional JSD term which changes our acquisition function from \Eref{eqn:student} to \Eref{eqn:addJSD}.
\textbf{\emph{+Entropy}} indicates the additional entropy term of the ``main'' branch output $H(\hat{Y})$ which changes our acquisition function from \Eref{eqn:addJSD} to $S(V,Q)+ \gamma H(\hat{Y})$.




% Finally, we perform an ablation study on each of the components of our SMEM method, and we show the
\Tref{table:ablation_ours} shows the fine-grained performance changes caused by the auxiliary terms, \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, \textbf{\emph{+Entropy}}.
We include traditional approaches, \textbf{\emph{Random}} and \textbf{\emph{Entropy}} for comparison. 
Although the performance improvements from each auxiliary terms might be seem marginal, we emphasize that the performance gain between \textbf{\emph{Entropy}} and our proposed SMEM model is noticeable.
Note that our model without any auxiliary terms already shows favorable performance.
Since the first stage is randomly initialized, comparison in the first stage is meaningless.
% Although each change seems to make a marginal difference, 
% By adding all the terms, the performance gap between the one with none of the terms and all the terms are clearly noticeable.
% Because the first stage does not involves sample acquisition, 
% we do not compare the model in the first stage.
%\djkim{(WE should change this part according to the updated result.)}
%\textbf{\emph{+JSD}} improves the performance when we use \textbf{\emph{+Entropy}}.
\textbf{\emph{+Entropy}} improves the performance consistently.
\textbf{\emph{+Distillation}} improves the performance when we use either \textbf{\emph{+JSD}} or \textbf{\emph{+Entropy}}.
%Moreover, \textbf{\emph{+Entropy}} improves the performance when we use \textbf{\emph{+Distillation}}.
Moreover, \textbf{\emph{+JSD}} improves the performance when we use both \textbf{\emph{+Distillation}} and \textbf{\emph{+Entropy}}.
Among all the baselines, our final setups (which includes all \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, and \textbf{\emph{+Entropy}}) shows the best performance in all stages.







\begin{figure}[t]
\vspace{0mm}
\centering
   \includegraphics[width=.8\linewidth]{Figures/VizWiz_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VizWiz Dataset. Our proposed method shows the best performance in most of the sampling stages.}
\label{fig:VizWiz}
\vspace{-2mm}
\end{figure}





\subsection{Results on VizWiz VQA Dataset}

To demonstrate the effectiveness of our method, we also evaluate our method on another VQA dataset, the VizWiz VQA~\cite{gurari2018vizwiz} dataset, that is arguably more difficult.
The VizWiz dataset contains 19,425 train image/question pairs and we sample 1,900 image/question pairs per stage with the final stage ending at 19,000 image/question pairs.
For architecture, we use a publicly available code of~\cite{yang2016stacked}\footnote{https://github.com/DenisDsh/VizWiz-VQA-PyTorch}, and show that our method is model agnostic.

We use the same baselines as the previous subsection, and experimental results are shown in \Fref{fig:VizWiz}.
As VizWiz is a more challenging dataset than VQA v2.0 dataset, %we have these and these and these results....
all the baselines show similar performance. Even the recent state-of-the-art such as \textbf{\emph{VAAL}} and \textbf{\emph{SRAAL}} show performance similar to that of all other baselines with no baseline being clearly above another.
% lower performance overall.
% One interesting observation is that, different from the other experiments, \textbf{\emph{LC}} shows better performance than \textbf{\emph{Random}} baseline.
Among all other baselines, our proposed method shows the best performance in most of the sampling stages. 





\begin{figure}[t]
\vspace{0mm}
\centering
   \includegraphics[width=.8\linewidth]{Figures/CP2_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VQA-CP2 Dataset. Our model shows favorable performance compared to the baseline approaches in most of the stages.}
\label{fig:VQA-CP2}
\vspace{0mm}
\end{figure}



\subsection{Results on VQA-CP2 Dataset}
We also evaluate our method the VQA-CP2~\cite{goyal2017making} dataset, which has a different data distribution between training and test splits.
VQA-CP2 is usually used to evaluate the robustness in uni-modal bias in VQA models.
As VQA-CP2 is a rearrangement of the VQA v2.0 dataset, the VQA-CP2 dataset size is similar yet slightly different and contains 438K train image/question pairs and we sample 40K image/question pairs per stage with the final stage ending at 400K image/question pairs.
We use the same network architecture from~\cite{anderson2018bottom} and we use the same baselines as VQA v2.0.

The experimental results on VQA-CP2 dataset is shown in \Fref{fig:VQA-CP2}.
Among the existing approaches, \textbf{\emph{Entropy}} shows the best performance, and the recent state-of-the-art methods of \textbf{\emph{VAAL}} and \textbf{\emph{SRAAL}} show mediocre performance, sometimes even performing worse than \textbf{\emph{Random}}.
Our model shows the highest peak performance and we can see an interesting case where \textbf{\emph{Entropy}} also peaks above the Reference.
We can conclude that our method is robust for modality bias as well.
Note that when tested on all 438K training data, the model performance showed to be 39.91\% (denoted by Reference in \Fref{fig:VQA-CP2}) which is lower than the performance of \emph{\textbf{Entropy}} and \emph{\textbf{Ours} trained with the subset of the training data}. 
%but using some of the Active Learning methods such as \emph{\textbf{Entropy}} and \emph{\textbf{Ours}} 
This
shows that by elaborately sampling some of the meaningful data, we are able to surpass the performance from the full dataset. We believe that this finding opens up interesting possible future research ideas.


\subsection{Results on NTU Action Recognition Dataset}
Although our model is designed specifically for a model with multi-modal input (\emph{e.g.}, vision-language tasks), we also evaluate our model on one of the popular multi-modal action recognition datasets, NTU RGB+D dataset~\cite{shahroudy2016ntu}, in order to show the extensibility of our approach.
We show through experiments the effectiveness of our approach,
% Although the motivation for our work comes from multi-modal inputs and show through experiments the effectiveness of our approach, \jwcho{redundant}
and we believe that this method can be expanded to experiments that use multiple inputs. 

We %experiment on
use the model from~\cite{li2018co} with the NTU RGB+D dataset~\cite{shahroudy2016ntu} which leverages multiple views or subjects with the same action class and trains the network for improved performance.
The dataset processing used in the implementation of~\cite{li2018co} makes use of 37,646 pairs of inputs and we sample 3,000 at each stage, ending at 30,000 pairs at the last stage. 
We followed the cross-subject evaluation~\cite{shahroudy2016ntu} that splits the 40 subjects into training and testing sets.
We apply our method on the subject dataset and treat each subject as a single modality and train additional classifiers similar to the VQA settings. 

We use the same baselines as the previous subsection, and show experimental results in \Fref{fig:NTU}.
%We create the base active learning baselines and show through~\Fref{fig:NTU} 
% the effectiveness of our approach on this setting as well. 
%and demonstrate that 
Note that the gap between \textbf{\emph{Margin}} or \textbf{\emph{LC}} and the other baselines is larger than that of the previous experiments.
Among \textbf{\emph{Random}}, \textbf{\emph{Entropy}}, \textbf{\emph{LL}}, \textbf{\emph{VAAL}}, and \textbf{\emph{SRAAL}},
\textbf{\emph{LL}} and \textbf{\emph{VAAL}} shows the best performance in the early stages, and \textbf{\emph{Entropy}} shows the best performance in the later stages.
Moreover, compared to the baseline approaches, our method shows favorable performance 
%compared to the baseline approaches 
for all sampling stages in the NTU RGB+D dataset as well.
The effectiveness of our approach opens up the possibilities of applying our method on other kinds of datasets and tasks where multiple inputs maybe used whether they are of the same modality of not.



\begin{figure}[t]
\vspace{0mm}
\centering
   \includegraphics[width=.8\linewidth]{Figures/NTU_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the NTU RGB+D Action Recognition Dataset. Although our method is designed specifically for VQA task, our method consistently outperforms all the existing approaches in every sampling stage in terms of action recognition accuracy.}
\label{fig:NTU}
\vspace{0mm}
\end{figure}



==> Legacy/unused_4_sec_experiment_humantech.tex <==
In this section, we describe the experimental setups, competing methods, and provide performance evaluations of the proposed methods.
% \djkim{TODO : add results of additional baselines (VAAL, SRAAL, and maybe core-set?)}









\subsection{Implementation Details}
The VQA 2.0 Dataset can be found at this link (\url{https://visualqa.org/}).
Following the model from~\cite{anderson2018bottom}, we make use of the pre-extracted image features from Mask-RCNN~\cite{he2017mask} for the visual input and Glove6B~\cite{pennington2014glove} embedding with a GRU~\cite{chung2014empirical} to process the question features. Then, the features are attended using the modified version of the attention proposed in~\cite{anderson2018bottom}~\footnote{The modified version of the attention proposed in~\cite{anderson2018bottom} is found on this github link: https://github.com/hengyuan-hu/bottom-up-attention-vqa}.
We train our model with a batch size of 512 and use the Adamax optimizer from the PyTorch library. The hyperparameters used are: Learning Rate: 0.002, Betas: (0.9, 0.999), eps: 1$e^{-0.8}$, Weight Decay: 0.
Model hyperparameters are listed next. The vocabulary size used is 19902, the output of the Mask-RCNN is 2048, as for the Attention, the input is set at 2048 for the visual input, but all hidden states, question input, and output values are set to 1024. The word embedding size used is 300, and the GRU hidden state is set to 1024. The classifier, which can be seen as all 3 classifiers as stated in the method section of our paper, has an input of 1024 and an output of 3129, which is the number of answer candidates.
% Following this, a classifier layer is used to classify the outputs. In addition to the classifier layer which takes the attended features as its input, we create 2 more classifier layers which takes the single modalities as its input as shown in~\ref{fig:architecture} as $g{\_}v(\cdot)$ and $g{\_}q(\cdot)$ respectively. These classifiers have the same exact properties as $g(\cdot)$, the only difference is that while $g(\cdot)$ takes in the input of $Z$ as shown in equation (2), classifiers $g{\_}v(\cdot)$ takes in $Z\textsubscript{v}$ and $g{\_}q(\cdot)$ takes in $Z\textsubscript{q}$. 

The VQA accuracy measure that we used is the from~\cite{antol2015vqa} and can be summarised as follows:
\begin{equation}
    Accuracy(A) = min\left\{\frac{\text{\# of humans that said }A}{3}, 1\right\},
    \label{eqn:VQA_accuracy}
\end{equation}
where $A$ is the Answer prediction from the model.

For our Active Learning setup, we set 10 stages with 40,000 question image pairs for each step, and increase 40,000 pairs each time, ending up at 400,000 at the final stage. We do not reinitialize the model each time but continue using the model that was previously trained. At Stage 0, we train the model for 20 epochs. For the next Stages from 1 to 9, as the model is already pre-trained in the previous stages, we train for only 10 epochs each. At the end of each epoch, the model is evaluated on the validation set that stays static and the evaluation score of the best is chosen at the end of each stage and reported as the accuracy of that stage including Stage 0.

Our model takes around 10 hours to train all 10 stages on a single Nvidia Titan Xp (12GB) GPU.





\subsection{Experimental Setup for VQA v2.0 Dataset}
%\subsection{Experiments on VQA v2.0}
\noindent\textbf{Dataset and metric.}
We evaluate our method on VQA v2.0 dataset~\cite{antol2015vqa}, which consists of 1.1M data points (visual-question-answer triplets), with 444K/214K/448K for train/val/test respectively.
Each image is set up with at least 3 questions and 10 answers per question and thus contains 204K images, 1.1M questions, 11.1M answers.
As for evaluation, we utilize the VQA accuracy metric~\cite{antol2015vqa}.


\noindent\textbf{Active Learning setup.}
For the Active Learning (AL) setup, labeled set $\mathcal{D}\textsubscript{L}$ with a size of 40,000 out of 443,757 training data points, which is roughly 10\% of the full dataset,
% \djkim{(as most of the existing AL works set 10\% of the full dataset as the budget)} 
is initialized randomly, and our model is trained until the training loss converges.
After converging, which marks the end of the first stage, we use this model to collect the samples from the unlabeled dataset $\mathcal{D}\textsubscript{U}$ according to an acquisition function $S(V,Q)$.
For every stage, we sample the next 40,000 data points from the unlabeled dataset and add them to the labeled dataset.
After increasing the labeled set, we train a newly initialized model using the resulting labeled set, and repeat the previous steps (marking the subsequent stages), increasing the dataset and training models for 10 iterations, resulting in a final $\mathcal{D}\textsubscript{L}$ size of 400,000 data points.



\noindent\textbf{Implementation details.}
%\subsection{Details of Network Architecture}
The base network architecture we adopt for this VQA task is identical to that of~\cite{anderson2018bottom}, with modifications to the classifier layer as we include 3 different classifiers. 
Full implementation details can be found in the supplementary section.
% Model architecture implementation details can be found in the supplementary section of this paper.
The only changes we make to the model is two additional classifier layers which takes the single modalities as its input as shown in~\Fref{fig:architecture} as $g_v(\cdot)$ and $g_q(\cdot)$ respectively. These classifiers are identical to the model's original classifier, $g(\cdot)$, and the difference is that while $g(\cdot)$ takes in the input of $\mathbf{z}$ as shown in equation (2), classifiers $g_v(\cdot)$ takes in $\mathbf{z}\textsubscript{v}$ and $g_q(\cdot)$ takes in $\mathbf{z}\textsubscript{q}$. 
Because we use identical classifiers, our method does not significantly increase parameters or calculation costs, making it cost-effective. In addition to this, we detach the classifiers from the model so the presence of the classifiers do not affect the performance of the model at all.
More details can be found in the supplementary material along with qualitative results on the VQA v2.0 dataset.
% -------------------------- move to supple? ---------------------------------
% Following the model from~\cite{anderson2018bottom}, we make use of the pre-extracted image features from Mask-RCNN~\cite{he2017mask} for the visual input and Glove6B~\cite{pennington2014glove} embedding with a GRU~\cite{chung2014empirical} to process the question features. Then, the features are attended using the modified version of the attention proposed in~\cite{anderson2018bottom}~\footnote{The modified version of the attention proposed in~\cite{anderson2018bottom} is found on this github link: https://github.com/hengyuan-hu/bottom-up-attention-vqa}.
% Following this, a classifier layer is used to classify the outputs. In addition to the classifier layer which takes the attended features as its input, we create 2 more classifier layers which takes the single modalities as its input as shown in~\ref{fig:architecture} as $g{\_}v(\cdot)$ and $g{\_}q(\cdot)$ respectively. These classifiers have the same exact properties as $g(\cdot)$, the only difference is that while $g(\cdot)$ takes in the input of $Z$ as shown in equation (2), classifiers $g{\_}v(\cdot)$ takes in $Z\textsubscript{v}$ and $g{\_}q(\cdot)$ takes in $Z\textsubscript{q}$. 
% \djkim{(maybe move this to the supplementary?)}
% ------------------------------------------------------------------------


\noindent\textbf{Baseline approaches.}
In order to demonstrate the effectiveness of our method, we compare the performance of our model to widely used sample acquisition approaches~\cite{culotta2005reducing,scheffer2001active,shen2017deep} as well as the recent deep Active Learning method~\cite{sinha2019variational,yoo2019learning,zhang2020state}:%\djkim{(Require explanation why we don't use VAAL or SAAL etc.)}~\jwcho{(tried to answer in related works. maybe that is a good enough explanation)}
{\setdefaultleftmargin{3mm}{}{}{}{}{}
\begin{itemize}
    \item \textbf{\emph{Random}} passive learning strategy that queries points following a uniformly random distribution.
    \item \textbf{\emph{Entropy}~\cite{shen2017deep}} queries instances that maximize the entropy of a model's output: $S(V,Q)=H(\hat{Y})$.
    \item \textbf{\emph{Margin}~\cite{scheffer2001active}} queries instances with the least margin between the output probabilities for the two most likely generated answers of a model: $S(V,Q)=1 + \hat{\mathbf{y}}^1-\hat{\mathbf{y}}^2$, where $\hat{\mathbf{y}}^1$ and $\hat{\mathbf{y}}^2$ are the probability of the first and second most confident model's responses.
    \item \textbf{\emph{Least Confident (LC)}~\cite{culotta2005reducing}} queries instances for which a model has the least confidence in its most likely generated sequence: $S(V,Q)=1-\hat{\mathbf{y}}^*$, where $\hat{\mathbf{y}}^*$ is the probability of the most confident model's response.
    \item \textbf{\emph{Learning Loss (LL)}~\cite{yoo2019learning}} adds a loss prediction module which measures how much a sample would affect the loss if sampled.
    \item \textbf{\emph{Variational Adversarial Active Learning (VAAL)}~\cite{sinha2019variational}} adds a VAE to generate a latent space and discriminate between labeled and unlabeled samples.
    \item \textbf{\emph{State Relabeling Adversarial Active Learning (SRAAL)}~\cite{zhang2020state}} Similar to VAAL, but also leverages the uncertainty of the task model to discriminate samples.
\end{itemize}
}

% \begin{figure}[t]
% \centering
% \vspace{-2mm}
% %\resizebox{1\linewidth}{!}{%
% %{\includegraphics[width=.8\linewidth,keepaspectratio]{Figures/quantitative_final}}
% {\includegraphics[width=1\linewidth,keepaspectratio]{Figures/quantitative_VQA_new}}
% %}
% %\vspace{-2mm}
% \caption{Comparison with existing approaches on the VQA v2.0 dataset. Reference is the best performance of the existing methods.
% Our model shows the best performance among all the other methods by a large margin.}
% \vspace{-2mm}
% \label{fig:quantitative}
% \end{figure}

\begin{table*}[t]
\vspace{-2mm}
\centering
\caption{Ablation study of our method. Our final method (the last row) shows the best performance among the variants of our methods in most of the Active Learning stages.%\djkim{(Justification to use Table. Mention that it is the same as Figures but more fine-grained values)}
}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{ c|ccc|cccccccccc }
    \hline
    Method&\textbf{\emph{+JSD}}&\textbf{\emph{+Distillation}}&\textbf{\emph{+Entropy}}&1&2&3&4&5&6&7&8&9&10\\
    \hline
    %Random&&&&50.42&53.93&	55.38&	56.72&	57.45&	57.93&	58.26&	58.49&	59.20&	59.33\\
    %Entropy&&&&50.16&	52.66&	54.24&	55.62&	56.59&	57.20&	58.19&	58.61&	59.28&	59.04\\
    Random&&&&50.56	&54.55	&55.93	&56.91	&58.59	&59.46	&60.27	&60.34	&61.11	&61.21\\
    Entropy&&&&50.74	&54.07	&55.49	&56.51	&58.21	&58.67	&60.30	&61.25	&61.50	&61.59\\
    \hline

    %\multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$        &50.52	&54.06	&55.59	&56.85	&57.70	&58.55	&59.06	&59.52	&59.93	&60.12\\%&50.33	&54.05	&\textbf{55.96}	&57.14	&57.90	&58.56	&59.13	&59.54	&60.10	&60.30\\
    %&$\checkmark$&$\times$&$\times$      &50.81	&53.92	&55.55	&56.78	&57.69	&58.32	&58.94	&59.33	&59.64	&60.02\\
    %&$\times$&$\checkmark$&$\times$      &50.27	&54.10	&55.77	&57.08	&57.89	&58.52	&59.03	&59.46	&59.89	&60.20\\
    %&$\checkmark$&$\checkmark$&$\times$    &50.77	&54.08	&55.78	&57.02	&57.90	&58.60	&59.13	&59.63	&59.91	&60.24\\
    %&$\times$&$\times$&$\checkmark$      &50.65	&53.97	&55.42	&56.65	&57.63	&58.51	&59.27	&59.82	&60.20	&60.36\\
    %&$\checkmark$&$\times$&$\checkmark$    &49.94	&53.61	&55.45	&56.75	&57.77	&58.61	&59.47	&60.04	&60.39	&60.53\\
    %&$\times$&$\checkmark$&$\checkmark$    &50.39	&53.98	&\textbf{55.92}	&\textbf{57.21}	&58.05	&58.84	&59.54	&60.09	&60.50	&60.61\\
    %&$\checkmark$&$\checkmark$&$\checkmark$ &{50.03}	&\textbf{54.13}	&{55.71}	&{56.99}	&\textbf{58.06}	&\textbf{58.85}	&\textbf{59.66}	&\textbf{60.21}	&\textbf{60.61}	&\textbf{60.81}\\
    
    
    \multirow{8}{*}{\textbf{Ours}}&$\times$&$\times$&$\times$  &49.91	&54.34	&56.80	&58.21	&59.53	&60.62	&61.20	&62.02	&62.60	&63.10\\
    &$\checkmark$&$\times$&$\times$                             &50.10	&54.11	&56.14	&57.89	&59.21	&60.20	&61.24	&61.86	&62.55	&63.11\\
    &$\times$&$\checkmark$&$\times$                             &50.49	&54.36	&56.79	&\textbf{58.30}	&59.42	&60.49	&61.05	&62.00	&62.45	&62.92\\
    &$\checkmark$&$\checkmark$&$\times$                         &50.30	&54.35	&56.29	&58.08	&59.20	&60.27	&61.14	&61.79	&62.51	&63.06\\
    &$\times$&$\times$&$\checkmark$                             &50.32	&54.61	&56.81	&58.29	&59.34	&60.41	&61.61	&62.40	&62.94	&63.22\\
    &$\checkmark$&$\times$&$\checkmark$                         &50.23	&54.44	&56.63	&58.22	&59.13	&60.42	&61.67	&\textbf{62.47}	&62.94	&63.26\\
    &$\times$&$\checkmark$&$\checkmark$                         &50.43	&54.30	&56.76	&58.25	&59.44	&60.32	&61.55	&62.45	&62.97	&63.29\\
    &$\checkmark$&$\checkmark$&$\checkmark$                     &50.51	&\textbf{54.86}	&\textbf{56.82}	&\textbf{58.30}	&\textbf{59.55}	&\textbf{60.63}	&\textbf{61.74}	&\textbf{62.47}	&\textbf{63.00}	&\textbf{63.31}\\
    
    \hline
\end{tabular}
}

%\vspace{-2mm}
\label{table:ablation_ours}
\end{table*}


\subsection{Results on VQA v2.0 Dataset}
% \djkim{(TODO : The improvements might be incremental. Need to improve.)}

%\djkim{(The reason why LC and margin are worse than random? Because the number of the classes are extremely large. Also, long-tailed distribution can be a problem.)}

% \djkim{(TODO : compare with ``Learning by asking Questions'' and ``VQA as meta-learning'', ``Learning loss for AC''. Maybe ``Core-set approach'' and ``query-by-committe''?)}

%\djkim{(TODO : other VQA datasets, CLEVER? VQAcp? VizWiz?)}

% \djkim{(TODO : different VQA architecture, CNN+LSTM, or BAN. Compare the gain from architecture and AL $\rightarrow$maybe we can't. the performance gain from the architecture is more than that from AL.)}

\noindent\textbf{Comparison with existing approaches.}
We compare our final method to existing AL methods~\cite{culotta2005reducing,scheffer2001active,shen2017deep,yoo2019learning} that do not originally consider multi-modality in \Fref{fig:quantitative}.
Among the existing methods, \textbf{\emph{Margin}} and \textbf{\emph{Least Confident(LC)}} show similarly poor performance, while \textbf{\emph{Random}} and \textbf{\emph{Entropy}} show better performance in the early stage and the late stage respectively. 
We conjecture that the poor performance of \textbf{\emph{Margin}} and \textbf{\emph{LC}} is due to the large number of classes. In VQA v2.0 dataset, there are 3129 number of candidate classes, even after cutting out redundant classes and answers that appear less than 9 times, which is noticeably larger than typical image classification datasets (\emph{i.e.}, ImageNet). The large number of classes can also cause the long-tailed distribution problem which makes AL with conventional approaches difficult. In particular, the model predictions might be dominated to major classes; thus regarding only the most confident class (\textbf{\emph{LC}}) or second (\textbf{\emph{Margin}}) might lead to biased acquisition to major classes.
Between \textbf{\emph{Random}} and \textbf{\emph{Entropy}},
\textbf{\emph{Random}} shows a higher score in the early stage, and \textbf{\emph{Entropy}} surpasses \textbf{\emph{Random}} in the later stages.
%A recent approach, \textbf{\emph{LL}}, shows
Note that recent state-of-the-art Active Learning methods, \textbf{\emph{LL}}, \textbf{\emph{VAAL}}, \textbf{\emph{VRAAL}}, show similar performance to \textbf{\emph{Random}} and \textbf{\emph{Entropy}} in VQA task.
Moreover, our proposed method shows the best performance compared to all the counterparts by a large margin in all stages.
Note that the best among the existing approaches achieved 59.28\% accuracy when using 400K training samples, which is similar performance of our model trained with 240K training samples, signifying that our method SMEM can save about 30\% of the human labeling effort compared to existing approaches.


\begin{figure*}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=.7\linewidth]{Figures/qualitative}\\
   \includegraphics[width=.7\linewidth]{Figures/qualitative3}\\
   \includegraphics[width=.7\linewidth]{Figures/qualitative2}
   \caption{Qualitative result of the Top-1 prediction of our model for every Active Learning stage.}
\label{fig:qualitative}
\end{figure*}




\noindent\textbf{Ablation study.}
We perform an ablation study on each of the  components of our final method.
% In addition, we also perform an analysis on each of the components of our final method.
\textbf{\emph{+Distillation}} is for the proposed self-distillation loss described 
% in \Sref{sec:distillation}.
previously.
\textbf{\emph{+Entropy}} indicates the additional entropy term of the ``main'' branch output $H(\hat{Y})$ which changes our acquisition function from \Eref{eqn:addJSD} to \Eref{eqn:final}.
\textbf{\emph{+Jensen-Shannon Divergence (+JSD)}} is the additional JSD term which changes our acquisition function from \Eref{eqn:student} to \Eref{eqn:addJSD}.



% Finally, we perform an ablation study on each of the components of our SMEM method, and we show the
\Tref{table:ablation_ours} shows the fine-grained performance changes caused by the auxiliary terms, \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, \textbf{\emph{+Entropy}}.
We include traditional approaches, \textbf{\emph{Random}} and \textbf{\emph{Entropy}}, to compare with our methods. 
Although the performance improvements from each auxiliary terms might be seem marginal, we emphasize that the performance gain between \textbf{\emph{Entropy}} and our proposed SMEM model is noticeable.
Note that our model without any auxiliary terms already shows favorable performance at AL stages.
Since the first stage is randomly initialized, comparison in the first stage is meaningless.
Although each change seems to make a marginal difference, by adding all the terms, the performance gap between the one with none of the terms and all the terms are clearly noticeable.
% Because the first stage does not involves sample acquisition, 
% we do not compare the model in the first stage.
%\djkim{(WE should change this part according to the updated result.)}
%\textbf{\emph{+JSD}} improves the performance when we use \textbf{\emph{+Entropy}}.
\textbf{\emph{+Entropy}} improves the performance consistently.
\textbf{\emph{+Distillation}} improves the performance when we use either \textbf{\emph{+JSD}} or \textbf{\emph{+Entropy}}.
%Moreover, \textbf{\emph{+Entropy}} improves the performance when we use \textbf{\emph{+Distillation}}.
Moreover, \textbf{\emph{+JSD}} improves the performance when we use both \textbf{\emph{+Distillation}} and \textbf{\emph{+Entropy}}.
Among all the baselines, our final setups (which includes all \textbf{\emph{+JSD}}, \textbf{\emph{+Distillation}}, and \textbf{\emph{+Entropy}}) shows the best performance in all stages.





\begin{figure*}[t]
%\vspace{-4mm}
\centering
%\resizebox{1\linewidth}{!}{%
\subfigure[Vanilla]{\includegraphics[width=0.33\linewidth]{Figures/ablation_plain}}
\subfigure[+Distillation]{\includegraphics[width=0.33\linewidth]{Figures/ablation+distillation}}
\subfigure[+Distillation+Entropy]{\includegraphics[width=0.33\linewidth]{Figures/ablation+distillation+entropy}}
%}
%\vspace{-2mm}
\caption{Comparison between different measuring methods for our method. 
Ours is the SMEM + JSD in all graphs above. 
(a):without anything, (b):with distillation loss, and (c):with both distillation loss and entropy.}
%\vspace{-2mm}
\label{fig:ablation}
\end{figure*}




\subsection{Additional Analysison VQA v2.0 Dataset}

\noindent\textbf{Other Approaches of Active Learning.}
As the comparison target of our approach, we also test different measures for distribution discrepancy.
In the following paragraphs, we introduce several possible candidates to measure the distances between single-modal and multi-modal answer representations.

\textbf{\emph{(1) KL-Divergence (KLD)}} is defined as follows:
\begin{equation}
    D_{KL}(\mathbf{y}||\mathbf{y}_q) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_q)}, %= H(Y,Y_q) - H(\hat{Y}),
\end{equation} 
\begin{equation}
    D_{KL}(\mathbf{y}||\mathbf{y}_v) = \sum_{i=1}^{|\mathcal{A}|}{\mathbf{y}^i\log(\mathbf{y}^i/\mathbf{y}^i_v)}. %= H(Y,Y_v) - H(\hat{Y}),
\end{equation} 
%where $H(Y,Y_q)$ and $H(Y,Y_v)$ are the cross-entropies of the single-modal answers compared to multi-modal answers.
Similar to our approach, by combining the two distance metrics via weighted sum, we have the KL-divergences:
\begin{equation}
    S(V,Q) = \alpha D_{KL}(\mathbf{y}||\mathbf{y}_q) + (1-\alpha) D_{KL}(\mathbf{y}||\mathbf{y}_v),
    \label{eqn:kld}
\end{equation}
where $\alpha$ is a hyper-parameter that weighs between visual and question scores.
Note that $S(V,Q)\geq0$, because KL-divergence is always non-negative.


\textbf{\emph{(2) Absolute Difference of KL-Divergence (AD-KLD)}} can also be used:
\begin{equation}
    S(V,Q) = |D_{KL}(\mathbf{y}||\mathbf{y}_q) - D_{KL}(\mathbf{y}||\mathbf{y}_v)|.
    \label{eqn:ad-kld}
\end{equation}
Although these methods have strong theoretical backing, we empirically show that for our problem, our proposed method shows the best performance.



\noindent\textbf{Ablation study for other approaches.}
Here, we introduce variants of our sampling methods.
\textbf{{\emph{KL-Divergence (KLD)}}} is described in \Eref{eqn:kld}. %\djkim{(multimodal1,2)}
\textbf{\emph{Jensen-Shannon Divergence only (JSD)}} is the baseline that is sampled by only using Jensen-Shannon divergence described as: %in \Eref{eqn:jsd}. %\djkim{(multimodal3)}
\begin{equation}
    JSD(\mathbf{y}_v||\mathbf{y}_q) = (D_{KL}(\mathbf{y}_v||M)+D_{KL}(\mathbf{y}_q||M))/2, 
    \label{eqn:jsd2}
\end{equation}
where  $M = (\mathbf{y}_v+\mathbf{y}_q)/2$. 
\textbf{\emph{Absolute Difference of KL-Divergence (AD-KLD)}} is described in \Eref{eqn:ad-kld}. %\djkim{(multimodal6)}
\textbf{\emph{Mutual Information (MI)}} is the baseline that is sampled by only using mutual information: $S(V,Q) = \alpha I(A;V|Q) + (1-\alpha) I(A;Q|V)$. %\djkim{(multimodal7,8)}
\textbf{\emph{Single-Modal Entropic Measure (SMEM) or (Ours)}} is our proposed method:% either before or after adding entropy term as described in \Eref{eqn:addJSD} or \Eref{eqn:final}.  %\djkim{(multimodalV,Q)}
\begin{equation}
    S(V,Q) = \alpha H(Y_q) + (1-\alpha) H(Y_v) + \beta JSD(\mathbf{y}_v||\mathbf{y}_q) + \gamma H(\hat{Y}).
    \label{eqn:finalfinal}
\end{equation}


The ablation study results are illustrated in \Fref{fig:ablation}.
We compare the AL performance of our model with other design choices for distribution discrepancy measures.
We draw the training curves for three different setups: (a) without distillation or entropy, (b) adding distillation loss only, and (c) adding distillation loss and entropy.
Each setup shows its strengths in different areas of the AL stages.
In (a), ours shows the best performance in the early stages with less data while \textbf{\emph{KLD}} shows better performance in the later stages as more data is accumulated.
In (b), ours shows the best performance with less data while \textbf{\emph{MI}} shows better performance as more data is accumulated.
In (c), we show that by taking the main entropy into account, our model shows the best performance compared to all the other design choices throughout all given stages.






\noindent\textbf{Qualitative Results}
\Fref{fig:qualitative} shows the qualitative results of our model for every AL stage. 
For each stage, we show the Top-1 predicted answer colored in blue if correct and red if not correct.
As the AL stages progress, the model is trained to generate increasingly accurate answers.
%More qualitative results can be found in the supplementary material.




\begin{figure}[b]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/VizWiz_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VizWiz Dataset. Our proposed method shows the best performance in most of the sampling stages.}
\label{fig:VizWiz}
\vspace{-2mm}
\end{figure}





\subsection{Results on VizWiz VQA Dataset}

To demonstrate the effectiveness of our method, we also evaluate our method on another VQA dataset, the VizWiz VQA~\cite{gurari2018vizwiz} dataset, that is arguably more difficult.
The VizWiz dataset contains 19,425 train image/question pairs and we sample 1,900 image/question pairs per stage with the final stage ending at 19,000 image/question pairs.
For architecture, we use a variant of~\cite{yang2016stacked}\footnote{https://github.com/DenisDsh/VizWiz-VQA-PyTorch}.

We use the same baselines as the previous subsection, and experimental results are shown in \Fref{fig:VizWiz}.
As VizWiz is a more challenging dataset than VQA v2.0 dataset, %we have these and these and these results....
all the baselines show similar performance. Even the recent state-of-the-art such as \textbf{\emph{VAAL}} and \textbf{\emph{SRAAL}} show performance similar to that of all other baselines with no baseline being clearly above another.
% lower performance overall.
% One interesting observation is that, different from the other experiments, \textbf{\emph{LC}} shows better performance than \textbf{\emph{Random}} baseline.
Among all other baselines, our proposed method shows the best performance in most of the sampling stages.





\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/CP2_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the VQA-CP2 Dataset. Our model shows favorable performance compared to the baseline approaches in most of the stages.}
\label{fig:VQA-CP2}
\vspace{-2mm}
\end{figure}

\subsection{Results on VQA-CP2 Dataset}
We also evaluate our method the VQA-CP2~\cite{goyal2017making} dataset, which has a different data distribution between training and test splits.
VQA-CP2 is usually used to evaluate the robustness in uni-modal bias in VQA models.
As VQA-CP2 is a rearrangement of the VQA v2.0 dataset, the VQA-CP2 dataset size is similar yet slightly different and contains 438K train image/question pairs and we sample 40K image/question pairs per stage with the final stage ending at 400K image/question pairs.
We use the same network architecture from~\cite{anderson2018bottom} and we use the same baselines as VQA v2.0.

The experimental results on VQA-CP2 dataset is shown in \Fref{fig:VQA-CP2}.
Among the existing approaches, \textbf{\emph{Entropy}} shows the best performance, and the recent state-of-the-art methods of \textbf{\emph{VAAL}} and \textbf{\emph{SRAAL}} show mediocre performance, sometimes even performing worse than \textbf{\emph{Random}}.
Our model shows the highest peak performance and we can see an interesting case where \textbf{\emph{Entropy}} also peaks above the Reference.
We can conclude that our method is robust for modality bias as well.
Note that when tested on all 438K training data, the model performance showed to be 39.91\% (denoted by Reference in \Fref{fig:VQA-CP2}) which is lower than the performance of \emph{\textbf{Entropy}} and \emph{\textbf{Ours} trained with the subset of the training data}. 
%but using some of the Active Learning methods such as \emph{\textbf{Entropy}} and \emph{\textbf{Ours}} 
This
shows that by elaborately sampling some of the meaningful data, we are able to surpass the performance from the full dataset. We believe that this finding opens up interesting possible future research ideas.


\begin{figure}[t]
\vspace{-2mm}
\centering
   \includegraphics[width=1\linewidth]{Figures/NTU_2.pdf}
   \vspace{-2mm}
   \caption{Comparison with existing approaches on the NTU RGB+D Action Recognition Dataset. Although our method is designed specifically for VQA task, our method consistently outperforms all the existing approaches in every sampling stage in terms of action recognition accuracy.}
\label{fig:NTU}
\vspace{-2mm}
\end{figure}

\subsection{Results on NTU Action Recognition Dataset}
Although our model is designed specifically for a model with multi-modal input (\emph{e.g.}, vision-language tasks), we also evaluate our model on one of the popular multi-modal action recognition datasets, NTU RGB+D dataset~\cite{shahroudy2016ntu}, in order to show the extensibility of our approach.
We show through experiments the effectiveness of our approach,
% Although the motivation for our work comes from multi-modal inputs and show through experiments the effectiveness of our approach, \jwcho{redundant}
and we believe that this method can be expanded to experiments that use multiple inputs. 

We %experiment on
use the model from~\cite{li2018co} with the NTU RGB+D dataset~\cite{shahroudy2016ntu} which leverages multiple views or subjects with the same action class and trains the network for improved performance.
The dataset processing used in the implementation of~\cite{li2018co} makes use of 37,646 pairs of inputs and we sample 3,000 at each stage, ending at 30,000 pairs at the last stage. 
We followed the cross-subject evaluation~\cite{shahroudy2016ntu} that splits the 40 subjects into training and testing sets.
We apply our method on the subject dataset and treat each subject as a single modality and train additional classifiers similar to the VQA settings. 

We use the same baselines as the previous subsection, and show experimental results in \Fref{fig:NTU}.
%We create the base active learning baselines and show through~\Fref{fig:NTU} 
% the effectiveness of our approach on this setting as well. 
%and demonstrate that 
Note that the gap between \textbf{\emph{Margin}} or \textbf{\emph{LC}} and the other baselines is larger than that of the previous experiments.
Among \textbf{\emph{Random}}, \textbf{\emph{Entropy}}, \textbf{\emph{LL}}, \textbf{\emph{VAAL}}, and \textbf{\emph{SRAAL}},
\textbf{\emph{LL}} and \textbf{\emph{VAAL}} shows the best performance in the early stages, and \textbf{\emph{Entropy}} shows the best performance in the later stages.
Moreover, compared to the baseline approaches, our method shows favorable performance 
%compared to the baseline approaches 
for all sampling stages in the NTU RGB+D dataset as well.
The effectiveness of our approach opens up the possibilities of applying our method on other kinds of datasets and tasks where multiple inputs maybe used whether they are of the same modality of not.






